37 New Validated Planets in Overlapping K2 Campaigns

We analysed 68 candidate planetary systems first identified during Campaigns 5 and 6 (C5 and C6) of the NASA \textit{K2} mission. We set out to validate these systems by using a suite of follow-up observations, including adaptive optics, speckle imaging, and reconnaissance spectroscopy. The overlap between C5 with C16 and C18, and C6 with C17, yields lightcurves with long baselines that allow us to measure the transit ephemeris very precisely, revisit single transit candidates identified in earlier campaigns, and search for additional transiting planets with longer periods not detectable in previous works. Using \texttt{vespa}, we compute false positive probabilities of less than 1\% for 37 candidates orbiting 29 unique host stars and hence statistically validate them as planets. These planets have a typical size of $2.2R_{\oplus}$ and orbital periods between 1.99 and 52.71 days. We highlight interesting systems including a sub-Neptune with the longest period detected by \textit{K2}, sub-Saturns around F stars, several multi-planetary systems in a variety of architectures. These results show that a wealth of planetary systems still remains in the \textit{K2} data, some of which can be validated using minimal follow-up observations and taking advantage of analyses presented in previous catalogs.

==> K2 in Cancri and Virginis arxiv/authors.tex <==
\author[J.~P.~de~Leon et al.]{J.~P.~de~Leon\orcid{0000-0002-6424-3410},$^{1}$\thanks{E-mail: jpdeleon@g.ecc.u-tokyo.ac.jp}
J.~Livingston\orcid{0000-0002-4881-3620},$^{1}$
M.~Endl,$^{2}$
W.~D.~Cochran\orcid{0000-0001-9662-3496},$^{2,3}$
T.~Hirano\orcid{0000-0003-3618-7535},$^{4}$
\newauthor
R.~A.~Garc\'\i a\orcid{0000-0002-8854-3776},$^{5}$
S.~Mathur\orcid{0000-0002-0129-0316},$^{6,7}$
K.~W.~F.~Lam\orcid{0000-0002-9910-6088},$^{8}$
J.~Korth\orcid{0000-0002-0076-6239},$^{9}$
A.~A.~Trani\orcid{0000-0001-5371-3432},$^{10}$
\newauthor
F.~Dai\orcid{0000-0002-8958-0683},$^{11}$
E.~D{\'\i}ez~Alonso\orcid{0000-0002-5826-9892},$^{12}$
A.~Castro-Gonz{\'a}lez\orcid{0000-0001-7439-3618},$^{12}$
M.~Fridlund\orcid{0000-0002-0855-8426},$^{14}$
\newauthor
A.~Fukui\orcid{0000-0002-4909-5763},$^{15,6}$
D.~Gandolfi\orcid{0000-0001-8627-9628},$^{16}$
P.~Kabath\orcid{0000-0002-1623-5352},$^{17}$
M.~Kuzuhara,$^{18}$
R.~Luque,$^{6,7}$
\newauthor
A.B.~Savel\orcid{0000-0002-2454-768X},$^{19}$
H.~Gill\orcid{0000-0001-6171-7951},$^{20}$
C.~Dressing\orcid{0000-0001-8189-0233},$^{20}$
S.~Giacalone\orcid{0000-0002-8965-3969},$^{20}$
N.~Narita\orcid{0000-0001-8511-2981},$^{15,6,21,22}$
\newauthor
E.~Palle\orcid{0000-0003-0987-1593},$^{6,7}$
V.~Van~Eylen\orcid{0000-0001-5542-8870},$^{23}$
and M.~Tamura\orcid{0000-0002-6510-0681}$^{1,21,24}$
\\
{\textit Affiliations are listed at the end of the paper}
}

==> K2 in Cancri and Virginis arxiv/newcommands.tex <==
\newcommand{\etal}{\mbox{\rm et al.~}}
\newcommand{\microns}{\ensuremath{\mu m}\xspace} 
\newcommand{\ms}{\mbox{m\,s$^{-1}$}\xspace}
\newcommand{\kms}{\mbox{km\,s$^{-1}$}\xspace}
\newcommand{\ks}{\mbox{km\,s$^{-1}$}\xspace}
\newcommand{\kse}{\mbox{km\,s$^{-1}$}\xspace}
\newcommand{\mse}{\mbox{m\,s$^{-1}$}\xspace}
\newcommand{\msy}{\mbox{m\,s$^{-1}$\,yr$^{-1}$}\xspace}
\newcommand{\msye}{\mbox{m\,s$^{-1}$\,yr$^{-1}$}\xspace}
\newcommand{\msun}{$M_{\odot}$\xspace}
\newcommand{\msune}{$M_{\odot}$\xspace}
\newcommand{\rsun}{$R_{\odot}$\xspace}
\newcommand{\rsune}{$R_{\odot}$\xspace}
\newcommand{\mjup}{$M_{\rm JUP}$\xspace}
\newcommand{\mjupe}{$M_{\rm JUP}$\xspace}
\newcommand{\msat}{$M_{\rm SAT}$\xspace}
\newcommand{\msate}{$M_{\rm SAT}$\xspace}
\newcommand{\mnep}{$M_{\rm NEP}$\xspace}
\newcommand{\mnepe}{$M_{\rm NEP}$\xspace}
\newcommand{\mearth}{$M_\oplus$\xspace}
\newcommand{\rearth}{$R_\oplus$\xspace}
\newcommand{\searth}{$S_\oplus$\xspace}
\newcommand{\searthe}{$S_\oplus$\xspace}
\newcommand{\rjup}{R$_{\rm JUP}$\xspace}
\newcommand{\msinie}{$M \sin i$\xspace}
\newcommand{\vsinie}{$V \sin i$\xspace}
\newcommand{\mbsini}{$M_b \sin i$\xspace}
\newcommand{\mcsini}{$M_c \sin i$\xspace}
\newcommand{\mdsini}{$M_d \sin i$\xspace}
\newcommand{\chisq}{$\chi_{\nu}^2$\xspace}
\newcommand{\chinu}{$\chi_{\nu}$\xspace}
\newcommand{\chinusq}{$\chi_{\nu}^2$\xspace}
\newcommand{\arel}{$a_{\rm rel}$\xspace}
\newcommand{\feh}{\ensuremath{[\mbox{Fe}/\mbox{H}]}\xspace}
\newcommand{\rphk}{\ensuremath{R'_{\mbox{\scriptsize HK}}}\xspace}
\newcommand{\lrphk}{\ensuremath{\log{\rphk}}\xspace}
\newcommand{\caii}{\ion{Ca}{2} H \& K\xspace}
\newcommand{\caiih}{\ion{Ca}{2} H\xspace}
\newcommand{\mv}{\ensuremath{M_{\mbox{\scriptsize V}}}\xspace}
\newcommand{\cs}{$\sqrt{\chi^2_{\nu}}$\xspace}
\newcommand{\etaearth}{$\mathbf \eta_{\oplus}$\xspace}
\newcommand{\etaearthe}{$\mathbf \eta_{\oplus}$\xspace}
\newcommand{\sini}{\ensuremath{\sin i}\xspace}
\newcommand{\msini}{\ensuremath{M \sin i}\xspace}
\newcommand{\mplsini}{\ensuremath{\mpl\sin i}\xspace}

\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%
\newcommand{\rmnum}[1]{\romannumeral #1}
\newcommand{\Rmnum}[1]{\expandafter\@slowromancap\romannumeral #1@}
\newcommand\sk[2]{Sk\,{$-#1{^\circ}#2$}}
\newcommand\tnc{\,\tablenotemark{c}}
\newcommand\tnd{\,\tablenotemark{d}}
\newcommand{\lsun}{$L_{\odot}$}
\newcommand{\vdag}{(v)^\dagger}
\newcommand{\MPS}{multi-planet systems\xspace}
\newcommand{\shk}{$S_\mathrm{HK}$\xspace}

%tools/software
\newcommand{\astropy}{\texttt{astropy}\xspace}
\newcommand{\isochrones}{\texttt{isochrones}\xspace}
\newcommand{\darthmouth}{\texttt{Darthmouth}\xspace}
\newcommand{\mist}{\texttt{MIST}\xspace}
\newcommand{\pytransit}{\texttt{PyTransit}\xspace}
\newcommand{\vespa}{\texttt{vespa}\xspace}
\newcommand{\batman}{\texttt{batman}\xspace}
\newcommand{\emcee}{\texttt{emcee}\xspace}
\newcommand{\lmfit}{\texttt{lmfit}\xspace}
\newcommand{\optimize}{\texttt{scipy.optimize}\xspace}
\newcommand{\trilegal}{\texttt{TRILEGAL}\xspace}
\newcommand{\everest}{\texttt{EVEREST}\xspace}
\newcommand{\ktwosff}{\texttt{K2SFF}\xspace}
\newcommand{\ktwophot}{\texttt{K2phot}\xspace}
\newcommand{\spock}{\texttt{spock}\xspace}
\newcommand{\dynamite}{\texttt{dynamite}\xspace}
\newcommand{\pyTTV}{\texttt{PyTTV}\xspace}
\newcommand{\celerite}{\texttt{celerite}\xspace}
\newcommand{\wotan}{\texttt{wotan}\xspace}
\newcommand{\tls}{\texttt{transit-least-squares}\xspace}
\newcommand{\isoclassify}{\texttt{isoclassify}\xspace}


% Stellar properties
\newcommand{\mstar}{\ensuremath{M_{\star}}\xspace}
\newcommand{\rstar}{\ensuremath{R_{\star}}\xspace} 
\newcommand{\lstar}{\ensuremath{L_{\star}}\xspace} 
\newcommand{\fe}{$[$Fe/H$]$\xspace}
\newcommand{\teff}{\ensuremath{T_{\mathrm{eff}}}\xspace}  
\newcommand{\logg}{\ensuremath{\log g}\xspace} 
\newcommand{\vsini}{\ensuremath{v \sin i}\xspace} 
\newcommand{\gcc}{g\,cm$^{-3}$\xspace} 
\newcommand{\gcce}{g\,cm$^{-3}$}
\newcommand{\dvdt}{\ensuremath{dv/dt}\xspace} 
\newcommand{\rhostar}{\ensuremath{\rho_{\star}}\xspace} 
\newcommand{\rhosun}{\ensuremath{\rho_{\odot}}\xspace} 

% planet parameters
\newcommand{\Mp}{\ensuremath{M_{P}}\xspace} 
% \newcommand{\Rp}{\ensuremath{R_P}\xspace}
\newcommand{\Prot}{$P_{\rm{rot}}$\xspace}
\newcommand{\Rp}{$R_\mathrm{P}$\xspace}
\newcommand{\Porb}{$P_\mathrm{orb}$\xspace}
\newcommand{\RpRs}{$R_p/R_s$\xspace}
\newcommand{\aRs}{$a/R_s$\xspace}
\newcommand{\To}{$T_0$\xspace}
\newcommand{\imppar}{$b$\xspace}
\newcommand{\Teq}{$T_{\mathrm{eq}}$\xspace}
\newcommand{\Me}{\ensuremath{M_{\oplus}}\xspace} 
\newcommand{\mJup}{M$_\mathrm{Jup}$\xspace}
\newcommand{\Sinc}{S$_\mathrm{inc}$\xspace}
% \newcommand{\Re}{\ensuremath{R_{\oplus}}\xspace} 
\newcommand{\kmax}{\RpRs$_{\mathrm{max}}$\xspace}

\newcommand{\corot}{\textit{CoRoT}\xspace} 
\newcommand{\kepler}{\textit{Kepler}\xspace} 
\newcommand{\ktwo}{\textit{K2}\xspace}
\newcommand{\spitzer}{\textit{Spitzer}\xspace}
\newcommand{\tess}{\textit{TESS}\xspace}
\newcommand{\gaia}{\textit{Gaia}\xspace} 
\newcommand{\jwst}{\textit{JWST}\xspace}
\newcommand{\cheops}{\textit{CHEOPS}\xspace}
\newcommand{\wise}{\textit{WISE}\xspace}
\newcommand{\poss}{\textit{POSS-1}\xspace}
\newcommand{\panstarrs}{\textit{PanSTARRS-1}\xspace}
%\newcommand{\gofal}{$\verb|GOF_AL|$\xspace}
\newcommand{\gofal}{\texttt{\mathrm{GOF_AL}}\xspace}
\newcommand{\maxrad}{\texttt{maxrad}\xspace}
\newcommand{\secthresh}{\texttt{secthresh}\xspace}
\newcommand{\dprec}{$\Delta_{\mathrm{prec}}$\xspace}

%path
\newcommand{\tablepath}{tables}

%paper-specific variables
\newcommand{\numstars}{68\xspace}
\newcommand{\numvp}{37\xspace}
\newcommand{\numvphost}{29\xspace}
\newcommand{\numpc}{28\xspace}
\newcommand{\numnewvp}{3\xspace}
\newcommand{\numoldpc}{34\xspace}
\newcommand{\numnewpc}{3\xspace}
\newcommand{\numfp}{8\xspace}
\newcommand{\nummulti}{6\xspace}

\newcommand{\nummulticamp}{48\xspace}

\newcommand{\numtargetswithspeckle}{29\xspace} %16 from WIYN/Livingston
\newcommand{\numtargetswithspecklecompanions}{7\xspace} %1 using WIYN/Liv data and rest comes from unpublished exofop
\newcommand{\numtargetswithoutfit}{12\xspace} %either undetected or low snr
%211336288, 211335816, 211826814, 212639319, 211305568, 212036875, 211731298, 211901114, 212470904, 211413752, 211797637, 212563850
\newcommand{\numtargetswithao}{6\xspace} %
\newcommand{\numtargetswithinaper}{24\xspace} % count from tab_gamma.tex
\newcommand{\numtargetswithspec}{58\xspace} %
\newcommand{\numtargetswithnewspec}{28\xspace} % from cochran alone 

\newcommand{\numprot}{42\xspace}
\newcommand{\minProt}{1.61\xspace}
\newcommand{\maxProt}{31.7\xspace}
\newcommand{\numprotwithplanets}{9\xspace}

\newcommand{\numstarsdave}{2\xspace}
%211843564, 212096658, 212428509, 212585579, 211988320

\newcommand{\numgaiabinary}{13\xspace}
\newcommand{\numAOGB}{8\xspace}
\newcommand{\numUSP}{5\xspace}
\newcommand{\numlongPorb}{2\xspace}

\newcommand{\fractionalenhancement}{X~\%\xspace}

\newcommand{\minP}{1.99\xspace}
\newcommand{\maxP}{52.71\xspace} %211611158.02	
%\newcommand{\maxP}{63.84\xspace}

\newcommand{\medianRp}{2.2~\rearth}
\newcommand{\meanRp}{2.35~\rearth}

\newcommand{\numstarswithinaperture}{16\xspace}
\newcommand{\numstarsruledout}{X\xspace}
\newcommand{\numstarspotentialNEBs}{9\xspace}

==> K2 in Cancri and Virginis arxiv/scratch.tex <==
\subsubsection{EPIC 211897691}
\begin{itemize}
    \item 2 planets with short and long periods but similar radius (~2 Rearth)
    \item low SNR and \vespa computed FPP=85\% for both candidates
    \item active star in 3 campaigns
\end{itemize}

\subsubsection{EPIC 212072539}
\begin{itemize}
    \item outer candidate by \citet{2018YuC16} and inner candidate by \citet{2019KruseC0to8}
    \item outer candidate is hi SNR but the outer is low and a bit V-shaped and hence \vespa computed FPP=95\%
    \item in 3 campaigns but C16 lc is bad
\end{itemize}

\subsubsection{EPIC 212555594}
\begin{itemize}
    \item CP accdg to exofop by \citet{2018MayoC1to10} but there is another candidate by \citet{2018PetiguraC5to8} but identical period
\end{itemize}

\subsubsection{Multi-planet system within the radius valley}
%\subsubsection{EPIC 211988320}
EPIC 211988320 has two planets straddling the radius valley \citep[1.5<\Rp<2.0;][]{2017FultonGap} with periods of 6.79 and 18.52 d.  %reminiscent of Davide's planets? 
The outer planet was detected by \cite{2019KruseC0to8} and \citet{2017DressingC1to7planets} while the inner planet is a new candidate validated in this work.
The other planet is actually larger than Rp>2Re

\begin{figure*}
    \includegraphics[clip,trim={0 0 0 0},width=1\textwidth]{fig_effect_of_parallax.png}
    \caption{Assessment of the impact of parallax on the stellar parameters used in this work. The red and blue points correspond to stars with (8 out of \numvp in our sample) and without high resolution optical or medium resolution NIR spectroscopic constraints, respectively (see \S\ref{sec:spec}). 
    The x/y-axes correspond to the value of each stellar parameter before/after incorporating parallaxes from Gaia DR2, and the dashed gray lines indicate the line y = x for reference. Without parallax information, two stars in our sample are confused as bright, faraway evolved giants when in fact they are faint, nearby dwarf stars.}
    \label{fig:parallax}
\end{figure*}

There are 14 muti-planetary system candidates in Cancri & Virginis constellations.
There are 54 nexsci PC with spec+imaging obs from exofop

@MISC{2016NewvilleLMFit,
  organisation = {{Newville}, M. and {Stensitzki}, T. and {Allen}, D.~B. and {Rawlik}, M. and 
	{Ingargiola}, A. and {Nelson}, A.},
    title = "{Lmfit: Non-Linear Least-Square Minimization and Curve-Fitting for Python}",
 keywords = {Software},
howpublished = {Astrophysics Source Code Library},
     year = 2016,
    month = jun,
archivePrefix = "ascl",
  eprint = {1606.014},
  adsurl = {http://adsabs.harvard.edu/abs/2016ascl.soft06014N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

\subsection{Host star properties}
planets in early type stars are rare
thin or thick disk origin?
The thin disc is vertically thin (Bovy et al. 2012; Haywood et al. 2013), rotation dominated (Edvardsson et al. 1993; Rix \& Bovy 2013), has a metallicity range of $-0.7 < \feh < +0.5$ dex (Bensby et al. 2014), and has ongoing star formation.  
The thick disc (Yoshii 1982; Gilmore \& Reid 1983) has larger vertical scale-heights but smaller radial scale-lengths than the thin disc (Bovy et al. 2012; Haywood et al. 2013; Hayden et al. 2015), and has rotation but also higher velocity dispersion (Haywood et al. 2013; Kordopatis et al. 2013b). It is also chemically different than the thin disc, having lower metallicities and higher [$\alpha$/Fe] (Edvardsson et al. 1993; Bensby et al. 2003; Kordopatis et al. 2013b; Nidever et al. 2014), pointing to a scenario where it is older than the thin disc.
Alpha elements (O, Mg, Si, S, Ca) are dispersed into the interstellar medium due to core-collapse supernova (SN II). However, [α/Fe] goes down with time as supernova Type Ia (SNe Ia) events start to happen that contribute more Fe. Stars with enhanced [α/Fe] are formed from gas that was enriched primarily by core-collapse supernovae. Therefore, [α/Fe] is indicative of a stellar populations’ star formation history, with stars having high [α/Fe] being older, on average

Recon Spectroscopy to identify astrophysical false positives and to contribute to improved stellar parameters for the host star in those cases where the uncertainty in the planetary mass and radius is limited by the  uncertainties in the mass and radius of the host star. Recon spectroscopy can identify eclipsing binaries that masquerade as transiting planets by revealing large velocity variations due to an orbiting stellar companion consistent with the photometric ephemeris from TESS. Blends of a target star with a nearby (usually fainter) eclipsing binary that is not spatially resolved can show composite spectra where the orbit of the contaminating eclipsing binary is consistent with the photometric ephemeris from TESS. These are but two examples of the false positives revealed by Recon Spectroscopy. Spectroscopic determinations of effective temperature, surface gravity, and metallicity can often contribute to improved estimates of the mass and radius of the host star, when analyzed with the help of stellar models or empirical relations

SED: We retrieved archival photometry for each target by cross-matching our sample against sources from the Howell-Everett (HE, Everett et al. 2012), Sloan Digitial Sky Survey (SDSS, Ahn et al. 2012), Two-Micron All-sky Survey (2MASS, Skrutskie et al. 2006), and Wide-field Infrared Survey Explorer (WISE, Cutri & et al. 2014) catalogues on Vizier using a 2' search cone  to construct SEDs, excluding targets which had fewer than five photometric data points.

\begin{figure*}
    \includegraphics[clip,trim={0 0 0 0},width=0.8\textwidth]{epic212297394_plots.pdf}
    \caption{Phase-folded plots of two planet candidates detected in EPIC 21227394 with \Porb of 2.29 d and 5.21 d.}
    \label{fig:lc}
\end{figure*}

\subsubsection{EPIC 211314705}
This target was observed in K2/C5 and we detected the signal in both \everest and \ktwosff light curves. \panstarrs images rule out potential nearby EB within the photometric aperture and our AO and speckle images further extend the constraint down to within a few arcseconds. We obtained an FPP<1\% using \vespa which rule out remaining false positive scenarios not constrained by our observations and hence the planet is validated.

\subsubsection{EPIC 211579112}
This target was observed in K2/C5 \& C18 and we detected the transits in both campaigns. \citet{2019KruseC0to8} detected the \Porb$=$17.7 d candidate using C5 light curve only and reported that the \Rp$=1.46\pm0.11$ candidate is near or within the habitable zone. \panstarrs show a faint nearby star which we ruled out as a potential nearby EB in \S \ref{sec:dilution}. Our AO and speckle contrast curves further extend the constraint down to within a few arcseconds. We obtained an FPP<1\% using \vespa which rule out remaining false positive scenarios not constrained by our observations and hence the planet is validated.

\subsubsection{EPIC 211763214}
This target was observed in K2/C5, C16, and C18 but we did not detect the \Porb$=$21.2 d candidate in the last campaign due to relatively high scattering in the light curve. Only light curve in C5 was previously analyzed by \citet{2019KruseC0to8} and \citet{2018MayoC1to10} so we added C16 data in this work. \citet{2018MayoC1to10} did not validate the candidate due to the lack of AO imaging data despite the reported very low FPP$=$0.5\%. Our AO and speckle images show no companions which enable us to finally validate the planet.

We also cross-matched the host star with the TIC-Gaia catalog \citet{2020CarilloTGv8} which provide a 95\% probability for the star to be in the thin-disc similar to the majority of known host stars.

\subsubsection{EPIC 211965883}
This target was previously analyzed by \citet{2017DressingC1to7planets} who reported the candidate with \Porb$=$10.55422 d 
%\Rp$=$2.86$\pm$0.28 \rearth using \rstar$=$0.60$\pm$0.03 \rsun 
but did not validate it due to the large FPP$=$34\%.
%\citet{2019KruseC0to8} derived a smaller radius, \Rp=1.33$^{+0.13}_{-0.29}$ \Rearth, as a result of larger but imprecise adopted stellar radius, $\Rstar=0.66$ from \gaia DR2.
We found no contaminating stars within the photometric aperture as well as close to the target using our AO and speckle images. We recomputed the FPP using these constraints which resulted to FPP<1\% and hence the planet is validated.

\subsubsection{EPIC 212088059}
This target was observed in K2/C5, C16, \& C18 and we detected the \Porb$=$10.4 d candidate in both \everest and \ktwosff light curves. \panstarrs images show a faint source within the aperture but our analysis in \S \ref{sec:dilution} rule out the nearby source as potential nearby EB. Also, our AO and speckle contrast curves further extend the constraint down to within a few arcseconds. We obtained an FPP<1\% using \vespa which rule out remaining false positive scenarios not constrained by our observations and hence the planet is validated.

\subsubsection{EPIC 212132195}
This target was observed in K2/C5 \& C16 but we detected the \Porb$=$26.2 d candidate marginally in C5, due to higher scatter in the second half of the campaign. The candidate was previously analyzed by \citet{2018MayoC1to10} using only the C5 data and did not validate it due to the lack of AO/speckle data which we provide in this work coupled with the C16 light curve. Archival POSS1 images help rule out background EBs. We recomputed FPP using \vespa and yielded FPP<1\% and hence the planet is validated. We also note that the star has a 69\% thin disc probability based on the TIC-Gaia catalog \citet{2020CarilloTGv8}.

\subsubsection{EPIC 212161956}
We detected the candidate with \Porb=7.2 d in both in K2/C5 \& 18 light curves. \panstarrs image shows two faint stars near the edge of the photometric aperture. As discussed in \S \ref{sec:dilution}, multi-aperture analysis rules out the nearby stars as potential sources of the signal. Our contrast curve extends the constraint down to within a few arcseconds. We obtained an FPP<1\% using \vespa which rule out remaining false positive scenarios not constrained by our observations and hence the planet is validated.

\subsubsection{EPIC 212278644}
This target was observed in K2/C6 and we detected the \Porb$=$12.4 d candidate in both \everest and \ktwosff light curves. \panstarrs image show a faint star within the photometric aperture which we ruled out as a potential nearby EB in \S \ref{sec:dilution}. We obtained an FPP<1\% using \vespa which rule out remaining false positive scenarios not constrained by our observations and hence the planet is validated.

\subsubsection{EPIC 212330265}
This target was observed in K2/C6 and we detected the candidate with \Porb$=$4.2 d recently reported by \citet{2019KruseC0to8}. \panstarrs images show no nearby, contaminating stars within the photometric aperture and archival POSS1 images help rule out potential background EBs. We recomputed the FPP using these constraints which resulted to FPP<1\% and hence the planet is validated.

\subsubsection{EPIC 212398508}
This target was observed in K2/C6 and we detected the \Porb$=$46.4 d candidate reported recently by \citet{2019KruseC0to8}. \gaia indicates a nearby star which is not bright enough to reproduce the signal. \panstarrs images show no other nearby, contaminating stars within the photometric aperture and archival POSS1 images help rule out potential background EBs. We recomputed the FPP using these constraints which resulted to FPP<1\% and hence the planet is validated.

\subsubsection{EPIC 212495601}
This target was observed in K2/C6 \& C17 and but we did not detect the \Porb=21.7 d candidate in C17 data due to noisy light curves. \panstarrs images show no nearby, contaminating stars within the photometric aperture and our contrast curves further extend the constraint down to within a few arcseconds. We obtained an FPP<1\% using \vespa which rule out remaining false positive scenarios not constrained by our observations and hence the planet is validated.

\subsubsection{EPIC 212543933}
This target was observed in K2/C6 and we detected the \Porb$=$21.7 d candidate in both \everest and \ktwosff light curves. \panstarrs images rule out potential nearby EB within the photometric aperture. We reran \vespa using our speckle contrast curve and obtained an FPP<1\% and hence the planet is validated.

\subsubsection{EPIC 212420823}
This target was observed in K2/C6 and we detected the \Porb=9 d candidate in both \everest and \ktwosff light curves. \panstarrs images rule out potential nearby EB within the photometric aperture and our contrast curve further extends the constraint down to within a few arcseconds. We obtained an FPP<1\% using \vespa which rule out remaining false positive scenarios not constrained by our observations and hence the planet is validated.

\subsection{Multi-planet systems}

\subsubsection{EPIC 212297394}
This target was observed in K2/C6 and we detected two planet candidates with \Porb=2.29 and 5.21 d. Both candidates were previously detected by \citet{2019KruseC0to8} but only the inner planet has so far been validated \citet{2019HellerTLS2} (Not clear why). \panstarrs image and our contrast curve further rules out nearby EBs. We obtained an FPP<1\% and hence the outer planet is validated.

\subsubsection{EPIC 212440430}
This target was observed in C6 \& C17 and we detected two planets with \Porb 4.16 d and 20.0 d (approximately in 5:1 \Porb resonance) in both in C6 and C17 light curves but only marginally in C17 due to higher scatter in the second half of the campaign. The outer planet was previously detected by \citet{2019KruseC0to8} using C5 light curve while the inner planet is a new detection. \panstarrs image and our contrast curve rules out potential nearby EBs. %Owing to multiplicity boost (CITE), these evidences significantly lowers their FPP (see Table \ref{tab:planet}). %Pope only reported one candidate while Cruz reported both candidates and and Heller validated the inner (2-day) planet.  
%https://arxiv.org/pdf/1905.09038.pdf

\section{Planet Validation}
%NEB (Nearby Eclipsing Binary): Indicates that the TESS detection was caused by a nearby eclipsing binary contaminating the TESS aperture, as determined from follow-up photometry that resolved the nearby eclipsing binary. BEB (Blended Eclipsing Binary): Indicates that an eclipsing binary blended in the follow-up and TESS apertures caused the TESS detection. These systems are generally classified as BEB as a result of a chromatic transit depth in follow-up photometry.  EB (Eclipsing Binary): Indicates that the TESS detection is caused by an event on target, but the event is too deep to be caused by an orbiting planet. 

\begin{comment}
\begin{figure*}
    \subfloat[EPIC-211314705b]{\includegraphics[clip,trim={4.5cm 1.75cm 4.5cm 0},width=0.3\textwidth]{epic211314705_4x4-eps-converted-to.pdf}}
    \hfill
    \subfloat[EPIC-211579112b]{\includegraphics[clip,trim={4.5cm 1.75cm 4.5cm 0},width=0.3\textwidth]{epic211579112_4x4-eps-converted-to.pdf}}
    \hfill
    \subfloat[EPIC-211763214b]{\includegraphics[clip,trim={4.5cm 1.75cm 4.5cm 0},width=0.3\textwidth]{epic211763214_4x4-eps-converted-to.pdf}}
    \hfill
    \subfloat[EPIC-211965883b]{\includegraphics[clip,trim={4.5cm 1.75cm 4.5cm 0},width=0.3\textwidth]{epic211965883_4x4-eps-converted-to.pdf}}
    \hfill
    \subfloat[EPIC-212088059b]{\includegraphics[clip,trim={4.5cm 1.75cm 4.5cm 0},width=0.3\textwidth]{epic212088059_4x4-eps-converted-to.pdf}}
    \hfill
    \subfloat[EPIC-212132195b]{\includegraphics[clip,trim={4.5cm 1.75cm 4.5cm 0},width=0.3\textwidth]{epic212132195_4x4-eps-converted-to.pdf}}
    \hfill
\includegraphics[clip,trim={0 0 0 0},width=0.49\textwidth]{fig_cc.png}
\caption{Subaru/IRCS images of the host stars. \textcolor{red}{Combine cc with inset AO images.}}
\label{fig:ao}
\end{figure*}

\begin{figure}
    \includegraphics[clip,trim={0 0 0 0},width=0.49\textwidth]{fig_cc_plot.png}
    \caption{5-$\sigma$ contrast curves extracted from the reduced Subaru/IRCS images in Figure \ref{fig:ao}.}
    \label{fig:cc}
    \end{figure}
\end{comment}

\subsection{M-R relation}
%Assuming that the M-R relation can be described as a power law with a dispersion that is constant and normally distributed, we find that M/M⊕ = 2.7(R/R⊕)^1.3, a scatter in mass of 1.9M⊕, and a mass constraint to physically plausible densities, is the "best-fit" probabilistic M-R relation for the sample of RV-measured transiting sub-Neptunes (Rpl < 4 R⊕).

We estimate the masses of each of the candidate planet based on their precise radii using the M-R relation \citep{2016WolfgangMRrelation}), applicable for transiting sub-Neptunes ($R_p$ < 4 \rearth) and assuming that the M-R relation can be described as a power law with a dispersion that is constant and normally distributed.

\textcolor{red}{See newer references for Mass-Radius relation for small planets: \citep[e.g.,][]{2018VanEylenRadiusValley,2017FultonGap}.}

\subsection{Interesting systems/Characterization targets}
% \item expanded vespa description/discussion
% \item add figure showing transits of multi-planet systems
% \item small/large aperture comparison
% \item archival imaging (if high proper motion)
% \item run vespa with phase-folded lightcurves from K2SFF
% \item compute mass upper limits (if any)
% \item decide on validated planets w/o imaging

%USP?

%\subsection{Mass characterization via precision RV}
% Our validated planet sample includes 18 planets smaller than 2R , several of which orbit bright host stars (J ≈ 7–9). These small planets thus present opportunities for detailed studies of terrestrial worlds via either RV measurements or transmission spectroscopy. 

Using the empirical mass-radius relation for small planets < 14.26\rearth from \citet{2017ChenKippingMRrelation}, we compute the maximum likelihood masses $m_p$
of our planet candidates and single transit events to then infer their expected RV semi-amplitudes using
\begin{equation}
    K_{RV}=2.4\ms \Big(\frac{m_p}{5M_{\oplus}}\Big) \Big(\frac{M_s}{0.5M_{\odot}}\Big)^{-2/3} \Big(\frac{P}{10 d}\Big)^{-1/3} 
\end{equation}

These values are shown in the first panel of Figure~\ref{fig:K} verson the V magnitude superposed with the set of confirmed transiting planets from the NASA Exoplanet Archive. Many existing high performance RV spectrographs are stable at the level of a few cm/s but RV observations are often limited by photon noise and intrinsic stellar activity at the level of 1 to a few m/s, even for relatively inactive stars (Fischer et al. 2016). The majority of our targets have expected $K_{RV}$ values in excess of this typical RV sensitivity limit and are reported in Table X.%~\ref{tab:planet}.


\begin{figure}
    \includegraphics[width=0.49\textwidth]{fig_MR.png}
    \caption{Mass estimates based on the Mass-Radius relation of \citet{2016WolfgangMRrelation}. The various curves denote the densities from H to Fe. %The majority of the validated planets reside within the Fulton gap denoted by black vertical lines.
    }
    \label{fig:MR}
\end{figure}

\begin{figure}
    \includegraphics[width=0.49\textwidth]{fig_RV_mag.png}
    \caption{\textcolor{red}{RV semi-amplitude as a function of \kepler magnitude. Our brightest targets have amplitudes <8 m/s  detectable with current generation spectrographs.}}
    \label{fig:K}
\end{figure}

\begin{figure}
    \includegraphics[width=0.49\textwidth]{fig_MR_comparison.png}
    \caption{Mass estimate comparison between \citet{2016WolfgangMRrelation} and \citet{2014Weiss&Marcy}.}
    \label{fig:MR_comparison}
\end{figure}

\subsubsection{Multi-aperture light curve analysis}
There have been six validated planets shown to be false positives by follow-up observations and analysis \citep{2017Cabrera3FP,2017Shporer3FP}. We briefly examine whether these instances are a cause for concern in our own results.

In the case of \citet{2017Cabrera3FP}, they found that two false positives exhibited increased transit depths for larger aperture masks (suggesting a nearby star was responsible for the eclipses) while the third showed a secondary eclipse at phase = 0.62 when they used a different data reduction process. The first two false positives would have failed the multi-aperture size test %variable-sized mask test 
we apply via our diagnostic plots, while the secondary eclipse from the third false positive would have been caught through a combination of our data reduction process and the "model-shift uniqueness" test we apply \citep{2016CoughlinModelShiftTest}.

As for \citet{2017Shporer3FP}, the vespa fit to the available photometry for each false positive was very poor and all three of the false positives were reported to be very large "planets." We addressed these concerns in two ways. First, we decided to only use 2MASS photometry in order to avoid systematic errors between photometric bands. Second, we chose not to validate any planet candidates larger than 8 $R\oplus$, since a candidate of that size or larger could actually be a small M dwarf. The only exception to this rule is if there are RV measurements that can rule out the eclipsing binary scenario, in which case we do report the FPP (and validate for FPP < 0.001) regardless of planet size.

\begin{itemize}
\item Our transit analyses (without density priors) yield mean stellar densities ($\rho_{*,LC}$) within 1$\sigma$ of the values from our independent assessment (\S X).
\item vespa FPP
\item gaia
\item AO imaging
\item using contrast curves and isochrones inputs listed in Table X, we find an FPP of X
\item From the observed transit depth, an EB with 100\% eclipse depths that is less than X mag fainter than the primary could reproduce the observed transit depth
\end{itemize}
% 1. There is not a composite spectrum.
% 2. There is not a companion in the aperture. (This was determined from archival imaging.)
% 3. There is not a companion in AO and/or speckle images. (This was determined from our AO and speckle images as well as any images for our candidates uploaded to https://exofop.ipac.caltech.edu/k2/ before 2017 August 9.)
% 4. There is no evidence of a secondary eclipse (at any arbitrary phase).
% 5. There is not an ephemeris match (see Section 2.4). If any of the above were false, the FPP was not re-
% ported in Table 4 and the candidate was not validated regardless of the FPP value vespa provided.

\subsubsection{NOT/FIES}
We also used the FIbre-fed Ec\'helle Spectrograph \citep[FIES;][]{1999FrandsenLindbergFIES,2014TeltingFIES} on the 2.56-m Nordic Optical Telescope (NOT) of Roque de los Muchachos Observatory in La Palma, Spain to collect high-resolution ($R\approx$67,000) spectra for X campaign X candidates (EPIC-XXXXXXXX, EPIC-XXXXXXXX, etc.). The observations were carried out between X to X UTC, within observing programs XXX and XXX. We followed the same strategy as in \citet{2013GandolfiKepler77} and traced the RV drift of the instrument by bracketing the science exposures with 90-sec ThAr spectra. We reduced the data using standard IRAF routines and extracted the RVs via multi-order cross-correlations using different RV standard stars observed with the same instrument.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The NASA {\it K2} mission \citep{2014HowellK2} has extended the legacy of {\it Kepler} by monitoring stars a series of $\sim$100 deg$^2$ fields along the ecliptic plane for $\sim$80 days each. {\it K2} has so far discovered $\sim$300 statistically validated or confirmed exoplanets exhibiting a broad diversity of properties and system architectures \citep[e.g.][]{2016CrossfieldC1to5,2018MayoC1to10}. The wider sky coverage of {\it K2} (compared to {\it Kepler}) has enabled discoveries of planets in a variety of stellar environments, including the first transiting multi-planet system in a cluster \citep{2018ALivingstonHyades}, as well as a planet orbiting a 5--10 Myr star \citep{2016DavidK2-33}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Using the mass-radius relation of \citet{2017ChenKippingMRrelation}, we estimate a mass of $\sim$4\,$M_{\rm{Jup}}$, with large uncertainties. However, because of the possibility that this planet is an inflated hot Jupiter, we consider the possibility that the planet has a mass as low as $\sim$1$\,M_\mathrm{Jup}$. Using Table 5 of \citet{2013ApJS..208....9P}\footnote{The updated version of the table is available at \url{http://www.pas.rochester.edu/~emamajek/EEM_dwarf_UBVIJHK_colors_Teff.txt}} along with the Gaia DR2 values of $\teff$ and $R_\star$ (see Table~\ref{tab:star}), the spectral type and mass of the host star are K6V and 0.68\,$M_\odot$, respectively. The host star mass, measured orbital period, and predicted planet mass result in an expected radial velocity semi-amplitude of $\sim$200--800 m\,s$^{-1}$. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{EPIC-211314705b}
Kepmag = 14.422.
V-Ks color: $M2.5\pm0.2$.
% Has TRES spectrum on ExoFOP (bieryla).
Has Subaru/IRCS AO.
% P = 3.79 d.
Has WIYN/NESSI, TRES


\subsubsection{EPIC-211579112b}
Kepmag = 15.768.
J-H color: $M3.9\pm1.2$.
% No spectra on ExoFOP.
Has Subaru/IRCS AO.
Has WIYN/NESSI
% P = 17.7 d.

\subsubsection{EPIC-211763214b}
Kepmag = 12.529.
V-Ks color: $K3.0\pm2.8$.
% Has TRES spectrum on ExoFOP (bieryla).
Has Subaru/IRCS AO.
Has WIYN/NESSI, TRES
% Predicted mass = $2.34^{+2.11}_{-1.00}$ Mearth.
% Predicted K = $0.58^{+0.52}_{-0.25}$ m/s.
% P = 21.197 d.

\subsubsection{EPIC-211965883b}
Kepmag = 14.138.
V-Ks color: $K6.4\pm0.2$.
Has TSPEC spectrum on ExoFOP (Dressing)
% Dressing+17: $M0V$ (not consistent with Huber).
Has Subaru/IRCS AO.
Has WIYN/NESSI
% Predicted mass = $6.47^{+5.09}_{-2.77}$ Mearth.
% Predicted K = $2.45^{+1.88}_{-1.04}$ m/s.
% P = 10.56 d.
\teff=4211 80,79;
\rstar=0.600 0.027,0.027;
\mstar=0.674 0.014,0.012 according to Table 4 of \citet[]{2017ApJ...836..167D}.
%see https://docs.google.com/spreadsheets/d/1Giwxhjnc7kq1K1-IfWDI1DZpVcCfyzZgHBgs_VHn-3w/edit#gid=0

\subsubsection{EPIC-212088059b}
Kepmag = 14.757.
V-Ks color: $M1.6\pm0.3$.
% No spectra on ExoFOP.
Has Subaru/IRCS AO.
Has WIYN/NESSI
% P = 10.37 d.

\subsubsection{EPIC-212132195b}
Kepmag = 11.670.
V-Ks color: $K3.4\pm0.1$.
Has SpeX spectrum on ExoFOP (Dressing).
% Dressing+17: $K3V$.
Has Subaru/IRCS AO.
Has WIYN/NESSI, TRES
% Predicted mass = $5.59^{+4.20}_{-2.33}$ Mearth.
% Predicted K = $1.50^{+1.14}_{-0.61}$ m/s.
% P = 26.195 d.

\subsubsection{EPIC-212161956b}
Kepmag = 14.778.
% No spectra on ExoFOP.
V-Ks color: $K5.2\pm0.2$.
Has WIYN/NESSI
% Predicted mass = $4.94^{+3.71}_{-1.94}$ Mearth.
% Predicted K = $2.29^{+1.69}_{-0.91}$ m/s.
% P = 7.19 d.

\subsubsection{EPIC-212278644b}
Kepmag = 13.949.
V-Ks color: $G5.1\pm1.1$.
% No spectra on ExoFOP.
Has WIYN/NESSI
% Predicted mass = $6.34^{+4.99}_{-2.72}$ Mearth.
% Predicted K = $1.81^{+1.43}_{-0.76}$ m/s.
% P = 12.43 d.
Has recon spec at McDonald 2.7m (B. Cochran)

\subsubsection{EPIC-212297394b}
Kepmag = 14.138.
V-Ks color: $K2.3\pm0.2$.
% No spectra on ExoFOP.
Has WIYN/DSSI on ExoFOP (Everett)
Has FIES
% Possible multi -- see ESPRINT spreadsheet.
% Predicted mass = $5.59^{+4.20}_{-2.26}$ Mearth.
% Predicted K = $2.35^{+1.77}_{-0.98}$ m/s.
% P = 5.21 d.

\subsubsection{EPIC-212330265b}
Kepmag = 14.949.
J-H color: $K5.1\pm2.4$.
% No spectra on ExoFOP.
Has WIYN/NESSI
% Predicted K = 1.3 m/s.
% P = 4.174 d.

\subsubsection{EPIC-212398508b}
Kepmag = 13.629.
V-Ks color: $K4.0\pm3.4$.
% No spectra on ExoFOP.
Has WIYN/NESSI
% Predicted mass = $6.47^{+5.09}_{-2.70}$ Mearth.
% Predicted K = $1.29^{+1.01}_{-0.54}$ m/s.
% P = 46.42 d.
Has recon spec at McDonald 2.7m (B. Cochran)

\subsubsection{EPIC-212420823b}
%ask 
Kepmag = 14.166.
V-Ks color: $K2.1\pm0.3$.
% No spectra on ExoFOP.
Has WIYN/NESSI
Has FIES
% Predicted mass = $5.48^{+4.11}_{-2.28}$ Mearth.
% Predicted K = $1.91^{+1.43}_{-0.79}$ m/s.
% P = 9.03 d.
% TTVs?

\subsubsection{EPIC-212440430b}
Kepmag = 13.267.
V-Ks color: $G6.0\pm0.9$.
% No spectra on ExoFOP.
Has WIYN/DSSI on ExoFOP (Everett)
% Predicted mass = $8.47^{+6.36}_{-3.73}$ Mearth.
% Predicted K = $2.04^{+1.61}_{-0.90}$ m/s.
% P = 19.99 d.
% Possible multi -- see ESPRINT spreadsheet.
% KEST note: $McDonald: Teff=5780+/-49 K, [Fe/H]=-0.02+/-0.03 dex, logg=4.44+/-0.12 (cgs), vsini=3.31+/-0.29 km/s, RV=-22.275+/-0.064 km/s$
Has recon spec at McDonald 2.7m (B. Cochran)

%\subsubsection{EPIC-212480208b}
%Kepmag = 10.892.
%V-Ks color: $G6.3\pm2.1$.
%Has TRES spectrum on ExoFOP (Bieryla).
%Has WIYN/DSSI on ExoFOP (Everett).
%Has WIYN/NESSI
% Predicted mass = $0.10^{+0.10}_{-0.05}$ Mearth.
% Predicted K = $0.03^{+0.03}_{-0.02}$ m/s.
% P = 10.09 d.
% KEST note: $RV=-12.731 +/- 1.453 km/s (RAVE survey). Mc Donald Mar16: Teff=5640+/-51 K, logg= 4.31+/-0.06 (cgs), [Fe/H]=-0.27+/-0.02 dex, vsini=3.15+/-0.32, RV=-10.55+/-0.24$ km/s (see PICK2\_201603.txt). Prot=30 days? Super cool object but super tough case!
%Has recon spec at McDonald 2.7m (B. Cochran)

\subsubsection{EPIC-212495601b}
Kepmag = 13.821.
V-Ks color: $G5.2\pm1.1$.
% No spectra on ExoFOP.
Has WIYN/NESSI
% Predicted mass = $5.26^{+4.14}_{-2.13}$ Mearth.
% Predicted K = $1.40^{+1.08}_{-0.57}$ m/s.
% P = 21.67 d.
Has recon spec at McDonald 2.7m (B. Cochran)

% \subsubsection{EPIC-212496592b}
% Kepmag = 12.966.
% V-Ks color: $K2.1\pm0.1$.
% Has TRES spectrum on ExoFOP (Bieryla).
% Has WIYN/DSSI on ExoFOP (Everett)
% Predicted mass = $2.65^{+2.19}_{-1.07}$ Mearth.
% Predicted K = $1.33^{+1.14}_{-0.55}$ m/s.
% P = 2.86 d.
% KEST note: $Mc Donald (Mar 2016): Teff = 5180+/-73 K, logg = 4.44+/-0.12 (cgs), [Fe/H] = -0.04+/-0.03 dex, vsini=1.85+/-0.22, RV= -9.02+/-0.16 km/s$ (see PICK2\_201603.txt).

\subsubsection{EPIC-212543933b}
Kepmag = 14.010.
V-Ks color: $G5.0\pm1.5$.
No spectra on ExoFOP.
Has WIYN/DSSI on ExoFOP (everett).
Predicted mass = $6.21^{+4.89}_{-2.66}$ Mearth.
Predicted K = $2.11^{+1.72}_{-0.88}$ m/s.
P = 7.8 d.
Bill Cochran got recon spec at McDonald 2.7m during May run.

\subsubsection{EPIC-212563850b}
Kepmag = 13.172.
V-Ks color: $K6.6\pm0.2$.
% No spectra on ExoFOP.
Has WIYN/NESSI
% Predicted mass = $1.13^{+0.85}_{-0.44}$ Mearth.
% Predicted K = $0.51^{+0.41}_{-0.20}$ m/s.
% P = 14.3 d.
Has recon spec at McDonald 2.7m (B. Cochran)

% \subsubsection{EPIC-212572439b}
% Kepmag = 12.835.
% V-Ks color: $K1.2\pm0.5$.
% Has TRES spectrum on ExoFOP (bieryla).
% Has TSPEC spectrum on ExoFOP (dressing), classified as K2V.
% Has SpeX spectrum on ExoFOP (dressing), classified as K2V.
% Has WIYN/DSSI on ExoFOP (everett).
% Has Gemini/DSSI on ExoFOP (everett).
% Predicted mass = $27.63^{+23.85}_{-12.80}$ Mearth.
% Predicted K = $15.01^{+13.13}_{-6.98}$ m/s.
% P = 2.58 d.
% Possible false positive based on DAVE pipeline (http://keplertcert.seti.org/DAVE/). Significant centroid offset measured. See the full report at: http://keplertcert.seti.org/DAVE/AllK2/Output/212572439/
% Possible false positive = Yes (Suspect contamination from EPIC 212351048.)

%-----------------------ADDITIONAL c16-------------------
\subsubsection{212178066}
% saturated based on Yu+16; https://arxiv.org/pdf/1803.04091.pdf
Bill Cochran got recon spec at McDonald 2.7m
has FASTcam Lucky imaging

\subsubsection{251319382}
3-planet system.
Bill Cochran got recon spec at McDonald 2.7m
TRES extracted spectra on ExoFOP (bieryla)
has FASTcam Lucky imaging

\subsubsection{211502222}
3-planet system.
Bill Cochran got recon spec at McDonald 2.7m
TRES extracted spectra on ExoFOP (bieryla)
has FASTcam Lucky imaging

\subsubsection{212048748}
bright M-dwarf.
Bill Cochran got recon spec at McDonald 2.7m
Has Subaru/IRCS AO.

\subsubsection{212081533}
Bill Cochran got recon spec at McDonald 2.7m
Has Subaru/IRCS AO.

% \subsubsection{EPIC-211446060b}
% Very nice candidate! M67 cluster member! Short transit duration suggests a dwarf host, maybe a warm Jupiter if the star is a dwarf. 

% \subsubsection{EPIC-212737443b}
% Kepmag = 14.461.
% J-H color: $M4.3\pm1.9$.
% Has TSPEC spectrum on ExoFOP (dressing), classified as K3V.
% Observing with WIYN/NESSI this semester.
% Predicted mass = $5.26^{+3.76}_{-2.13}$ Mearth.
% Predicted K = $1.95^{+1.44}_{-0.78}$ m/s.
% P = 13.6 d.

%Davide for FIES
%WIYN/NESSI: Livingston (or Howell/Everett)
%WIYN/DSSI: Howell/Everett (usually)
%McDonald: B. Cochran/ M. Endl


\begin{figure*}
    \includegraphics[width=1\textwidth]{fig_with-without-rhostar-prior.png}
\caption{Difference of resulting MCMC best-fit transit parameters with and without stellar density prior for each star (denoted by its last 4 EPIC numbers).}
\label{fig:rhostar-prior}
\end{figure*}



==> K2 in Cancri and Virginis arxiv/tables/tab_Prot.tex <==
%from Savita: We have 36 stars with reliable results, 3 stars where Prot is ~twice the orbital period of the  PL and 3 stars with a “maybe” period. 
\begin{tabular}{llll}
\hline
EPIC		&	\Prot & $S_{ph}$ & Note  \\	
\hline
211314705 &  $10.39\pm0.81$ &    $2135.89\pm122.63$ &        \\ %FP
211342524 &  $12.19\pm1.06$ &    $ 1681.88\pm74.84$ &        \\ %PC
211357309 &  $16.41\pm1.25$ &    $ 1067.07\pm47.57$ &      T \\ %PC
211399359 &  $17.23\pm1.67$ &    $3817.92\pm171.21$ &       \\ %PC
211413752 &  $24.87\pm2.64$ &    $  898.20\pm33.88$ &      VP \\ %VP-3 or 5 planets
211502222 &   $9.98\pm0.71$ &    $  208.41\pm11.87$ &      VP \\ %VP, Porb=9.4 & 23
211578235 &  $14.69\pm1.13$ &    $4648.31\pm206.41$ &        \\ %PC, LR Porb=11
211579112 &  $31.71\pm3.60$ &    $4445.99\pm265.41$ &        \\ %FP, 17.7
211611158 &  $17.35\pm2.87$ &    $  903.46\pm43.65$ &      VP \\ %VP, Porb=10 & 52.7
211645912 &  $10.83\pm0.86$ &    $6021.45\pm267.27$ &        \\ %PC, Porb=10.6
211731298 &  $11.85\pm0.99$ &    $4979.20\pm239.15$ &       VP \\ %VP, Porb=7.44
211741619 &   $9.39\pm0.89$ &    $ 1594.10\pm91.51$ &        \\
211762841 &  $13.15\pm1.28$ &    $2954.98\pm131.30$ &        \\
211796070 &  $21.66\pm2.59$ &    $  540.95\pm24.24$ &        \\
211799258 &  $26.48\pm3.62$ &    $7293.34\pm323.67$ &        \\
211800191 &   $2.19\pm0.13$ &    $  233.98\pm20.68$ &    \\
211843564 &  $18.47\pm1.49$ &    $3910.77\pm173.68$ &        \\
211886472 &  $19.79\pm1.44$ &    $  301.09\pm12.22$ &        \\
211897691 &  $11.13\pm0.83$ &    $5909.71\pm239.18$ &        \\
211965883 &  $10.61\pm0.82$ &    $3341.08\pm191.71$ &        \\
211987231 &   $7.30\pm0.54$ &    $1754.43\pm100.89$ &        \\
211988320 &  $24.53\pm1.64$ &    $  961.51\pm55.35$ &      VP  \\ %VP,Porb=36.4
211997641 &   $3.43\pm0.24$ &    $5469.70\pm387.92$ &    \\
212041476 &  $27.61\pm3.25$ &    $  992.11\pm55.44$ &      VP \\ %VP,Porb=2.78
212066407 &   $1.61\pm0.12$ &    $  129.69\pm13.58$ &    \\
212088059 &  $18.47\pm1.60$ &    $5285.10\pm188.854$ &      VP \\ %VP,Porb=10.36
212096658 &  $30.24\pm3.26$ &    $  625.50\pm22.11$ &        \\ %FP, EB
212138198 &  $16.99\pm2.04$ &    $ 1146.94\pm51.11$ & T \\
212315941 &  $12.70\pm0.97$ &    $ 1733.76\pm96.92$ &        \\
212330265 &  $16.76\pm1.75$ &    $5356.76\pm656.14$ &        \\
212428509 &   $5.34\pm0.36$ &    $  335.27\pm18.84$ &        \\ %FP, EB
212440430 &   $8.22\pm0.47$ &    $  554.50\pm25.42$ &      \\ %VP, Porb=4.2 & 20
212543933 &  $25.23\pm1.82$ &    $  351.01\pm19.85$ &    VP \\ %VP, Porb=7.8
212570977 &  $12.70\pm1.16$ &    $6097.36\pm250.89$ &       \\ %PC, Porb=8.9
212586030 &  $16.61\pm1.46$ &    $  365.39\pm15.24$ &        \\
212628098 &   $4.02\pm0.28$ &  $20639.54\pm1369.17$ &        \\
212703473 &  $20.49\pm1.78$ &      $958.19\pm53.76$ &        \\
212773272 &   $5.27\pm0.41$ &   $12122.11\pm675.84$ &        \\
212797028 &  $25.05\pm2.77$ &    $ 2010.69\pm82.87$ &    T   \\
251288417 &  $30.84\pm3.52$ &   $14425.97\pm802.14$ &        \\
251319382 &  $17.59\pm1.14$ &    $  485.29\pm27.24$ &   VP \\ %VP: Porb=3.7, 8.2 & 14.9 
\hline
\end{tabular}

==> K2 in Cancri and Virginis arxiv/tables/tab_ao.tex <==

211941472

Separation (arcsec) = 0.203
Position angle (degr. N through E) = 117.346
Magnitude difference = 0.37

832nm
------
Separation (arcsec) = 0.203
Position angle (degr. N through E) = 116.595
Magnitude difference = 0.32

211886472
Filter (nm) = 692
Separation (arcsec) = 0.323
Position angle (degr.) = 278.867
Mag. difference = 4.015

Filter (nm) = 880
Separation (arcsec) = 0.326
Position angle (degr.) = 279.746
Mag. difference = 3.767


==> K2 in Cancri and Virginis arxiv/tables/tab_campaign.tex <==
%https://keplerscience.arc.nasa.gov/k2-fields.html
\begin{tabular}{ccccc}
    \hline
    Campaign & Start & End & RA & Dec. \\
    \hline
    Cancer	& & & & \\
    5	& 2015 Apr 27 &	2015 Jul 10 & 08:40:38	& 16:49:47 \\
    16  & 2017 Dec 07 &	2018 Feb 25	& 08:54:50	& 18:31:31	\\
    18	& 2018 May 12 &	2018 Jul 02	& 08:40:39	& 16:49:40 \\
    Virgo	& & & & \\
    6	& 2015 Jul 14 & 2015 Sep 30	& 13:39:28	& -11:17:43	\\
    17  & 2018 Mar 01 &	2018 May 08	& 13:30:12	& -07:43:16	\\
    \hline
\end{tabular}

==> K2 in Cancri and Virginis arxiv/tables/tab_fpp.tex <==
\begin{tabular}{lrrrrrrrr}
\hline
ID &  $\mathrm{L_{beb}}^{a}$ &  $\mathrm{L_{beb}Px2}^{a}$ &  $\mathrm{L_{eb}}^{b}$ &  $\mathrm{L_{eb}Px2}^{b}$ &  $\mathrm{L_{heb}}^{c}$ &  $\mathrm{L_{heb}Px2}^{c}$ &  $\mathrm{L_{pl}}^{d}$ &      FPP \\
\hline
211314705.01 &     0.00e+00 &         0.00e+00 &    2.80e-05 &        1.31e-06 &     2.45e-06 &         3.75e-07 &    7.26e-03 & 4.41e-03 \\
211357309.01 &     6.77e-04 &         3.47e-04 &    0.00e+00 &        0.00e+00 &     0.00e+00 &         0.00e+00 &    2.10e-02 & 4.65e-02 \\
211383821.01 &     3.74e-04 &         1.13e-03 &    4.41e-04 &        1.89e-04 &     7.57e-18 &         3.85e-05 &    6.89e-02 & 3.06e-02 \\
211399359.01 &     0.00e+00 &         0.00e+00 &    2.58e-17 &        8.80e-15 &     1.05e-96 &         6.95e-47 &    4.45e-02 & 1.99e-13 \\
211401787.01 &     4.08e-07 &        2.78e-131 &    1.40e-06 &        2.31e-17 &     2.15e-07 &         9.35e-11 &    9.88e-03 & 2.04e-04 \\
211413752.03 &     7.72e-08 &         4.13e-15 &    1.51e-05 &        2.92e-07 &     2.26e-13 &         5.41e-19 &    5.12e-03 & 3.01e-03 \\
211413752.04 &     3.60e-05 &         2.84e-06 &    8.14e-04 &        5.88e-05 &     7.47e-06 &         3.39e-06 &    1.87e-02 & 4.69e-02 \\
211413752.05 &     9.13e-07 &         6.85e-14 &    8.74e-08 &        1.46e-08 &     4.86e-07 &         1.43e-09 &    3.44e-03 & 4.37e-04 \\
211439059.01 &     1.55e-06 &         1.74e-19 &    3.50e-06 &        1.67e-07 &     2.87e-07 &         1.82e-08 &    1.49e-03 & 3.69e-03 \\
211490999.01 &     2.10e-05 &         4.38e-13 &    3.53e-04 &        1.74e-08 &     3.10e-06 &         1.30e-21 &    2.91e-02 & 1.28e-02 \\
211502222.01 &    3.04e-136 &         0.00e+00 &    3.43e-17 &        1.92e-18 &     0.00e+00 &        1.30e-146 &    1.38e-06 & 2.62e-11 \\
211502222.02 &     2.57e-06 &         6.71e-09 &    1.46e-05 &        1.66e-07 &     6.17e-07 &         2.63e-09 &    5.83e-03 & 3.07e-03 \\
211578235.01 &     2.46e-03 &         2.38e-04 &    7.38e-03 &        2.44e-04 &     7.65e-04 &         1.62e-05 &    4.45e-03 & 7.14e-01 \\
211579112.01 &     3.54e-11 &         6.45e-12 &    5.52e-06 &        1.58e-07 &     2.97e-07 &         7.04e-08 &    2.23e-03 & 2.70e-03 \\
211611158.02 &     1.15e-05 &         1.11e-29 &    6.40e-05 &        1.11e-09 &     5.99e-20 &         8.72e-17 &    4.43e-03 & 1.68e-02 \\
211647930.01 &     1.01e-09 &         2.28e-88 &    5.96e-24 &        8.14e-48 &     3.08e-08 &         4.80e-11 &    4.27e-03 & 7.46e-06 \\
211694226.01 &     6.88e-04 &         2.08e-03 &    2.16e-04 &        7.91e-05 &     1.62e-05 &         2.09e-05 &    3.18e-02 & 8.88e-02 \\
211730024.01 &     3.12e-22 &        1.11e-100 &    8.89e-08 &        9.20e-10 &     3.10e-15 &         2.82e-11 &    1.15e-02 & 7.83e-06 \\
211743874.01 &     5.09e-07 &         1.15e-30 &    5.97e-06 &        8.43e-08 &     7.55e-08 &         7.38e-10 &    4.01e-03 & 1.65e-03 \\
211762841.01 &     1.63e-03 &         6.82e-03 &    1.69e-03 &        3.98e-04 &     1.39e-05 &         6.48e-05 &    7.18e-02 & 1.29e-01 \\
211763214.01 &     0.00e+00 &         0.00e+00 &    1.90e-21 &        1.40e-15 &     1.41e-17 &         1.79e-36 &    9.87e-04 & 1.43e-12 \\
211770696.01 &     8.75e-08 &         5.38e-80 &   1.27e-131 &        1.29e-53 &     8.17e-12 &         8.61e-25 &    1.14e-03 & 7.65e-05 \\
211779390.01 &     2.91e-05 &         4.57e-06 &    2.54e-05 &        3.43e-07 &     5.66e-07 &         1.72e-06 &    1.63e-02 & 3.77e-03 \\
211796070.01 &     4.00e-12 &         1.16e-12 &    1.90e-12 &        2.30e-12 &     6.88e-13 &         2.19e-12 &    8.81e-49 & 1.00e+00 \\
211797637.01 &     7.91e-04 &         5.53e-03 &    8.93e-04 &        3.46e-04 &     4.11e-08 &         1.09e-06 &    1.45e-02 & 3.43e-01 \\
211799258.01 &     0.00e+00 &         0.00e+00 &    5.25e-03 &        3.84e-03 &     9.89e-04 &         3.18e-04 &    4.17e-03 & 7.14e-01 \\
211800191.01 &     1.44e-05 &         0.00e+00 &    1.21e-03 &        3.33e-04 &     1.92e-05 &         2.77e-06 &    1.96e-02 & 7.47e-02 \\
211817229.01 &     1.19e-03 &         3.81e-03 &    2.41e-06 &        7.41e-06 &     3.73e-06 &         2.85e-05 &    4.89e-02 & 9.36e-02 \\
211897691.01 &     1.14e-05 &         4.12e-05 &    1.08e-05 &        2.96e-05 &     7.92e-07 &         3.94e-07 &    1.18e-03 & 7.41e-02 \\
211897691.02 &     3.33e-05 &         6.57e-05 &    3.36e-05 &        2.51e-05 &     1.77e-06 &         1.33e-06 &    1.42e-03 & 1.02e-01 \\
211923431.01 &     6.27e-09 &         7.11e-10 &    3.97e-07 &        2.96e-15 &     2.31e-07 &         1.69e-09 &    2.17e-03 & 2.94e-04 \\
211939692.04 &     3.42e-08 &         4.74e-20 &    1.28e-04 &        2.17e-06 &     4.52e-07 &         5.82e-08 &    2.12e-05 & 8.60e-01 \\
211965883.01 &     4.69e-05 &         8.29e-13 &    4.74e-04 &        1.19e-04 &     4.31e-05 &         4.71e-06 &    2.75e-03 & 2.00e-01 \\
211978988.01 &     2.18e-06 &        3.24e-123 &    1.79e-05 &        5.19e-07 &     1.34e-12 &         3.46e-27 &    1.74e-02 & 1.18e-03 \\
211987231.01 &     8.84e-86 &        3.45e-303 &    9.06e-03 &        2.37e-04 &     2.93e-04 &         2.53e-06 &    1.01e-04 & 9.90e-01 \\
211995398.01 &     1.42e-07 &         3.03e-09 &    3.20e-09 &        5.94e-13 &     6.17e-59 &         3.14e-42 &    2.75e-03 & 5.40e-05 \\
211997641.01 &     0.00e+00 &         0.00e+00 &    0.00e+00 &        2.29e-02 &     3.61e-04 &         5.31e-04 &    1.14e-04 & 9.95e-01 \\
212006318.01 &     8.30e-06 &         6.26e-13 &    8.15e-05 &        1.11e-06 &     4.57e-06 &         4.11e-09 &    4.56e-03 & 2.05e-02 \\
212009150.01 &     1.14e-05 &         4.58e-06 &    2.68e-06 &        4.60e-14 &     6.37e-08 &         5.92e-08 &    1.72e-04 & 9.81e-02 \\
212040382.01 &     3.30e-99 &         0.00e+00 &    3.15e-04 &        2.79e-22 &     3.86e-18 &         1.92e-13 &    1.82e-02 & 1.70e-02 \\
212041476.01 &     2.07e-05 &         1.45e-06 &    7.51e-06 &        1.49e-07 &     1.17e-05 &         4.09e-07 &    7.89e-02 & 5.31e-04 \\
212058012.01 &     2.24e-06 &         5.49e-32 &    2.09e-04 &        1.84e-09 &     9.24e-09 &         8.13e-13 &    3.86e-02 & 5.43e-03 \\
212072539.01 &     1.84e-07 &         2.30e-43 &   1.05e-195 &       7.94e-112 &     1.18e-55 &         6.15e-41 &    2.07e-03 & 8.88e-05 \\
212072539.02 &     2.58e-04 &         1.01e-03 &    1.91e-04 &        1.08e-04 &     4.41e-05 &         2.16e-05 &    3.67e-02 & 4.27e-02 \\
212081533.01 &     0.00e+00 &         1.62e-54 &    1.63e-17 &        6.43e-21 &     5.45e-06 &         5.58e-14 &    3.44e-02 & 1.59e-04 \\
212088059.01 &     2.21e-05 &         1.36e-34 &    7.45e-08 &        5.42e-08 &     4.04e-08 &         2.35e-08 &    2.47e-02 & 9.00e-04 \\
212132195.01 &     0.00e+00 &         0.00e+00 &    1.13e-06 &        1.88e-07 &     2.50e-18 &         3.77e-15 &    1.38e-02 & 9.57e-05 \\
212161956.01 &     8.03e-06 &         4.74e-08 &    1.97e-05 &        1.08e-06 &     5.50e-06 &         7.07e-08 &    1.55e-02 & 2.22e-03 \\
212178066.01 &     1.00e-07 &         1.32e-23 &    5.81e-06 &        7.82e-08 &     4.83e-08 &         2.22e-12 &    1.55e-03 & 3.88e-03 \\
212204403.01 &     1.76e-04 &         1.35e-36 &    1.25e-06 &        1.74e-11 &     1.16e-27 &         2.24e-27 &    7.94e-02 & 2.23e-03 \\
212204403.02 &     3.72e-06 &         4.18e-23 &    2.90e-06 &        6.37e-08 &     1.64e-14 &         1.01e-16 &    6.10e-03 & 1.09e-03 \\
212278644.01 &     1.43e-03 &         6.70e-04 &    2.79e-04 &        6.85e-06 &     5.12e-05 &         2.12e-07 &    0.00e+00 & 1.00e+00 \\
212297394.01 &     3.85e-05 &         2.54e-39 &    4.22e-06 &        1.50e-06 &     8.13e-07 &         1.23e-09 &    1.54e-02 & 2.92e-03 \\
212420823.01 &     1.75e-06 &         3.52e-37 &    3.18e-06 &        7.20e-10 &     8.77e-08 &         4.70e-09 &    3.19e-03 & 1.57e-03 \\
212428509.01 &     5.81e-05 &         0.00e+00 &    1.71e-02 &        1.19e-03 &     9.56e-04 &         2.22e-06 &    1.27e-04 & 9.93e-01 \\
212435047.01 &     9.99e-04 &        8.63e-218 &    1.40e-03 &        2.12e-04 &     0.00e+00 &         3.40e-23 &    1.70e-02 & 1.33e-01 \\
212440430.01 &     2.02e-05 &         4.82e-08 &    2.45e-05 &        6.33e-08 &     1.35e-08 &         1.38e-12 &    1.42e-02 & 3.14e-03 \\
212440430.02 &     2.90e-05 &         1.30e-15 &    4.73e-06 &        3.79e-08 &     1.36e-06 &         1.02e-08 &    7.97e-03 & 4.39e-03 \\
212495601.01 &     1.37e-06 &         5.23e-42 &    3.01e-06 &        8.27e-09 &     2.94e-15 &         6.04e-13 &    0.00e+00 & 1.00e+00 \\
212543933.01 &     1.29e-05 &         3.37e-10 &    1.12e-05 &        7.01e-07 &     1.11e-07 &         1.19e-09 &    1.73e-02 & 1.43e-03 \\
212570977.01 &     2.74e-56 &         0.00e+00 &    1.98e-03 &        7.06e-12 &     5.32e-05 &         1.08e-11 &    8.40e-03 & 1.95e-01 \\
212587672.01 &     5.03e-06 &         3.45e-46 &    6.50e-05 &        9.03e-07 &     4.69e-08 &         3.14e-11 &    9.20e-03 & 7.66e-03 \\
212628098.01 &     3.11e-52 &         0.00e+00 &    1.21e-03 &        3.03e-03 &     3.26e-04 &         2.90e-04 &    3.08e-03 & 6.12e-01 \\
212628477.01 &     9.23e-06 &         3.94e-85 &    5.83e-04 &        7.63e-04 &     1.17e-04 &         1.68e-05 &    1.32e-03 & 5.31e-01 \\
212634172.01 &     6.54e-05 &         3.36e-03 &    2.67e-03 &        9.14e-04 &     3.52e-04 &         3.04e-04 &    3.25e-02 & 1.91e-01 \\
212661144.01 &     2.30e-04 &        2.03e-127 &    3.32e-04 &        1.35e-05 &     7.72e-05 &         8.01e-06 &    6.53e-02 & 1.00e-02 \\
212690867.01 &     1.39e-03 &         7.96e-04 &    3.02e-04 &        4.80e-05 &     4.50e-05 &         6.43e-06 &    1.79e-03 & 5.92e-01 \\
212797028.01 &     2.97e-05 &        5.45e-283 &    5.44e-05 &        1.97e-05 &     1.19e-04 &         1.83e-06 &    1.81e-04 & 5.53e-01 \\
251319382.01 &     6.66e-07 &         1.22e-11 &    4.27e-06 &        7.25e-12 &     3.74e-08 &         3.30e-14 &    2.47e-02 & 2.01e-04 \\
251319382.02 &     7.62e-07 &        5.55e-157 &    3.53e-05 &        4.27e-10 &     1.30e-08 &         3.48e-30 &    2.72e-02 & 1.32e-03 \\
251319382.03 &     1.69e-05 &         9.16e-06 &    2.07e-04 &        4.27e-05 &     7.05e-07 &         1.18e-06 &    6.40e-03 & 4.15e-02 \\
251554286.01 &     2.94e-06 &        2.03e-276 &    3.74e-05 &        4.43e-08 &     3.86e-11 &         5.34e-21 &    1.27e-02 & 3.16e-03 \\
\hline
\end{tabular}

==> K2 in Cancri and Virginis arxiv/tables/tab_gamma.tex <==
%see speckle column
%https://docs.google.com/spreadsheets/d/1rkl2KmnDyM6GYDNbZQldvsjV2dNm6eGsbKAyqkKUlrQ/edit#gid=366354925
%211987231,212628098,212661144 have companions detected in speckle and gaia DR2
%212088059,212161956, 212563850,251554286 have gaia detections but none in speckle
%
\begin{tabular}{lllll}
\hline
      EPIC & $\Delta_{K_p}$ & $r$ [$\arcsec$] & $\gamma_\mathrm{pri}$ & $\gamma_\mathrm{sec}$ \\
\hline
%%%%%%%%%%%%%%speckle detections; not Kp band actually but z-band~880nm
 211439059 &  1.07 &  0.23 &       1.37 &       3.68 \\
 211941472 &  0.32 &  0.20 &       1.74 &       2.34 \\
 211987231 &  1.70 &  0.94 &       1.21 &       5.77 \\
 212066407 &  4.06 &  0.22 &       1.02 &      43.07 \\
 212315941 &  1.29 &  0.07 &       1.30 &       4.28 \\
 212628098 &  2.39 &  1.65 &       1.11 &      10.05 \\
 212661144 &  2.85 &  2.94 &       1.07 &      14.87 \\
 \hline
 211335816 &  3.24 &  7.65 &       1.05 &      20.75 \\
 211357309 &  2.25 & 18.94 &       1.13 &       8.92 \\
 211383821 &  6.86 & 19.15 &       1.00 &     554.16 \\
 211399359 &  3.83 & 12.35 &       1.03 &      35.01 \\
 211401787 &  6.81 & 26.31 &       1.00 &     529.45 \\
 211413752 &  5.83 &  4.70 &       1.00 &     215.07 \\
 211502222 &  9.62 & 20.22 &       1.00 &    7015.58 \\
 211578235 &  5.58 & 19.61 &       1.01 &     171.32 \\
 211611158 &  5.97 & 11.68 &       1.00 &     246.44 \\
 211765695 &  2.90 & 13.67 &       1.07 &      15.48 \\
 211770696 &  7.17 & 12.29 &       1.00 &     735.68 \\
 211797637 &  4.10 & 15.55 &       1.02 &      44.83 \\
 211826814 &  4.84 & 14.76 &       1.01 &      87.03 \\
 211995398 &  0.60 &  4.17 &       1.58 &       2.74 \\
 212058012 &  2.58 &  6.49 &       1.09 &      11.75 \\
 212088059 &  6.28 & 11.77 &       1.00 &     326.98 \\
 212099230 &  5.29 & 12.30 &       1.01 &     131.12 \\
 212161956 &  3.53 &  8.85 &       1.04 &      26.91 \\
 212178066 & 13.38 & 21.56 &       1.00 &  225299.47 \\
 212278644 &  6.88 & 11.67 &       1.00 &     564.19 \\
 212297394 &  6.21 & 24.20 &       1.00 &     305.79 \\
 212428509 &  3.33 &  1.09 &       1.05 &      22.52 \\
 212435047 &  7.08 & 12.00 &       1.00 &     678.40 \\
 212440430 &  6.08 &  6.00 &       1.00 &     271.20 \\
 212563850 &  1.77 &  9.67 &       1.20 &       6.11 \\
 212690867 &  0.88 & 18.93 &       1.44 &       3.26 \\
 212797028 &  5.99 & 13.27 &       1.00 &     249.67 \\
 251554286 &  4.41 &  9.85 &       1.02 &      59.12 \\
 \hline
\end{tabular}
%  211428897 &   1.04 &           1.14 &      &      \\ %see below
%  %https://exofop.ipac.caltech.edu/k2/edit_obsnotes.php?id=211428897
%  211439059 &   0.20 &           1.00 & 1.40 & 3.51 \\ % new unpublished(?) data from everett & ciardi; not detected in  Gaia
% %  211939692 &   0.20 &           0.37 & 1.71 & 2.41 \\ %new unpublished(?) data from ciardi
%  211987231 &   0.90 &           1.67 & 1.21 & 5.66 \\  %see below too; new unpublished(?) data from ciardi; not detected in Gaia
%  212066407 &   0.20 &           4.00 & 1.03 & 40.81 \\ %see below too; new unpublished(?) data from everett, ciardi, & zeigler; not detected in Gaia
%  212315941 &   0.06 &           1.29 & 1.30 & 4.28 \\ %new unpublished(?) data from everett; not detected in Gaia
%  212628098 &   1.25 &           3.82 & 1.03 & 34.73\\ %PC; see below too; new unpublished(?) data from everett & ciardi; Gemini detected a sec but WIYN did not; has Gaia
%  212661144 &  2.487 &           2.76 &      &     \\ %companion in livingston but speckle data from everett shows no detection; has gaia
%  211941472 &  0.203 & 0.37 & & \\ %M18 candidate but no speckle; new unpublished(?) data from everett & ciardi; has no Gaia
% %  211886472 &   0.30 &           4.00 & 1.03 & 40.81\\ %PC in M18 with speckle
% %  212138198 &   0.27 &           2.04 & 1.15 & 7.55 \\ %PC in M18 with spec; see below too
% %  212534729 &   0.17 &           1.23 & 1.32 & 4.10 \\ % PC in M18 with speckle
% %  212703473 &   0.22 &           0.84 & 1.46 & 3.17\\ %FP; PC in M18 with speckle
% \hline
% %%%%%%%%%%%%%%gaia detections
%  212099230 & 10.1    &           5.25 &           1.01 &          127.0 \\
% %  212297394 &  24.20 &           6.21 &           1.28 &         390.67 \\
%  212628098 &   1.65 &           2.39 &           1.22 &          11.00 \\
%  211987231 &   1.07 &           1.70 &           1.24 &           5.92 \\
%  211399359 &  12.35 &           3.83 &           1.17 &          39.84 \\
%  212440430 &   6.04 &           6.08 &           1.01 &         273.86 \\
%  212428509 &   1.09 &           3.33 &           1.05 &          22.52 \\
% %  211578235 &  19.61 &           5.58 &           1.01 &         172.69 \\ %outside aper
% %  211442571 &  28.05 &           2.13 &           1.14 &           8.09 \\
% %  211799258 &  13.48 &           3.79 &           1.03 &          33.78 \\
% %  211305568 &  19.00 &           3.90 &           1.06 &          38.44 \\
% %  212009150 &  15.75 &           4.62 &           1.01 &          71.42 \\
% %  212585579 &   7.60 &           4.50 &           1.03 &          65.08 \\ %Liv18 FP
% %  212570977 &  21.50 &           3.68 &           1.03 &          30.77 \\
%  212398508 &   2.77 &           3.62 &           1.04 &          29.08 \\ %2 transits only
% %  211817229 &  12.11 &           4.36 &           1.94 &         107.81 \\ %high pm
%  211335816 &   7.65  &            3.24 &         1.05 &          20.75 \\ 
% %  211342524 &   9.87 &           6.55 &           1.19 &         493.06 \\ %Liv18 FP
% %  212066407 &  26.83 &           4.90 &           1.07 &          97.93 \\
% %  212690867 &  18.93 &           0.88 &           1.62 &           3.65 \\
% %  211797637 &  15.55 &           4.10 &           1.03 &          44.99 \\
% %  212634172 &  29.19 &           5.54 &           1.01 &         165.47 \\
%  212058012 &   6.47 &           2.58 &           1.09 &          11.75 \\
% %  211997641 &  19.98 &           3.24 &           1.08 &          21.38 \\
% %  212088059 &  11.77 &           6.28 &           1.01 &         329.21 \\
%  211995398 &   4.20 &           0.60 &           1.58 &           2.74 \\
%  212138198 &   3.00 &           7.81 &           1.01 &        1345.90 \\
% %  211762841 &  14.90 &           4.68 &           1.11 &          82.95 \\
% %  212773272 &  11.16 &          -3.92 &          38.07 &           1.03 \\ %removed
% %  251288417 &  23.51 &           2.18 &           1.13 &           8.42 \\
%  251554286 & 9.85 & 4.41 & 1.02 & 59.12    \\ %new
%  211357309 &  18.94 &           2.25 &           1.13 &           8.92 \\
%  211413752 & 4.70   &           5.83 &           1.01 &         215.07 \\ %not detected in speckle data
%  212161956 & 8.85 & 3.53 & 1.04 & 26.91  \\ %new
%  212661144 &    2.94 & 2.85  & 1.07 & 14.87 \\ 
% %   211401787 & 26.31 & 6.81 & 1.00 & 529.45 \\ % near boundary
%  211428897 &    2.18 & -1.21 & 4.04 & 1.33 \\ %new
%  % 212096658 %ttv
%  212178066 & 21.56 & 13.38 & 1.00 & 225299.47 \\ % crowded field
%  212420823 & 18.47 & 6.47 & 1.00 & 388.38 \\ % new
%  212563850 & 9.67 & 1.77 & 1.20 & 6.11 \\ %new

==> K2 in Cancri and Virginis arxiv/tables/tab_lc.tex <==
EPIC      & c5           & c6           & c16          & c17          & c18          \\
\hline
211314705 & $\checkmark$ &              &              &              &              \\
211579112 & $\checkmark$ &              &              &              &              \\
211763214 & $\checkmark$ &              & $\checkmark$ &              & $\checkmark$ \\
211965883 & $\checkmark$ &              &              &              &              \\
212088059 & $\checkmark$ &              & $\checkmark$ &              & $\checkmark$ \\
212132195 & $\checkmark$ &              &              &              &              \\
212161956 & $\checkmark$ &              &              &              &              \\
212278644 &              & $\checkmark$ &              &              &              \\
212297394 &              & $\checkmark$ &              &              &              \\
212330265 &              & $\checkmark$ &              &              &              \\
212398508 &              & $\checkmark$ &              &              &              \\
212420823 &              & $\checkmark$ &              &              &              \\
212440430 &              & $\checkmark$ &              & $\checkmark$ &              \\
212495601 &              & $\checkmark$ &              & $\checkmark$ &              \\
212543933 &              & $\checkmark$ &              &              &  
     \\
%212563850 &              & $\checkmark$ &              & $\checkmark$ &              \\
\hline

==> K2 in Cancri and Virginis arxiv/tables/tab_obs.tex <==
%current star count: 70
\begin{tabular}{ccccc}
% \begin{tabular}{p{7cm}p{7cm}p{7cm}p{7cm}p{7cm}}
\hline
EPIC & K2/C & AO & SI & RS \\
\hline
211314705 & 5 & This work & This work & \\ %VP here but no spec! 
211335816 & 5/18 & & & This work \\ % FP in DAVE using everest lc; not detected
211336288 & 5/18 & & & \\ %not detected
211357309 & 5/18 & & & This work \\
211383821 & 5/18 & & & D17 \\
211399359 & 5/18 & D19 & & P18 \\ %has Gemini/Keck AO cc; PC in L18 due to LR
211401787 & 5/18 & & M18 & This work \\ %vp; spanish
211413752 & 5/16/18 & & This work & P18 \\ %AO; PC due to AO even though multi; try pixel light curves to determine source; speckle from Everett not in M18
211439059 & 5/18 & & This work & P18 \\ %ao,gb; SI come from Everett not in M18
211490999 & 5/16/18 & & This work & P18 \\ %vespa pc

211502222 & 16 & & & This work \\ %has SOAR speckle .fits 
211578235 & 5/18 & This work & & P18 \\ %has Gemini AO cc from Ciardi not published in P18; spanish
211579112 & 5/18 & This work & This work & \\ %VP here but no spec!
211611158 & 5/16/18 & & & M18 \\ %kp; vp; reran starfit and calcfpp; 0.02 not updating; update fpp in table; longest period; spanish
211645912 & 5/18 & & This work & P18 \\
211647930 & 16 & & & This work \\ %vp, no spec
211694226 & 5/16/18 & & & D17 \\ %new
211730024 & 16 & & & This work \\ %vp, has SOAR SI
211731298 & 5/18 & & & \\ %K19 params is based on GaiaDR2; Z19 is based on H16; VP here but no spec & low SNR!
211743874 & 5/18 & & This work & P18 \\ %vp; add entry in Table 5; everett speckle not reported in M18

211763214 & 5/16/18 & This work & This work & M18 \\ %reran starfit and calcfpp; update fpp in table
211762841 & 5/18 & & & D17 \\
211770696 & 5/18 & & M18 & P18 \\ %vp
211797637 & 5/18 & & & \\ % PC low SNR
211799258 & 5/18 & D17 & & D17 \\ % update star params; Tab1 in D17 used Gemini SI; has Gemini/Keck AO cc
211779390 & 5/18 & & & This work \\ %no spec
211800191 & 5/18 & & M18 & This work \\ %pc->fp, spanish; PC in M18 though FPP=1!
211817229 & 5/18 & & & D17 \\ %gb; spanish
211843564 & 5/18 & & & \\ %from SED fit; inconsistent; see Martinez in exofop; SE
211923431 & 5/18 & This work & & \\ %VP here but no spec! added shARCs AO cc

211939692 & 5/18 & & This work & \\ % PC; SI come from Everett; spanish
211965883 & 5 & This work & This work & D17 \\
211978988 & 5/18 & & & M18 \\  %reran starfit and calcfpp; update fpp in table
211987231 & 5 & & Mat18 & This work \\ %aogb; SI come from Everett
211995398 & 5/18 & & & \\ %from SED fit; no spec; PC here
211997641 & 5/16 & This work & & \\ %has SOAR SI; new; add vespa results; added shARCs AO cc
212006318 & 5/18 & & This work & P18 \\ %M18 PC but no SI
212009150 & 5/16/18 & & & \\ %no spec; PC here
212040382 & 16 & This work & & This work \\ %added shARCs AO cc
212041476 & 16 & & & This work \\ %vp; has SOAR SI

212058012 & 16 & & & This work \\ %vp; has SOAR SI
212072539 & 5/16/18 & & & \\ % VP here but no spec!
212081533 & 16 & This work & & This work \\ %vp; added shARCs AO cc
212088059 & 5/16/18 & This work & This work & D17 \\ %vp but has nearby star outside aperture
212099230 & 5/16/18 & & Mat18 & This work \\ %no secondary from WIYN but has in Gemini! FP in DAVE using everest lc; fp using pixel-ninja; actually 212099120
212132195 & 5/18 & This work & This work & M18 \\ %vp; spanish
212161956 & 5/18 & & This work & \\ %new; add vespa
212178066 & 16/18 & & & This work \\ %vp but be careful on using noisy c18 lc; has SOAR SI
212204403 & 16 & & & This work \\ % vp,vp; has SOAR SI
212278644 & 6 & & & This work \\ 

%%%==50==%%%
212297394 & 6 & & This work & \\ % VP here but no spec!
212420823 & 6 & & This work & This work \\ % new P16,K19; add FPP in Table 5
212428509 & 6/17 & & This work & P18 \\ %SE; PC in Liv18
212435047 & 6/17 & & This work & P18 \\
212440430 & 6/17 & & This work & This work \\ %vp,vp, P16,K19
212495601 & 6/17 & & This work & This work \\ %vespa is VP
212543933 & 6 & & This work & This work \\ %vp
212570977 & 6/17 & & This work & P18 \\
212563850 & 6/17 & & This work & This work \\ %FP in Kruse
212587672 & 6/17 & & M18 & P18 \\ %inner planet is KP by H19

212628098 & 6/17 & & Mat18 & D17 \\ %SI come from Everett not in M18; has Gemini AO cc
212628477 & 17 & & This work & This work \\ %new; add vespa
212634172 & 6/17 & & & D17 \\
212661144 & 6/17 & & This work & \\ %new; add vespa results; SI from Everett not in M18 
212639319 & 6/17 & & M18 & P18 \\ %no vespa results; no signal in C17
212690867 & 6/17 & & & D17 \\
212797028 & 6/17 & & This work & P18 \\ %SI come from Everett; not reported in P18 
251319382 & 16 & & This work & This work \\ %vp,vp,pc
251554286 & 17 & & This work & This work \\ 
\hline
% 212150006 & 5/18 & & & This work \\ % no lcs
% 212036875 & 16 & & This work & This work \\ % new from Yu; unconverged so cant run vespa
% 212066407 & 5/18 & & A18 & P18 \\ %aogb; unconverged SI come from Everett not in M18
% 211906259, 211914960, 212024672, 212796016, 211645912: not detected
% 211305568 & 5/18 & & & D17 \\ %low SNR
% 211342524 & 5/18 & & This work & P18 \\ %L18 FP
% 211428897 & 5/18 & & Mat18 & This work \\ %at least 3-planet system; with nearby companion in speckle accdg to exofop notes; 3 PCs in DAVE: http://keplertcert.seti.org/DAVE/; SI come from Everett
% 211442571 & 5/18 & & & \\ %only K19, FP anyway due to GB but high pm
% 211765695 & 16 & & & \\ % from Fei, pc & pc; no new obs
% 211892082 & 16 & & & \\ % from Fei, vp; no new obs
% 211741619 & 16 & & & D17 \\ %no new data
% 211797214 & 16 & & & \\ % from Fei, vp & pc
% 211796070 & 5/18 & & & \\ %from SED fit; FP anyway
% 211826814 & 5/18 & & & D17 \\ %low SNR; no parallax
% 211886472 & 5/16 & & This work & M18 \\ %no vespa results but has speckle and M18 star params; has Zeigler SOAR also in M18
% 211897691 & 5/16/18 & & & \\ %from SED fit; 2 PCs here; Libralato16 in M44; update vespa for .02
% 211901114 & 5/16/18 & & & \\ %new; unconverged; young
% 211941472 & 5/16/18 & & This work & M18 \\ %not validated by M18 because no speckle; speckle reveals secondary; SI come from Everett; negative parallax
% 211988320 & 5 & & & D17 \\ % PC due to 2 transits
% 212096658 & 5/16/18 & & & \\ % no vespa entry; v-shaped, ttv; SE; FP in K18
% 251288417 & 16 & & & \\ %no vespa entry
% 212138198 & 5/18 & & This work & P18 \\ %ao,gb; M18
% 212315941 & 6 & & Mat18 & \\ % no vespa entry; multi or EB?; ao,gb; SI from from Everett not in M18; no new data
% 212330265 & 6 & & & D17 \\ %no new data
% 212396050 & 6 & & Zeigler & \\ %not detected
% 212398508 & 6 & & This work & This work \\ % 2 tranits only; with gaia; PLA not useful
% 212422536 & 6 & & & \\ %VP but no spec! multi; removed no new data
% 212534729 & 6/17 & & This work & This work \\ %ao,gb; M18
% 212470904 & 6/17 & This work & \\ %new; low snr
% 212585579 & 6 & & This work & P18 \\ %L18 FP; SE
% 212555594 & 6 & & This work & M18 \\ %no vespa entry; rerun vespa with less noisy LC; KP and another candidate from P18 but only 1 camp
% 212572439 & 6/17 & & & This work \\ % FP; true source is 212572452 accdg to DAVE
% 212586030 & 6/17 & & This work & M18 \\ %no vespa entry in Table 5; MCMC not converged; L18 FP
% 212703473 & 6 & & & This work \\ %M18
% 212773272 & 6/17 & & This work & D17 \\ % FP in D17; sec eclipse; SI already reported

% \multicolumn{5}{l}{$^a$ \ktwo campaign}; 
% \multicolumn{5}{l}{$^b$ Adaptive optics}; 
% \multicolumn{5}{l}{$^c$ Speckle imaging};
% \multicolumn{5}{l}{$^d$ Reconnaissance spectroscopy}\\
\end{tabular}

==> K2 in Cancri and Virginis arxiv/tables/tab_obs2.tex <==
\begin{tabular}{ccccccccc}
\hline
EPIC & C5 & C6 & C16 & C17 & C18 & AO$^a$ & SI$^b$ & RS$^c$ \\
\hline
212072539 & \cmark & & \cmark & & \cmark &  &   &   \\
212081533 & & & \cmark & & & \cmark &   &  \cmark\\
212088059 & \cmark & & \cmark & & \cmark &  & \cmark & \cmark  \\ %dressing
212096658 & \cmark & & \cmark & & \cmark &  &   &   \\
212132195 & \cmark & & & & \cmark & \cmark & \cmark &   \\
212138198 & \cmark & & & & \cmark &  & \cmark  & \cmark \\ %Gemini-N/DSSI (692,880nm) %isaacson
212178066 & & & \cmark & & \cmark &  &   &  \cmark\\
212204403 & & & \cmark & & &  &   &  \cmark\\
212278644 & & \cmark & & & &  &   &  \cmark\\
212297394 & & \cmark & & & &  & \cmark &   \\
212315941 & & \cmark & & & &  & \cmark &   \\
212330265 & & \cmark & & & &  &   & \cmark \\ %dressing
212398508 & & \cmark & & & &  & \cmark &  \cmark\\
212422536 & & \cmark & & & &  &   &   \\
212428509 & & \cmark & & \cmark & &  & \cmark & \cmark \\ %isaacson
212435047 & & \cmark & & \cmark & &  & \cmark &  \cmark \\ %isaacson
212440430 & & \cmark & & \cmark & &  & \cmark &  \cmark\\
212495601 & & \cmark & & \cmark & &  & \cmark &  \cmark\\
212534729 & & \cmark & & \cmark & &  & \cmark &  \cmark\\
212543933 & & \cmark & & & &  & \cmark &  \cmark\\
212570977 & & \cmark & & \cmark & &  & \cmark &  \cmark \\ %isaacson
212585579 & & \cmark & & & &  & \cmark & \cmark \\ %isaacson
212586030 & & \cmark & & \cmark & &  & \cmark & \cmark \\ %isaacson
212587672 & & \cmark & & \cmark & &  & \cmark & \cmark \\
212628098 & & \cmark & & \cmark & &  &   &   \\
212634172 & & \cmark & & \cmark & &  &   & \cmark \\ %dressing
212639319 & & \cmark & & \cmark & &  & \cmark &  \cmark \\ %isaacson
212690867 & & \cmark & & \cmark & &  &   & \cmark \\ %dressing
212703473 & & \cmark & & & &  & \cmark &  \cmark\\
212773272 & & \cmark & & \cmark & &  & \cmark & \cmark \\
212797028 & & \cmark & & \cmark & &  & \cmark &   \\
251288417 & & & \cmark & & &  &   & \cmark \\ %dressing
251319382 & & & \cmark & & &  & \cmark &  \cmark\\
212178066 & & & \cmark & & \cmark &  &   &  \cmark\\
212204403 & & & \cmark & & &  &   &  \cmark\\
212278644 & & \cmark & & & &  &   &  \cmark\\
212297394 & & \cmark & & & &  & \cmark &   \\
212315941 & & \cmark & & & &  & \cmark &   \\
212330265 & & \cmark & & & &  &   & \cmark \\ %dressing
212398508 & & \cmark & & & &  & \cmark &  \cmark\\
212422536 & & \cmark & & & &  &   &   \\
212428509 & & \cmark & & \cmark & &  & \cmark & \cmark \\ %isaacson
212435047 & & \cmark & & \cmark & &  & \cmark &  \cmark \\ %isaacson
212440430 & & \cmark & & \cmark & &  & \cmark &  \cmark\\
212495601 & & \cmark & & \cmark & &  & \cmark &  \cmark\\
212534729 & & \cmark & & \cmark & &  & \cmark &  \cmark\\
212543933 & & \cmark & & & &  & \cmark &  \cmark\\
212570977 & & \cmark & & \cmark & &  & \cmark &  \cmark \\ %isaacson
212585579 & & \cmark & & & &  & \cmark & \cmark \\ %isaacson
212586030 & & \cmark & & \cmark & &  & \cmark & \cmark \\ %isaacson
212587672 & & \cmark & & \cmark & &  & \cmark & \cmark \\
212628098 & & \cmark & & \cmark & &  &   &   \\
212634172 & & \cmark & & \cmark & &  &   & \cmark \\ %dressing
212639319 & & \cmark & & \cmark & &  & \cmark &  \cmark \\ %isaacson
212690867 & & \cmark & & \cmark & &  &   & \cmark \\ %dressing
212703473 & & \cmark & & & &  & \cmark &  \cmark\\
212773272 & & \cmark & & \cmark & &  & \cmark & \cmark \\
212797028 & & \cmark & & \cmark & &  & \cmark &   \\
251288417 & & & \cmark & & &  &   & \cmark \\ %dressing
251319382 & & & \cmark & & &  & \cmark &  \cmark\\
%211335816, 211428897, 212150006, 212099230, 212420823, 212470904, 212563850, 212572439,  212684448, 211446060, 211604981, 211858489, 212036875, 212048748, 251554286, 212628477
\hline
\multicolumn{9}{l}{$^a$ Adaptive optics}\\
\multicolumn{9}{l}{$^b$ Speckle imaging}\\
\multicolumn{9}{l}{$^c$ Reconnaissance spectroscopy}\\
\end{tabular}
% %see https://docs.google.com/spreadsheets/d/1Giwxhjnc7kq1K1-IfWDI1DZpVcCfyzZgHBgs_VHn-3w/edit#gid=994714091
% EPIC      & photometry        & AO imaging  &  /lucky imaging & recon.  specarchival imaging \\ \hline %& parallax\\ \hline
% 211314705 & \ktwo/c5           & Subaru/IRCS & WIYN/NESSI & TRES & - \\%& Gaia DR2 \\ %NOT in Kruse+2019
% 211579112 & \ktwo/c5           & Subaru/IRCS & WIYN/NESSI & - & - \\%& Gaia DR2 \\ %planet candidates in or near the habitable zone with planet radii small than 2 R⊕ also found recently by Kruse+2019
% 211763214 & \ktwo/c5,16,18  & Subaru/IRCS   & WIYN/NESSI,DSSI & - %TRES: no uncertainty 
% & POSS \\%& Gaia DR2\\
% 212088059 & \ktwo/c5,16,18  & Subaru/IRCS & WIYN/NESSI & - & POSS \\%& Gaia DR2\\
% 212132195 & \ktwo/c5           & Subaru/IRCS & WIYN/NESSI,DSSI & SpEX, TRES & POSS \\%& Gaia DR2\\
% 212161956 & \ktwo/c5,18        &     -        & WIYN/NESSI & - & POSS \\%& Gaia DR2\\
% 212278644 & \ktwo/c6           &     -       &  -          & McDonald/Tull & - \\%& Gaia DR2\\ %NOT in Kruse+2019
% 212297394 & \ktwo/c6           &     -        & WIYN/DSSI  & NOT/FIES & - \\%& Gaia DR2\\ %multiplanet; 0.2 has 2.28896-d based on TLS survey II (Heller+2019)
% 212330265 & \ktwo/c6           &     -        &  -          & -  & POSS \\%& Gaia DR2\\ 
% 212398508 & \ktwo/c6           &     -        & WIYN/NESSI & McDonald/Tull & POSS \\%& Gaia DR2\\
% 212420823 & \ktwo/c6           &     -        & WIYN/NESSI & NOT/FIES & - \\%& Gaia DR2\\
% 212440430 & \ktwo/c6,17      &       -      & WIYN/DSSI & McDonald/Tull & - \\%& Gaia DR2\\
% 212495601 & \ktwo/c6,17      &       -      & WIYN/NESSI & McDonald/Tull & - \\%& Gaia DR2 \\
% 212543933 & \ktwo/c6           &     -        & WIYN/DSSI & McDonald/Tull & - \\%& Gaia DR2\\
% %212563850 & \ktwo/c6,17      &             & WIYN/NESSI & McDonald/Tull & POSS1 & Gaia DR2\\  %FP
% %\hline
% % additional
% %212178066 & \ktwo/c16 &             & FASTcam & McDonald/Tull \\
% %251319382 & \ktwo/c16 &             & FASTcam & McDonald/Tull, TRES \\
% %211502222 & \ktwo/c16 &             & FASTcam & McDonald/Tull, TRES \\
% %212048748 & \ktwo/c16 & Subaru/IRCS &         & McDonald/Tull \\
% %212081533 & \ktwo/c16 & Subaru/IRCS &         & McDonald/Tull \\
% %TSPEC
% % http://www.astro.caltech.edu/palomar/observer/200inchResources/tspecspecs.html
% %WIYN/NESSI (NASA Exoplanet Star (and)   Imager) is a   instrument that utilizes two electron-multiplying CCD cameras to capture   images in two colors simultaneously.   observations provide resolutions at or near the diffraction limit of the telescope allowing companion detection and characterization to delta magnitudes of approximately 5. NESSI will have remote controlled filter wheels in each beam, split by the dichroic at 686.4nm.
% % http://www.wiyn.org/Instruments/wiynnessi.html
% %DSSI (Differential   Survey Instrument, built by Elliott Horch, SCSU) provides simultaneous 2-band diffraction-limited high-resolution optical imaging (FWHM~0.05" at 650nm) of targets as faint as V~15, over a ~2.8 arcsecond field-of-view. DSSI will be offered once or twice in the semester, depending on demand. The visiting DSSI instrument team will operate a mini-queue program during these runs and will take all observations for successful proposers. The DSSI team will provide their standard pipeline-reduced data products (includes reconstructed image and sensitivity curve) to PIs. There is no requirement to collaborate with the DSSI team for this level of service. Details of the use of DSSI at WIYN are given in Howell et al., 2011, AJ, 142, 19, Horch et al., 2012, AJ, 143, 10, and 2011, AJ, 141, 180. The PI for this program is Steve Howell (NASA Ames Research Center).
% %TRES (Tillinghast Reflector Echelle Spectrograph) is a fiber-fed (sky+object+calibration spectrum) optical echelle spectrograph on the 1.5-meter Tillinghast telescope at the Smithsonian Astrophysical Observatory's Fred L. Whipple Observatory on Mt. Hopkins in Arizona.
% % http://tdc-www.harvard.edu/instruments/tres/

==> K2 in Cancri and Virginis arxiv/tables/tab_planet_fpp1.tex <==
\renewcommand{\arraystretch}{1.5}
\begin{tabular}{lllllllllrrllll}
\hline
% \scriptsize
EPIC &             Name &            $T_{0}$ [BKJD] &                              $P$ [d] &      $R_p/R_{\star}$ [\%] &              $a/R_{\star}$ &                     $b$ &            $T_{14}$ [hr] &            \Teq [K] &             $R_p$ [\rearth] &     SNR &  FPP &  notes & disposition &           ref \\
\hline
211314705.01 & K2-329 b &  2307.225970$^{+0.004008}_{-0.003737}$ &   3.793306$^{+0.000324}_{-0.000343}$ &   3.53$^{+0.17}_{-0.17}$ &    19.05$^{+0.21}_{-0.21}$ &  0.24$^{+0.17}_{-0.16}$ &   1.53$^{+0.04}_{-0.08}$ &       543$^{+8}_{-9}$ &      1.56$^{+0.08}_{-0.08}$ &   20.49 & 0.00 &            &          VP &        P16 \\
211357309.01 & &  2306.751359$^{+0.000665}_{-0.000677}$ &   0.463975$^{+0.000000}_{-0.000000}$ &   1.59$^{+0.12}_{-0.05}$ &     3.78$^{+0.47}_{-1.04}$ &  0.47$^{+0.32}_{-0.32}$ &   0.86$^{+0.05}_{-0.04}$ &    1269$^{+18}_{-15}$ &      0.86$^{+0.07}_{-0.03}$ &   72.92 & 0.05 &            &          PC &        A16 \\
211383821.01 & &  2307.154894$^{+0.001782}_{-0.001753}$ &   1.567125$^{+0.000003}_{-0.000003}$ &   1.81$^{+0.21}_{-0.08}$ &     6.41$^{+0.67}_{-1.77}$ &  0.42$^{+0.35}_{-0.29}$ &   1.74$^{+0.09}_{-0.08}$ &    1005$^{+15}_{-13}$ &      1.24$^{+0.14}_{-0.06}$ &   25.67 & 0.03 &            &          PC &        P16 \\
211399359.01 & &  2308.417493$^{+0.000125}_{-0.000118}$ &   3.114897$^{+0.000001}_{-0.000001}$ &  15.06$^{+0.09}_{-0.08}$ &    11.64$^{+0.09}_{-0.16}$ &  0.10$^{+0.10}_{-0.07}$ &   2.34$^{+0.01}_{-0.01}$ &     979$^{+20}_{-22}$ &     12.94$^{+0.40}_{-0.34}$ &  479.01 & 0.00 &         LR &          PC &        P16 \\
211401787.01 & K2-330 b &  2318.064162$^{+0.001517}_{-0.001464}$ &  13.774798$^{+0.000028}_{-0.000028}$ &   1.69$^{+0.08}_{-0.03}$ &    21.76$^{+1.56}_{-4.85}$ &  0.38$^{+0.32}_{-0.26}$ &   4.57$^{+0.08}_{-0.07}$ &       969$^{+9}_{-9}$ &      2.77$^{+0.14}_{-0.09}$ &   57.88 & 0.00 &            &          VP &        P16 \\
211413752.01 & K2-268 b &  2307.846650$^{+0.002133}_{-0.002101}$ &   9.327527$^{+0.000021}_{-0.000020}$ &   3.12$^{+0.91}_{-0.22}$ &    17.17$^{+4.82}_{-9.46}$ &  0.65$^{+0.30}_{-0.45}$ &   3.35$^{+0.62}_{-0.11}$ &     696$^{+12}_{-13}$ &      2.69$^{+0.77}_{-0.21}$ &  141.74 &   -- &            &          KP &  L18 \\
211413752.02 & K2-268 c &  2310.654276$^{+0.002437}_{-0.002523}$ &   2.151676$^{+0.000005}_{-0.000006}$ &   1.75$^{+0.14}_{-0.06}$ &     7.76$^{+0.72}_{-1.84}$ &  0.42$^{+0.33}_{-0.30}$ &   1.97$^{+0.06}_{-0.05}$ &    1136$^{+18}_{-19}$ &      1.50$^{+0.12}_{-0.07}$ &   34.08 &   -- &            &          KP &  L18 \\
211413752.03 & K2-268 f &  2309.191739$^{+0.003964}_{-0.003853}$ &  26.270570$^{+0.000105}_{-0.000109}$ &   2.59$^{+0.17}_{-0.08}$ &    41.41$^{+3.15}_{-8.33}$ &  0.39$^{+0.29}_{-0.27}$ &   4.62$^{+0.13}_{-0.11}$ &      492$^{+8}_{-10}$ &      2.23$^{+0.15}_{-0.09}$ &   27.64 & 0.00 &            &          VP &        K19 \\
211413752.04 & K2-268 d &  2310.974654$^{+0.003182}_{-0.003300}$ &   4.528598$^{+0.000016}_{-0.000015}$ &   1.73$^{+0.16}_{-0.06}$ &    12.57$^{+1.18}_{-3.32}$ &  0.40$^{+0.35}_{-0.28}$ &   2.57$^{+0.12}_{-0.10}$ &     888$^{+16}_{-15}$ &      1.49$^{+0.14}_{-0.07}$ &   74.65 & 0.05 &            &          VP &        K19 \\
211413752.05 & K2-268 e &  2309.343959$^{+0.004850}_{-0.004706}$ &   6.131243$^{+0.000032}_{-0.000033}$ &   1.55$^{+0.13}_{-0.08}$ &    16.93$^{+1.89}_{-4.06}$ &  0.42$^{+0.32}_{-0.28}$ &   2.54$^{+0.14}_{-0.13}$ &     801$^{+13}_{-13}$ &      1.33$^{+0.11}_{-0.08}$ &   24.63 & 0.00 &            &          VP &        K19 \\
211439059.01 & &  2313.521148$^{+0.007066}_{-0.008427}$ &  18.637056$^{+0.000183}_{-0.000174}$ &   1.68$^{+0.14}_{-0.09}$ &    24.57$^{+2.88}_{-6.31}$ &  0.42$^{+0.33}_{-0.29}$ &   5.32$^{+0.33}_{-0.28}$ &     610$^{+18}_{-21}$ &      2.15$^{+0.21}_{-0.16}$ &   13.76 & 0.00 &         GB &          FP &        P16 \\
211490999.01 & &  2313.329630$^{+0.002489}_{-0.002464}$ &   9.844401$^{+0.000706}_{-0.000686}$ &   2.86$^{+0.18}_{-0.09}$ &    19.68$^{+1.63}_{-4.63}$ &  0.40$^{+0.32}_{-0.27}$ &   3.64$^{+0.12}_{-0.10}$ &     799$^{+19}_{-24}$ &      2.96$^{+0.21}_{-0.16}$ &   36.86 & 0.01 &            &          PC &        P16 \\
211502222.01 & K2-331 c &  3280.304754$^{+0.002330}_{-0.002335}$ &  22.996591$^{+0.001848}_{-0.001859}$ &   2.35$^{+0.11}_{-0.07}$ &    37.87$^{+2.65}_{-7.38}$ &  0.37$^{+0.30}_{-0.25}$ &   4.43$^{+0.10}_{-0.09}$ &     673$^{+12}_{-11}$ &      2.72$^{+0.14}_{-0.10}$ &   33.14 & 0.00 &            &          VP &        Y18 \\
211502222.02 & K2-331 b &  3267.920192$^{+0.005312}_{-0.005582}$ &   9.398977$^{+0.001506}_{-0.001348}$ &   1.55$^{+0.12}_{-0.07}$ &    16.76$^{+1.93}_{-4.78}$ &  0.43$^{+0.34}_{-0.29}$ &   3.92$^{+0.22}_{-0.19}$ &     909$^{+14}_{-14}$ &      1.79$^{+0.14}_{-0.10}$ &   20.63 & 0.00 &            &          VP &  This work \\
211578235.01 & &  2314.979746$^{+0.000259}_{-0.000261}$ &  11.007605$^{+0.000004}_{-0.000004}$ &  12.95$^{+5.24}_{-3.07}$ &    30.60$^{+2.90}_{-1.51}$ &  0.98$^{+0.07}_{-0.06}$ &   1.56$^{+0.03}_{-0.05}$ &     874$^{+34}_{-35}$ &     16.49$^{+6.44}_{-4.00}$ &  266.82 & 0.71 &         LR &          PC &        B16 \\
211579112.01 & &  2323.420746$^{+0.002160}_{-0.002168}$ &  17.706320$^{+0.000063}_{-0.000063}$ &   7.07$^{+0.33}_{-0.31}$ &    66.30$^{+2.39}_{-2.60}$ &  0.39$^{+0.13}_{-0.20}$ &   2.03$^{+0.09}_{-0.10}$ &       266$^{+5}_{-8}$ &      2.20$^{+0.19}_{-0.15}$ &   17.04 & 0.00 &            &          VP &        P16 \\
211611158.01 & K2-185 b &  2311.727092$^{+0.005898}_{-0.005466}$ &  10.616384$^{+0.000069}_{-0.000074}$ &   1.11$^{+0.06}_{-0.06}$ &    21.50$^{+0.85}_{-0.92}$ &  0.74$^{+0.05}_{-0.05}$ &   2.60$^{+0.17}_{-0.18}$ &     809$^{+22}_{-25}$ &      1.15$^{+0.07}_{-0.07}$ &   16.71 &   -- &            &          KP &  M18 \\
211611158.02 & K2-185 c &  2326.157391$^{+0.002498}_{-0.002358}$ &  52.713494$^{+0.000155}_{-0.000164}$ &   2.32$^{+0.05}_{-0.05}$ &    62.62$^{+2.50}_{-2.69}$ &  0.73$^{+0.03}_{-0.03}$ &   4.64$^{+0.08}_{-0.08}$ &     477$^{+14}_{-17}$ &      2.39$^{+0.09}_{-0.09}$ &   48.91 & 0.02 &            &          VP &        M18 \\
211647930.01 & K2-333 b &  3264.395983$^{+0.000766}_{-0.000749}$ &  14.759287$^{+0.000243}_{-0.000240}$ &   4.61$^{+0.10}_{-0.05}$ &    23.06$^{+0.72}_{-2.14}$ &  0.26$^{+0.23}_{-0.18}$ &   4.96$^{+0.05}_{-0.04}$ &     826$^{+14}_{-17}$ &      6.18$^{+0.28}_{-0.25}$ &  113.06 & 0.00 &            &          VP &        Y18 \\
211694226.01 & &  2342.946754$^{+0.002181}_{-0.002209}$ &   1.918518$^{+0.000006}_{-0.000006}$ &   1.61$^{+0.18}_{-0.13}$ &    12.01$^{+2.49}_{-3.32}$ &  0.42$^{+0.35}_{-0.30}$ &   1.09$^{+0.14}_{-0.14}$ &     816$^{+16}_{-23}$ &      1.08$^{+0.13}_{-0.10}$ &   13.54 & 0.09 &            &          PC &        D17 \\
211730024.01 & K2-334 b &  3263.810228$^{+0.000550}_{-0.000536}$ &   5.113981$^{+0.000061}_{-0.000062}$ &   3.43$^{+0.18}_{-0.05}$ &    15.35$^{+1.09}_{-3.58}$ &  0.38$^{+0.33}_{-0.26}$ &   2.46$^{+0.06}_{-0.03}$ &    1380$^{+34}_{-30}$ &      5.65$^{+0.36}_{-0.28}$ &  133.98 & 0.00 &            &          VP &        Y18 \\
211743874.01 & K2-335 b &  2315.209626$^{+0.002700}_{-0.002774}$ &  12.283211$^{+0.000051}_{-0.000051}$ &   1.51$^{+0.08}_{-0.05}$ &    20.30$^{+1.76}_{-4.76}$ &  0.40$^{+0.31}_{-0.28}$ &   4.31$^{+0.13}_{-0.12}$ &     949$^{+21}_{-26}$ &      2.21$^{+0.18}_{-0.14}$ &   24.89 & 0.00 &            &          VP &        P16 \\
211762841.01 & &  2307.265782$^{+0.000812}_{-0.000828}$ &   1.565010$^{+0.000002}_{-0.000002}$ &   2.89$^{+0.29}_{-0.16}$ &    16.94$^{+2.87}_{-4.05}$ &  0.43$^{+0.31}_{-0.28}$ &   0.65$^{+0.06}_{-0.08}$ &     931$^{+13}_{-13}$ &      1.91$^{+0.19}_{-0.12}$ &   21.45 & 0.13 &            &          PC &        D17 \\
211763214.01 & K2-336 b &  2313.585567$^{+0.004276}_{-0.004476}$ &  21.194733$^{+0.000108}_{-0.000107}$ &   1.40$^{+0.10}_{-0.05}$ &    32.37$^{+2.92}_{-8.35}$ &  0.41$^{+0.33}_{-0.28}$ &   4.65$^{+0.16}_{-0.14}$ &     569$^{+15}_{-22}$ &      1.22$^{+0.09}_{-0.05}$ &   22.34 & 0.00 &            &          VP &        P16 \\
211770696.01 & K2-337 b &  2312.963531$^{+0.002514}_{-0.002528}$ &  16.273563$^{+0.000054}_{-0.000053}$ &   1.80$^{+0.10}_{-0.04}$ &    15.39$^{+1.13}_{-3.59}$ &  0.38$^{+0.32}_{-0.26}$ &   7.64$^{+0.14}_{-0.11}$ &     850$^{+19}_{-18}$ &      2.62$^{+0.19}_{-0.14}$ &   41.74 & 0.00 &            &          VP &        P16 \\
211779390.01 & K2-338 b &  2308.526349$^{+0.001912}_{-0.001839}$ &   3.850614$^{+0.000012}_{-0.000012}$ &   1.48$^{+0.15}_{-0.07}$ &    15.13$^{+1.75}_{-4.06}$ &  0.42$^{+0.34}_{-0.29}$ &   1.78$^{+0.11}_{-0.10}$ &     783$^{+12}_{-14}$ &      1.03$^{+0.11}_{-0.05}$ &   21.05 & 0.00 &            &          VP &        P16 \\
211796070.01 & &  2307.731014$^{+0.002660}_{-0.002404}$ &   1.889933$^{+0.000007}_{-0.000007}$ &   1.44$^{+0.09}_{-0.07}$ &     8.83$^{+1.23}_{-2.28}$ &  0.42$^{+0.33}_{-0.29}$ &   1.50$^{+0.13}_{-0.12}$ &    1371$^{+57}_{-63}$ &      1.40$^{+0.10}_{-0.08}$ &   15.16 & 1.00 &            &          FP &        B16 \\
211797637.01 & &  2306.788585$^{+0.002729}_{-0.002963}$ &   1.640772$^{+0.000112}_{-0.000102}$ &   1.62$^{+0.13}_{-0.09}$ &    10.09$^{+2.04}_{-3.24}$ &  0.45$^{+0.35}_{-0.31}$ &   1.11$^{+0.15}_{-0.14}$ &    1315$^{+59}_{-52}$ &      1.34$^{+0.15}_{-0.08}$ &   53.49 & 0.34 &            &          PC &        B16 \\
211799258.01 & &  2320.146470$^{+0.000338}_{-0.000330}$ &  19.533884$^{+0.000009}_{-0.000009}$ &  27.02$^{+1.82}_{-1.52}$ &  125.14$^{+16.96}_{-9.74}$ &  0.59$^{+0.11}_{-0.25}$ &   1.34$^{+0.06}_{-0.07}$ &       326$^{+5}_{-7}$ &     13.04$^{+0.95}_{-0.82}$ &  112.72 & 0.71 &         LR &          PC &        D17 \\
\hline
\end{tabular}

==> K2 in Cancri and Virginis arxiv/tables/tab_planet_fpp2.tex <==
%212099230 is an NEB
\renewcommand{\arraystretch}{1.5}
\begin{tabular}{lllllllllrrllll}
\hline
EPIC &          Name &               $T_{0}$ [BKJD] &                              $P$ [d] &      $R_p/R_{\star}$ [\%] &              $a/R_{\star}$ &                     $b$ &            $T_{14}$ [hr] &            \Teq [K] &             $R_p$ [\rearth] &     SNR &  FPP &  notes & disposition &           ref \\
\hline
211800191.01 & &  2307.749483$^{+0.000190}_{-0.000208}$ &   1.106170$^{+0.000000}_{-0.000000}$ &   4.79$^{+2.51}_{-0.46}$ &     3.01$^{+0.47}_{-0.32}$ &  0.96$^{+0.04}_{-0.02}$ &   1.22$^{+0.04}_{-0.08}$ &    2011$^{+42}_{-46}$ &      6.42$^{+3.40}_{-0.75}$ &  329.65 & 0.07 &            &          PC &        P16 \\
211817229.01 & &  2307.694394$^{+0.000563}_{-0.000557}$ &   4.353783$^{+0.000003}_{-0.000003}$ &   6.55$^{+0.58}_{-0.41}$ &  86.19$^{+16.61}_{-22.23}$ &  0.41$^{+0.33}_{-0.29}$ &   0.37$^{+0.06}_{-0.05}$ &       348$^{+2}_{-2}$ &      1.14$^{+0.10}_{-0.07}$ &   37.80 & 0.09 &            &          PC &        D17 \\
211843564.01 & &  2307.077984$^{+0.000425}_{-0.000489}$ &   0.452018$^{+0.000000}_{-0.000000}$ &   7.93$^{+2.11}_{-0.42}$ &     4.96$^{+0.74}_{-1.95}$ &  0.49$^{+0.40}_{-0.35}$ &   0.68$^{+0.10}_{-0.05}$ &    1345$^{+23}_{-31}$ &      5.12$^{+1.30}_{-0.37}$ &   70.96 & 0.20 &         GB &          FP &        K19 \\
211897691.01 & &  2309.493095$^{+0.001192}_{-0.001177}$ &   5.750534$^{+0.000007}_{-0.000007}$ &   2.81$^{+0.25}_{-0.09}$ &    33.89$^{+3.12}_{-8.35}$ &  0.41$^{+0.32}_{-0.29}$ &   1.22$^{+0.05}_{-0.04}$ &     761$^{+14}_{-20}$ &      2.23$^{+0.20}_{-0.12}$ &   44.28 & 0.07 &        rho &          PC &        P16 \\
211897691.02 & K2-339 b &  2320.004667$^{+0.004642}_{-0.005128}$ &  19.507428$^{+0.000116}_{-0.000113}$ &   2.44$^{+0.23}_{-0.12}$ &   40.71$^{+4.50}_{-11.08}$ &  0.44$^{+0.33}_{-0.30}$ &   3.40$^{+0.18}_{-0.16}$ &     508$^{+12}_{-12}$ &      1.92$^{+0.19}_{-0.12}$ &   34.81 & 0.10 &            &          VP &        K19 \\
211923431.01 & K2-340 b &  2310.815863$^{+0.002975}_{-0.003102}$ &  29.740451$^{+0.000169}_{-0.000161}$ &   2.68$^{+0.17}_{-0.10}$ &    40.80$^{+3.40}_{-9.36}$ &  0.39$^{+0.31}_{-0.27}$ &   5.29$^{+0.19}_{-0.15}$ &     606$^{+31}_{-36}$ &      3.36$^{+0.44}_{-0.32}$ &   23.52 & 0.00 &            &          VP &        P16 \\
211939692.04 & &  2333.057118$^{+0.006513}_{-0.006699}$ &  26.855455$^{+0.000193}_{-0.000186}$ &   3.24$^{+1.31}_{-0.50}$ &     5.96$^{+0.73}_{-0.55}$ &  0.98$^{+0.02}_{-0.01}$ &  10.77$^{+0.39}_{-0.48}$ &     804$^{+32}_{-42}$ &      4.91$^{+1.97}_{-0.76}$ &   95.22 & 0.86 &            &          PC &        K19 \\
211965883.01 & &  2313.496997$^{+0.002648}_{-0.002570}$ &  21.110323$^{+0.001461}_{-0.001397}$ &   3.86$^{+2.36}_{-0.27}$ &  90.71$^{+19.45}_{-55.17}$ &  0.57$^{+0.40}_{-0.39}$ &   1.58$^{+0.37}_{-0.14}$ &       414$^{+5}_{-6}$ &      2.56$^{+1.62}_{-0.19}$ &  121.03 & 0.20 &            &          PC &        P16 \\
211978988.01 & K2-341 b &  2319.708694$^{+0.002195}_{-0.002083}$ &  36.552551$^{+0.000127}_{-0.000122}$ &   2.51$^{+0.17}_{-0.07}$ &   42.13$^{+3.55}_{-10.63}$ &  0.41$^{+0.32}_{-0.28}$ &   6.25$^{+0.17}_{-0.11}$ &     598$^{+16}_{-15}$ &      3.21$^{+0.25}_{-0.19}$ &   45.54 & 0.00 &            &          VP &        M18 \\
211987231.01 & &  2308.813645$^{+0.000170}_{-0.000172}$ &  17.035141$^{+0.000070}_{-0.000069}$ &  29.39$^{+3.60}_{-4.71}$ &    40.32$^{+0.36}_{-0.27}$ &  1.07$^{+0.04}_{-0.06}$ &   2.35$^{+0.02}_{-0.02}$ &     866$^{+30}_{-45}$ &     56.30$^{+8.74}_{-9.62}$ & 3162.20 & 0.99 &      LR,GB &          FP &        B16 \\
211995398.01 & &  2336.854100$^{+0.001240}_{-0.001254}$ &  32.579267$^{+0.000066}_{-0.000067}$ &  14.96$^{+0.50}_{-0.45}$ &    51.19$^{+4.75}_{-5.01}$ &  0.45$^{+0.15}_{-0.26}$ &   5.14$^{+0.17}_{-0.14}$ &     580$^{+28}_{-38}$ &     29.88$^{+3.95}_{-3.35}$ &   67.94 & 0.00 &         LR &          PC &        P16 \\
211997641.01 & &  3263.517490$^{+0.000156}_{-0.000099}$ &   1.744545$^{+0.000000}_{-0.000000}$ &  63.11$^{+8.98}_{-3.22}$ &     3.46$^{+0.15}_{-0.05}$ &  0.75$^{+0.13}_{-0.05}$ &   5.92$^{+0.08}_{-0.09}$ &  2534$^{+154}_{-178}$ &  179.37$^{+31.30}_{-24.23}$ & 8429.32 & 0.99 &         LR &          FP &        Y18 \\
212006318.01 & &  2314.327580$^{+0.006214}_{-0.007226}$ &  14.457821$^{+0.000149}_{-0.000146}$ &   1.41$^{+0.12}_{-0.07}$ &    15.20$^{+1.72}_{-4.36}$ &  0.44$^{+0.33}_{-0.30}$ &   6.65$^{+0.34}_{-0.33}$ &     936$^{+30}_{-34}$ &      2.41$^{+0.28}_{-0.20}$ &   33.81 & 0.02 &            &          PC &        P16 \\
212009150.01 & &  2312.162629$^{+0.002507}_{-0.002465}$ &   6.833191$^{+0.000022}_{-0.000021}$ &   5.60$^{+1.07}_{-0.37}$ &   40.03$^{+8.40}_{-18.34}$ &  0.49$^{+0.40}_{-0.34}$ &   1.22$^{+0.22}_{-0.15}$ &       344$^{+3}_{-4}$ &      1.47$^{+0.30}_{-0.11}$ &   49.97 & 0.10 &            &          PC &        K19 \\
212040382.01 & &  3266.349509$^{+0.000271}_{-0.000270}$ &   4.445602$^{+0.000028}_{-0.000029}$ &   7.32$^{+0.06}_{-0.07}$ &     6.54$^{+0.28}_{-0.23}$ &  0.68$^{+0.03}_{-0.04}$ &   4.37$^{+0.03}_{-0.04}$ &    1764$^{+74}_{-84}$ &     18.58$^{+1.97}_{-1.64}$ &  451.26 & 0.02 &         LR &          PC &        Y18 \\
212041476.01 & &  3262.559797$^{+0.001203}_{-0.001199}$ &   2.783676$^{+0.000073}_{-0.000072}$ &   2.03$^{+0.12}_{-0.06}$ &    14.50$^{+1.22}_{-3.43}$ &  0.40$^{+0.32}_{-0.27}$ &   1.38$^{+0.05}_{-0.04}$ &    1280$^{+22}_{-23}$ &      2.16$^{+0.14}_{-0.09}$ &   42.77 & 0.00 &        rho &          PC &        Y18 \\
212058012.01 & K2-342 b &  3266.107260$^{+0.002390}_{-0.002546}$ &  11.561052$^{+0.000690}_{-0.000668}$ &   1.55$^{+0.10}_{-0.04}$ &    21.96$^{+2.02}_{-5.36}$ &  0.42$^{+0.31}_{-0.29}$ &   3.73$^{+0.10}_{-0.08}$ &     861$^{+14}_{-15}$ &      2.03$^{+0.13}_{-0.09}$ &   37.15 & 0.01 &            &          VP &        Y18 \\
212072539.01 & K2-343 c &  2311.624554$^{+0.001285}_{-0.001309}$ &   7.676972$^{+0.000012}_{-0.000012}$ &   4.02$^{+0.19}_{-0.10}$ &    26.11$^{+1.88}_{-5.92}$ &  0.36$^{+0.33}_{-0.25}$ &   2.20$^{+0.08}_{-0.07}$ &       465$^{+7}_{-7}$ &      2.02$^{+0.10}_{-0.07}$ &   50.40 & 0.00 &            &          VP &        Y18 \\
212072539.02 & K2-343 b &  2308.324970$^{+0.001208}_{-0.001231}$ &   2.787174$^{+0.000004}_{-0.000004}$ &   3.29$^{+0.30}_{-0.11}$ &    13.47$^{+1.69}_{-4.14}$ &  0.48$^{+0.33}_{-0.32}$ &   1.46$^{+0.08}_{-0.05}$ &     653$^{+10}_{-12}$ &      1.65$^{+0.16}_{-0.08}$ &   62.62 & 0.04 &            &          VP &        K19 \\
212081533.01 & K2-344 b &  3262.747731$^{+0.001269}_{-0.001250}$ &   3.355850$^{+0.000091}_{-0.000093}$ &   2.95$^{+0.19}_{-0.09}$ &    13.79$^{+1.25}_{-3.53}$ &  0.41$^{+0.33}_{-0.28}$ &   1.76$^{+0.07}_{-0.05}$ &      722$^{+7}_{-10}$ &      1.59$^{+0.10}_{-0.05}$ &   43.44 & 0.00 &            &          VP &        Y18 \\
212088059.01 & K2-345 b &  2308.710348$^{+0.001423}_{-0.001468}$ &  10.367437$^{+0.000020}_{-0.000019}$ &   3.67$^{+0.35}_{-0.13}$ &   36.12$^{+3.76}_{-10.25}$ &  0.43$^{+0.34}_{-0.30}$ &   2.08$^{+0.11}_{-0.08}$ &       437$^{+4}_{-5}$ &      2.11$^{+0.20}_{-0.09}$ &   50.61 & 0.00 &            &          VP &        P16 \\
212132195.01 & K2-346 b &  2331.390197$^{+0.002081}_{-0.002164}$ &  26.201446$^{+0.003331}_{-0.003124}$ &   2.97$^{+0.25}_{-0.11}$ &   56.68$^{+5.27}_{-13.31}$ &  0.42$^{+0.31}_{-0.28}$ &   3.33$^{+0.12}_{-0.10}$ &       450$^{+5}_{-5}$ &      2.26$^{+0.19}_{-0.10}$ &   25.59 & 0.00 &            &          VP &        P16 \\
212161956.01 & K2-347 b &  2307.699277$^{+0.001927}_{-0.001812}$ &   7.187257$^{+0.000020}_{-0.000021}$ &   3.35$^{+0.09}_{-0.09}$ &    21.52$^{+0.37}_{-0.37}$ &  0.21$^{+0.13}_{-0.14}$ &   2.57$^{+0.06}_{-0.07}$ &     640$^{+20}_{-21}$ &      2.41$^{+0.11}_{-0.10}$ &   27.59 & 0.00 &            &          VP &        P16 \\
212178066.01 & &  3262.901443$^{+0.003040}_{-0.003115}$ &  15.611913$^{+0.000393}_{-0.000412}$ &   1.98$^{+0.15}_{-0.09}$ &    29.57$^{+3.14}_{-7.87}$ &  0.43$^{+0.32}_{-0.30}$ &   3.72$^{+0.16}_{-0.14}$ &       835$^{+8}_{-9}$ &      2.97$^{+0.29}_{-0.17}$ &   20.02 & 0.00 &  saturate &          PC &        Y18 \\
212204403.01 & K2-348 b &  3263.716772$^{+0.000995}_{-0.001053}$ &   4.688418$^{+0.000119}_{-0.000117}$ &   3.50$^{+0.25}_{-0.08}$ &    12.55$^{+0.93}_{-2.62}$ &  0.39$^{+0.30}_{-0.27}$ &   2.75$^{+0.07}_{-0.04}$ &     908$^{+12}_{-11}$ &      3.26$^{+0.22}_{-0.11}$ &   75.18 & 0.00 &            &          VP &        Y18 \\
212204403.02 & K2-348 c &  3271.435651$^{+0.003152}_{-0.003022}$ &  12.550171$^{+0.001018}_{-0.001057}$ &   2.87$^{+0.24}_{-0.11}$ &    24.47$^{+2.35}_{-6.03}$ &  0.43$^{+0.31}_{-0.30}$ &   3.68$^{+0.14}_{-0.11}$ &       655$^{+7}_{-9}$ &      2.67$^{+0.23}_{-0.11}$ &   28.30 & 0.00 &            &          VP &        Y18 \\
212278644.01 & &  2394.558248$^{+0.014831}_{-0.014570}$ &  12.421322$^{+0.005559}_{-0.004657}$ &   2.11$^{+0.27}_{-0.14}$ &    17.50$^{+3.29}_{-7.33}$ &  0.49$^{+0.38}_{-0.34}$ &   4.84$^{+0.64}_{-0.46}$ &     965$^{+34}_{-39}$ &      3.42$^{+0.60}_{-0.39}$ &   38.97 & 1.00 &            &          FP &        P16 \\
212297394.01 & K2-304 c & 2389.478879$^{+0.003648}_{-0.003472}$ &   5.213965$^{+0.000442}_{-0.000442}$ &   2.58$^{+0.18}_{-0.11}$ &    14.45$^{+1.25}_{-3.23}$ &  0.39$^{+0.32}_{-0.27}$ &   2.62$^{+0.11}_{-0.11}$ &     866$^{+27}_{-37}$ &      2.27$^{+0.19}_{-0.14}$ &   21.14 & 0.00 &            &          VP &        P16 \\
212297394.02 & K2-304 b &  2384.963190$^{+0.004892}_{-0.004738}$ &   2.289363$^{+0.000232}_{-0.000251}$ &   1.69$^{+0.12}_{-0.12}$ &     8.53$^{+1.18}_{-1.79}$ &  0.41$^{+0.29}_{-0.26}$ &   1.88$^{+0.17}_{-0.16}$ &    1149$^{+43}_{-44}$ &      1.48$^{+0.13}_{-0.11}$ &   11.89 &   -- &            &          KP &  H19 \\

\hline
\end{tabular}

==> K2 in Cancri and Virginis arxiv/tables/tab_planet_fpp3.tex <==
\renewcommand{\arraystretch}{1.5}
\begin{tabular}{lllllllllrrllll}
\hline
EPIC &          Name &               $T_{0}$ [BKJD] &                              $P$ [d] &      $R_p/R_{\star}$ [\%] &              $a/R_{\star}$ &                     $b$ &            $T_{14}$ [hr] &            \Teq [K] &             $R_p$ [\rearth] &     SNR &  FPP &  notes & disposition &           ref \\
\hline
212420823.01 & K2-349 b &  2386.127431$^{+0.003865}_{-0.003894}$ &   9.032178$^{+0.000874}_{-0.000874}$ &   2.55$^{+0.18}_{-0.12}$ &    19.99$^{+1.94}_{-4.52}$ &  0.40$^{+0.31}_{-0.27}$ &   3.25$^{+0.15}_{-0.14}$ &       518$^{+5}_{-4}$ &      1.38$^{+0.10}_{-0.07}$ &   23.75 & 0.00 &            &          VP &        P16 \\
212428509.01 & &  2386.832645$^{+0.000130}_{-0.000131}$ &   5.335929$^{+0.000001}_{-0.000001}$ &  23.57$^{+0.72}_{-1.28}$ &     8.66$^{+0.04}_{-0.04}$ &  1.08$^{+0.01}_{-0.02}$ &   2.84$^{+0.01}_{-0.01}$ &    1218$^{+28}_{-28}$ &     34.37$^{+2.11}_{-2.28}$ & 3989.14 & 0.99 &         LR &          FP &        P18 \\
212435047.01 & &  2385.443969$^{+0.002187}_{-0.002349}$ &   1.115494$^{+0.000063}_{-0.000061}$ &   1.26$^{+1.21}_{-0.08}$ &     4.33$^{+1.08}_{-2.98}$ &  0.62$^{+0.38}_{-0.42}$ &   1.65$^{+0.57}_{-0.14}$ &    1860$^{+33}_{-35}$ &      1.54$^{+1.49}_{-0.13}$ &  172.91 & 0.13 &            &          PC &        P16 \\
212440430.01 & K2-350 c &  2395.164968$^{+0.002851}_{-0.002858}$ &  19.991944$^{+0.000123}_{-0.000194}$ &   2.39$^{+0.20}_{-0.09}$ &    28.71$^{+2.95}_{-8.21}$ &  0.45$^{+0.33}_{-0.29}$ &   4.94$^{+0.19}_{-0.20}$ &     687$^{+16}_{-18}$ &      2.74$^{+0.25}_{-0.18}$ &   33.77 & 0.00 &            &          VP &        P16 \\
212440430.02 & K2-350 b &  2386.277628$^{+0.003444}_{-0.003308}$ &   4.163873$^{+0.000022}_{-0.000023}$ &   1.35$^{+0.10}_{-0.08}$ &    10.68$^{+1.20}_{-2.62}$ &  0.41$^{+0.32}_{-0.28}$ &   2.75$^{+0.16}_{-0.16}$ &    1158$^{+29}_{-34}$ &      1.54$^{+0.15}_{-0.11}$ &   16.67 & 0.00 &            &          VP &  This work \\
212495601.01 & &  2396.654065$^{+0.004748}_{-0.004464}$ &  21.674345$^{+0.000160}_{-0.000165}$ &   2.19$^{+0.15}_{-0.10}$ &    30.45$^{+2.90}_{-7.50}$ &  0.41$^{+0.32}_{-0.28}$ &   5.10$^{+0.22}_{-0.20}$ &     665$^{+16}_{-19}$ &      2.47$^{+0.21}_{-0.17}$ &   15.25 & 1.00 &            &          FP &        P16 \\
212543933.01 & K2-351 b &  2390.495191$^{+0.002614}_{-0.002604}$ &   7.806164$^{+0.000673}_{-0.000623}$ &   2.21$^{+0.13}_{-0.09}$ &    20.20$^{+1.80}_{-4.36}$ &  0.39$^{+0.30}_{-0.27}$ &   2.78$^{+0.12}_{-0.11}$ &     934$^{+28}_{-32}$ &      2.54$^{+0.25}_{-0.19}$ &   23.08 & 0.00 &            &          VP &        P16 \\
212570977.01 & &  2390.894185$^{+0.000333}_{-0.000329}$ &   8.853066$^{+0.000004}_{-0.000004}$ &  14.98$^{+0.20}_{-0.16}$ &    17.95$^{+0.60}_{-0.69}$ &  0.29$^{+0.11}_{-0.16}$ &   4.20$^{+0.05}_{-0.04}$ &     912$^{+32}_{-29}$ &     18.34$^{+1.22}_{-1.07}$ &  295.58 & 0.20 &         LR &          PC &        P16 \\
212587672.01 & K2-307 c &  2404.042492$^{+0.001902}_{-0.001818}$ &  23.228555$^{+0.000068}_{-0.000071}$ &   2.15$^{+0.17}_{-0.07}$ &   50.74$^{+5.07}_{-15.28}$ &  0.43$^{+0.35}_{-0.30}$ &   3.25$^{+0.13}_{-0.09}$ &     658$^{+13}_{-14}$ &      2.32$^{+0.19}_{-0.12}$ &   46.10 & 0.01 &            &          VP &        P16 \\
212587672.02 & K2-307 b &  2394.644991$^{+0.004543}_{-0.004448}$ &  15.280780$^{+0.000121}_{-0.000116}$ &   1.17$^{+0.09}_{-0.07}$ &    30.75$^{+3.74}_{-8.15}$ &  0.43$^{+0.33}_{-0.29}$ &   3.46$^{+0.20}_{-0.21}$ &     756$^{+14}_{-15}$ &      1.26$^{+0.11}_{-0.09}$ &   14.56 &   -- &            &          KP &  H19 \\
212628098.01 & &  2390.347813$^{+0.000248}_{-0.000257}$ &   4.352495$^{+0.000002}_{-0.000002}$ &  23.27$^{+1.27}_{-0.87}$ &    20.86$^{+1.34}_{-1.22}$ &  0.69$^{+0.07}_{-0.07}$ &   1.63$^{+0.05}_{-0.06}$ &     777$^{+11}_{-10}$ &     24.80$^{+1.81}_{-1.30}$ &  229.66 & 0.61 &         LR &          PC &        P18 \\
212628477.01 & &  3347.727411$^{+0.001377}_{-0.001341}$ &  15.423327$^{+0.000580}_{-0.000550}$ &  11.62$^{+1.08}_{-0.71}$ &  90.89$^{+11.67}_{-23.65}$ &  0.43$^{+0.33}_{-0.29}$ &   1.33$^{+0.16}_{-0.10}$ &     835$^{+18}_{-20}$ &     17.17$^{+1.98}_{-1.39}$ &   47.84 & 0.53 &         LR &          PC &  This work \\
212634172.01 & &  2384.597110$^{+0.000405}_{-0.000407}$ &   2.851687$^{+0.000002}_{-0.000002}$ &   6.39$^{+0.78}_{-0.19}$ &    27.20$^{+2.96}_{-8.99}$ &  0.44$^{+0.37}_{-0.31}$ &   0.78$^{+0.07}_{-0.04}$ &       555$^{+5}_{-5}$ &      2.75$^{+0.30}_{-0.11}$ &  198.53 & 0.19 &            &          PC &        K19 \\
212661144.01 & &  2385.909593$^{+0.001217}_{-0.001215}$ &   2.458749$^{+0.000004}_{-0.000004}$ &   2.81$^{+0.18}_{-0.10}$ &    14.78$^{+1.45}_{-3.74}$ &  0.40$^{+0.34}_{-0.28}$ &   1.20$^{+0.06}_{-0.06}$ &    1357$^{+60}_{-58}$ &      3.31$^{+0.30}_{-0.22}$ &   43.10 & 0.01 &            &          PC &        D17 \\
212690867.01 & &  2396.603761$^{+0.002469}_{-0.002550}$ &  25.856312$^{+0.000090}_{-0.000088}$ &   4.53$^{+0.26}_{-0.16}$ &   68.44$^{+6.84}_{-15.84}$ &  0.42$^{+0.30}_{-0.29}$ &   2.77$^{+0.14}_{-0.12}$ &       290$^{+3}_{-3}$ &      2.91$^{+0.18}_{-0.12}$ &   28.58 & 0.59 &            &          PC &        D17 \\
212797028.01 & &  2397.464819$^{+0.000578}_{-0.000580}$ &  29.982306$^{+0.000027}_{-0.000028}$ &  14.37$^{+0.15}_{-0.13}$ &    28.98$^{+0.41}_{-0.41}$ &  0.84$^{+0.01}_{-0.01}$ &   6.12$^{+0.06}_{-0.06}$ &     763$^{+26}_{-26}$ &     27.82$^{+2.08}_{-1.81}$ &  528.48 & 0.55 &         LR &          PC &        P18 \\
251319382.01 & K2-352 c &  3265.716929$^{+0.002711}_{-0.002885}$ &   8.234885$^{+0.000508}_{-0.000475}$ &   1.85$^{+0.12}_{-0.05}$ &    16.35$^{+1.46}_{-4.07}$ &  0.41$^{+0.32}_{-0.28}$ &   3.59$^{+0.11}_{-0.09}$ &     885$^{+12}_{-14}$ &      1.92$^{+0.13}_{-0.07}$ &   54.86 & 0.00 &            &          VP &        Y18 \\
251319382.02 & K2-352 d &  3270.622842$^{+0.002276}_{-0.002256}$ &  14.871387$^{+0.000916}_{-0.000936}$ &   2.14$^{+0.12}_{-0.06}$ &    25.94$^{+2.11}_{-5.93}$ &  0.39$^{+0.31}_{-0.27}$ &   4.14$^{+0.11}_{-0.09}$ &     727$^{+10}_{-10}$ &      2.23$^{+0.13}_{-0.09}$ &   36.20 & 0.00 &            &          VP &        Y18 \\
251319382.03 & K2-352 b &  3265.635282$^{+0.003388}_{-0.003276}$ &   3.665912$^{+0.000273}_{-0.000295}$ &   1.32$^{+0.10}_{-0.06}$ &    15.66$^{+2.02}_{-4.09}$ &  0.42$^{+0.33}_{-0.29}$ &   1.63$^{+0.12}_{-0.11}$ &    1160$^{+16}_{-15}$ &      1.37$^{+0.10}_{-0.07}$ &   20.01 & 0.04 &            &          VP &  This work \\
251554286.01 & K2-353 b &  3356.851818$^{+0.000977}_{-0.000988}$ &  15.466805$^{+0.000572}_{-0.000565}$ &   5.03$^{+0.11}_{-0.09}$ &    25.06$^{+0.61}_{-0.61}$ &  0.77$^{+0.02}_{-0.02}$ &   3.39$^{+0.07}_{-0.06}$ &     735$^{+13}_{-14}$ &      5.55$^{+0.22}_{-0.20}$ &   74.92 & 0.00 &            &          VP &  This work \\
\hline
\end{tabular}

==> K2 in Cancri and Virginis arxiv/tables/tab_star1.tex <==
%phot_spec_parallax
% \begin{tabular}{llllllrlrr}
\begin{tabular}{cccccccccc}
\hline
EPIC &          \rstar [\rsun] &          \mstar [\msun] &             \teff [K] &             \logg [cgs] &                \feh [dex] &  $K_p$ [mag] &  $\pi$ [mas] &  $\verb|GOF_AL|^a$ &  $\verb|D|^b$ \\
\hline
211314705 &  0.41$^{+0.01}_{-0.01}$ &  0.43$^{+0.01}_{-0.01}$ &    3669$^{+88}_{-82}$ &  4.86$^{+0.01}_{-0.01}$ &   -0.04$^{+0.2}_{-0.24}$ &    14.38 &        10.87 &    6.67 &    6.44 \\
211335816 &  1.65$^{+0.08}_{-0.07}$ &  1.29$^{+0.05}_{-0.05}$ &  6236$^{+140}_{-138}$ &  4.12$^{+0.04}_{-0.04}$ &   0.03$^{+0.09}_{-0.08}$ &    11.94 &         1.86 &    3.93 &    0.00 \\
211336288 &  0.56$^{+0.01}_{-0.01}$ &  0.58$^{+0.01}_{-0.01}$ &    4052$^{+42}_{-38}$ &   4.7$^{+0.01}_{-0.01}$ &  -0.07$^{+0.07}_{-0.07}$ &    14.56 &         4.95 &   -2.44 &    0.00 \\
211357309 &  0.44$^{+0.01}_{-0.01}$ &  0.47$^{+0.01}_{-0.01}$ &    4134$^{+60}_{-51}$ &  4.82$^{+0.01}_{-0.01}$ &   -0.9$^{+0.11}_{-0.15}$ &    13.08 &        14.49 &   15.83 &   13.48 \\
211383821 &  0.62$^{+0.01}_{-0.01}$ &  0.64$^{+0.01}_{-0.01}$ &    4343$^{+46}_{-45}$ &  4.65$^{+0.01}_{-0.01}$ &  -0.11$^{+0.07}_{-0.07}$ &    14.02 &         4.34 &   -3.23 &    0.00 \\
211399359 &  0.76$^{+0.02}_{-0.02}$ &  0.82$^{+0.02}_{-0.02}$ &    5000$^{+76}_{-71}$ &  4.58$^{+0.02}_{-0.03}$ &   0.03$^{+0.05}_{-0.06}$ &    14.39 &         2.23 &   -0.97 &    0.00 \\
211401787 &   1.5$^{+0.03}_{-0.03}$ &  1.23$^{+0.02}_{-0.02}$ &    6232$^{+33}_{-39}$ &  4.18$^{+0.02}_{-0.02}$ &  -0.03$^{+0.03}_{-0.03}$ &     9.51 &         6.22 &    9.52 &    0.00 \\
211413752 &  0.78$^{+0.02}_{-0.02}$ &  0.84$^{+0.02}_{-0.02}$ &    5106$^{+70}_{-61}$ &  4.58$^{+0.02}_{-0.03}$ &   0.03$^{+0.05}_{-0.05}$ &    13.56 &         3.02 &   -5.01 &    0.00 \\
211439059 &  0.85$^{+0.05}_{-0.03}$ &   0.9$^{+0.03}_{-0.03}$ &    5472$^{+85}_{-93}$ &  4.54$^{+0.03}_{-0.05}$ &  -0.01$^{+0.06}_{-0.06}$ &    13.03 &         3.04 &  264.08 & 5704.41 \\
211490999 &  0.94$^{+0.04}_{-0.04}$ &  0.91$^{+0.03}_{-0.03}$ &    5543$^{+80}_{-78}$ &  4.45$^{+0.05}_{-0.04}$ &  -0.01$^{+0.05}_{-0.05}$ &    13.44 &         2.13 &   -3.42 &    0.00 \\
211502222 &  1.06$^{+0.03}_{-0.02}$ &   1.1$^{+0.03}_{-0.04}$ &    5994$^{+93}_{-91}$ &  4.43$^{+0.02}_{-0.03}$ &   0.08$^{+0.08}_{-0.08}$ &    11.19 &         4.70 &   13.25 &    0.00 \\
211578235 &   1.15$^{+0.1}_{-0.08}$ &   0.9$^{+0.02}_{-0.02}$ &    5653$^{+55}_{-54}$ &  4.27$^{+0.06}_{-0.07}$ &  -0.12$^{+0.05}_{-0.05}$ &    14.33 &         1.28 &   -3.91 &    0.00 \\
211579112 &  0.28$^{+0.02}_{-0.01}$ &  0.27$^{+0.01}_{-0.02}$ &  3315$^{+137}_{-152}$ &  4.97$^{+0.03}_{-0.03}$ &   0.09$^{+0.15}_{-0.17}$ &    16.48 &         8.09 &    5.06 &    4.50 \\
211611158 &  0.94$^{+0.03}_{-0.03}$ &  0.96$^{+0.05}_{-0.07}$ &  5788$^{+190}_{-157}$ &  4.48$^{+0.03}_{-0.04}$ &    -0.1$^{+0.16}_{-0.2}$ &    12.06 &         3.70 &    8.70 &    0.00 \\
211645912 &  0.97$^{+0.03}_{-0.03}$ &  1.03$^{+0.03}_{-0.03}$ &    5892$^{+73}_{-71}$ &  4.48$^{+0.02}_{-0.03}$ &    0.0$^{+0.05}_{-0.05}$ &    12.47 &         2.84 &    3.36 &    0.00 \\
211647930 &  1.22$^{+0.05}_{-0.05}$ &  1.06$^{+0.04}_{-0.04}$ &    5880$^{+85}_{-82}$ &  4.29$^{+0.04}_{-0.04}$ &   0.07$^{+0.07}_{-0.07}$ &    11.99 &         2.88 &    4.93 &    0.00 \\
211730024 &  1.49$^{+0.07}_{-0.06}$ &  1.36$^{+0.05}_{-0.05}$ &  6502$^{+132}_{-130}$ &  4.22$^{+0.04}_{-0.04}$ &     0.17$^{+0.1}_{-0.1}$ &    11.35 &         2.66 &   13.35 &    1.92 \\
211743874 &  1.33$^{+0.07}_{-0.06}$ &  1.23$^{+0.04}_{-0.04}$ &    6222$^{+96}_{-91}$ &  4.28$^{+0.04}_{-0.04}$ &    0.1$^{+0.05}_{-0.05}$ &    12.47 &         1.76 &    3.08 &    0.00 \\
211762841 &  0.61$^{+0.01}_{-0.01}$ &  0.63$^{+0.02}_{-0.01}$ &    4079$^{+50}_{-48}$ &  4.68$^{+0.01}_{-0.01}$ &   0.13$^{+0.07}_{-0.07}$ &    14.79 &         4.14 &    0.58 &    0.00 \\
211763214 &   0.8$^{+0.01}_{-0.01}$ &  0.86$^{+0.03}_{-0.05}$ &  5424$^{+192}_{-144}$ &  4.56$^{+0.02}_{-0.03}$ &   -0.17$^{+0.16}_{-0.2}$ &    12.51 &         4.15 &    5.57 &    0.00 \\
211770696 &  1.32$^{+0.06}_{-0.06}$ &  0.94$^{+0.04}_{-0.03}$ &    5869$^{+88}_{-81}$ &  4.17$^{+0.04}_{-0.04}$ &  -0.27$^{+0.06}_{-0.06}$ &    12.23 &         2.34 &    4.06 &    0.00 \\
211779390 &  0.63$^{+0.01}_{-0.01}$ &  0.66$^{+0.02}_{-0.02}$ &    4558$^{+91}_{-81}$ &  4.65$^{+0.01}_{-0.01}$ &  -0.23$^{+0.12}_{-0.13}$ &    13.05 &         6.34 &    0.18 &    0.00 \\
211796070 &  0.89$^{+0.03}_{-0.03}$ &  0.15$^{+0.05}_{-0.03}$ &    4134$^{+88}_{-68}$ &   3.7$^{+0.15}_{-0.13}$ &  -2.93$^{+0.26}_{-0.25}$ &    13.88 &         3.68 &   -4.15 &    0.00 \\
211797637 &  0.78$^{+0.02}_{-0.03}$ &  0.17$^{+0.06}_{-0.04}$ &    4144$^{+93}_{-74}$ &  3.88$^{+0.16}_{-0.14}$ &  -2.78$^{+0.31}_{-0.26}$ &    13.69 &         4.49 &   -7.90 &    0.00 \\
211799258 &  0.44$^{+0.01}_{-0.01}$ &  0.47$^{+0.01}_{-0.01}$ &    3699$^{+66}_{-74}$ &  4.82$^{+0.01}_{-0.01}$ &   0.04$^{+0.17}_{-0.16}$ &    15.91 &         5.49 &    8.06 &    7.94 \\
211800191 &  1.22$^{+0.06}_{-0.05}$ &  0.94$^{+0.05}_{-0.04}$ &  5929$^{+120}_{-112}$ &  4.24$^{+0.04}_{-0.04}$ &  -0.28$^{+0.06}_{-0.06}$ &    12.44 &         2.47 &    5.03 &    0.00 \\
211817229 &    0.16$^{+0.0}_{-0.0}$ &    0.14$^{+0.0}_{-0.0}$ &    3246$^{+32}_{-37}$ &  5.17$^{+0.01}_{-0.01}$ &  -0.23$^{+0.06}_{-0.06}$ &    15.49 &        23.29 &   20.31 &   31.01 \\
211843564 &  0.59$^{+0.02}_{-0.02}$ &  0.61$^{+0.02}_{-0.02}$ &    3944$^{+42}_{-43}$ &  4.69$^{+0.02}_{-0.02}$ &   0.22$^{+0.13}_{-0.13}$ &    16.05 &         2.62 &   21.12 &   35.81 \\
211897691 &  0.72$^{+0.03}_{-0.03}$ &  0.74$^{+0.04}_{-0.03}$ &    4857$^{+86}_{-84}$ &  4.59$^{+0.02}_{-0.02}$ &  -0.11$^{+0.14}_{-0.14}$ &    14.34 &         2.75 &   -4.78 &    0.00 \\
211923431 &   1.13$^{+0.14}_{-0.1}$ &  0.93$^{+0.04}_{-0.04}$ &    5532$^{+90}_{-90}$ &   4.3$^{+0.07}_{-0.09}$ &   0.08$^{+0.13}_{-0.14}$ &    14.13 &         1.33 &   -3.26 &    0.00 \\
211939692 &  1.39$^{+0.06}_{-0.06}$ &  1.34$^{+0.08}_{-0.09}$ &  6806$^{+411}_{-293}$ &  4.28$^{+0.04}_{-0.05}$ &  -0.06$^{+0.17}_{-0.22}$ &    11.72 &         2.42 &    6.15 &    0.00 \\
211965883 &  0.61$^{+0.01}_{-0.01}$ &  0.63$^{+0.02}_{-0.01}$ &    4314$^{+50}_{-47}$ &  4.67$^{+0.01}_{-0.01}$ &  -0.14$^{+0.07}_{-0.07}$ &    14.09 &         4.74 &    0.02 &    0.00 \\
211978988 &  1.16$^{+0.06}_{-0.05}$ &  0.98$^{+0.07}_{-0.07}$ &    5817$^{+45}_{-48}$ &   4.3$^{+0.05}_{-0.05}$ &  -0.05$^{+0.18}_{-0.18}$ &    12.56 &         2.34 &    2.37 &    0.00 \\
211987231 &  1.46$^{+0.15}_{-0.12}$ &  1.11$^{+0.09}_{-0.07}$ &  5980$^{+118}_{-133}$ &  4.16$^{+0.07}_{-0.07}$ &  -0.01$^{+0.08}_{-0.09}$ &    11.89 &         2.60 &   50.13 &   99.62 \\
211995398 &  1.16$^{+0.15}_{-0.13}$ &  0.13$^{+0.03}_{-0.02}$ &    3921$^{+91}_{-83}$ &  3.43$^{+0.08}_{-0.09}$ &  -2.17$^{+0.29}_{-0.29}$ &    16.70 &         1.33 &    1.78 &    1.06 \\
211997641 &  2.54$^{+0.35}_{-0.28}$ &  1.65$^{+0.15}_{-0.16}$ &  6591$^{+338}_{-304}$ &  3.84$^{+0.08}_{-0.09}$ &   0.07$^{+0.16}_{-0.17}$ &    12.87 &         0.96 &   13.09 &    3.46 \\
212006318 &   1.56$^{+0.11}_{-0.1}$ &  1.11$^{+0.07}_{-0.05}$ &    5891$^{+89}_{-88}$ &   4.1$^{+0.05}_{-0.05}$ &   0.03$^{+0.06}_{-0.06}$ &    12.96 &         1.41 &    6.10 &    0.00 \\
212009150 &  0.24$^{+0.01}_{-0.01}$ &  0.22$^{+0.01}_{-0.01}$ &    3293$^{+46}_{-45}$ &  5.03$^{+0.01}_{-0.01}$ &   0.02$^{+0.05}_{-0.06}$ &    16.28 &         9.92 &    8.93 &    8.91 \\
212036875 &  1.47$^{+0.05}_{-0.05}$ &  1.22$^{+0.02}_{-0.02}$ &    6394$^{+57}_{-51}$ &  4.19$^{+0.02}_{-0.02}$ &  -0.21$^{+0.03}_{-0.03}$ &    10.91 &         3.23 &   12.44 &    1.37 \\
212040382 &   2.33$^{+0.25}_{-0.2}$ &  1.32$^{+0.11}_{-0.07}$ &  6310$^{+146}_{-141}$ &  3.83$^{+0.07}_{-0.07}$ &  -0.21$^{+0.13}_{-0.12}$ &    12.51 &         1.05 &    4.56 &    0.00 \\
212041476 &  0.97$^{+0.03}_{-0.03}$ &  1.01$^{+0.03}_{-0.04}$ &    5791$^{+74}_{-78}$ &  4.47$^{+0.03}_{-0.03}$ &   0.03$^{+0.06}_{-0.06}$ &    12.09 &         3.60 &    8.84 &    0.00 \\
212058012 &  1.09$^{+0.03}_{-0.03}$ &  1.01$^{+0.05}_{-0.05}$ &  5920$^{+104}_{-104}$ &  4.36$^{+0.03}_{-0.03}$ &  -0.06$^{+0.08}_{-0.09}$ &    11.07 &         4.77 &   12.98 &    0.00 \\
212066407 &   2.0$^{+0.18}_{-0.16}$ &   1.2$^{+0.07}_{-0.06}$ &    5943$^{+88}_{-87}$ &  3.92$^{+0.05}_{-0.05}$ &  -0.08$^{+0.06}_{-0.05}$ &    12.27 &         1.07 &   40.79 &   48.41 \\
212072539 &  0.46$^{+0.01}_{-0.01}$ &  0.49$^{+0.01}_{-0.01}$ &    3804$^{+93}_{-74}$ &   4.8$^{+0.01}_{-0.01}$ &   -0.1$^{+0.18}_{-0.25}$ &    15.13 &         5.99 &    2.77 &    0.69 \\
212081533 &  0.49$^{+0.01}_{-0.01}$ &  0.51$^{+0.01}_{-0.01}$ &    4374$^{+38}_{-34}$ &  4.76$^{+0.01}_{-0.01}$ &  -0.95$^{+0.02}_{-0.02}$ &    12.74 &        13.27 &    7.29 &    0.00 \\
212088059 &  0.52$^{+0.01}_{-0.01}$ &  0.56$^{+0.01}_{-0.01}$ &    3779$^{+30}_{-26}$ &  4.74$^{+0.01}_{-0.01}$ &   0.26$^{+0.07}_{-0.07}$ &    14.70 &         6.13 &    4.22 &    2.45 \\
212099230 &  0.98$^{+0.02}_{-0.02}$ &   0.9$^{+0.03}_{-0.02}$ &    5469$^{+63}_{-57}$ &   4.4$^{+0.02}_{-0.02}$ &   0.05$^{+0.08}_{-0.08}$ &    10.52 &         8.06 &   10.17 &    0.00 \\
212132195 &   0.7$^{+0.01}_{-0.01}$ &  0.71$^{+0.02}_{-0.02}$ &    4801$^{+49}_{-49}$ &   4.6$^{+0.01}_{-0.01}$ &  -0.18$^{+0.08}_{-0.08}$ &    11.68 &         9.44 &    4.98 &    0.00 \\
212161956 &  0.63$^{+0.02}_{-0.02}$ &  0.66$^{+0.03}_{-0.03}$ &  4599$^{+178}_{-152}$ &  4.65$^{+0.02}_{-0.02}$ &  -0.26$^{+0.17}_{-0.21}$ &    14.81 &         3.09 &   -1.92 &    0.00 \\
212178066 &   1.2$^{+0.02}_{-0.01}$ &   1.2$^{+0.04}_{-0.04}$ &    6243$^{+89}_{-94}$ &  4.36$^{+0.02}_{-0.02}$ &   0.08$^{+0.08}_{-0.08}$ &     6.75 &        28.33 &   10.59 &    0.00 \\
212204403 &  0.85$^{+0.02}_{-0.02}$ &  0.83$^{+0.02}_{-0.01}$ &    5077$^{+40}_{-39}$ &   4.5$^{+0.02}_{-0.01}$ &   0.13$^{+0.05}_{-0.05}$ &    12.33 &         4.93 &    6.94 &    0.00 \\
212278644 &  1.47$^{+0.14}_{-0.13}$ &  1.14$^{+0.06}_{-0.05}$ &    5978$^{+64}_{-65}$ &  4.16$^{+0.07}_{-0.07}$ &   0.03$^{+0.02}_{-0.02}$ &    14.00 &         1.04 &   -1.75 &    0.00 \\
212297394 &   0.8$^{+0.03}_{-0.03}$ &  0.83$^{+0.05}_{-0.04}$ &  5171$^{+172}_{-130}$ &  4.55$^{+0.03}_{-0.03}$ &  -0.03$^{+0.15}_{-0.16}$ &    14.19 &         2.36 &   -2.45 &    0.00 \\
212420823 &    0.49$^{+0.0}_{-0.0}$ &  0.54$^{+0.01}_{-0.01}$ &    4385$^{+29}_{-31}$ &  4.78$^{+0.01}_{-0.01}$ &  -0.66$^{+0.04}_{-0.04}$ &    14.18 &         2.18 &   -3.28 &    0.00 \\
212428509 &  1.29$^{+0.06}_{-0.06}$ &  0.88$^{+0.03}_{-0.02}$ &    5834$^{+68}_{-54}$ &  4.17$^{+0.04}_{-0.04}$ &  -0.37$^{+0.06}_{-0.06}$ &    12.57 &         2.24 &    2.34 &    0.00 \\
212435047 &   1.1$^{+0.04}_{-0.04}$ &  1.01$^{+0.04}_{-0.04}$ &    5842$^{+85}_{-81}$ &  4.36$^{+0.04}_{-0.04}$ &   0.01$^{+0.06}_{-0.06}$ &    12.35 &         2.74 &    4.57 &    0.00 \\
212440430 &  1.04$^{+0.06}_{-0.05}$ &  0.98$^{+0.02}_{-0.02}$ &    5789$^{+46}_{-50}$ &  4.39$^{+0.05}_{-0.04}$ &  -0.02$^{+0.03}_{-0.03}$ &    13.31 &         2.01 &   -2.14 &    0.00 \\
212495601 &  1.03$^{+0.05}_{-0.05}$ &  0.87$^{+0.02}_{-0.01}$ &    5666$^{+46}_{-47}$ &  4.35$^{+0.04}_{-0.04}$ &  -0.19$^{+0.02}_{-0.02}$ &    13.82 &         1.59 &   -2.90 &    0.00 \\
\hline
\end{tabular}


==> K2 in Cancri and Virginis arxiv/tables/tab_star2.tex <==
% \begin{tabular}{llllllrlrr}
\begin{tabular}{cccccccccc}
\hline
EPIC &          \rstar [\rsun] &          \mstar [\msun] &             \teff [K] &             \logg [cgs] &                \feh [dex] &  $K_p$ [mag] &  $\pi$ [mas] &  $\verb|GOF_AL|^a$ &  $\verb|D|^b$ \\
\hline
212543933 &  1.05$^{+0.07}_{-0.06}$ &  1.02$^{+0.02}_{-0.02}$ &    5769$^{+39}_{-37}$ &   4.4$^{+0.06}_{-0.06}$ &   0.08$^{+0.02}_{-0.02}$ &    13.99 &         1.41 &   -2.83 &    0.00 \\
212570977 &  1.12$^{+0.07}_{-0.06}$ &  1.05$^{+0.04}_{-0.04}$ &    5698$^{+87}_{-91}$ &  4.36$^{+0.06}_{-0.05}$ &   0.24$^{+0.05}_{-0.05}$ &    13.94 &         1.40 &   -2.37 &    0.00 \\
212587672 &  0.98$^{+0.04}_{-0.03}$ &  0.99$^{+0.03}_{-0.04}$ &    6004$^{+77}_{-78}$ &  4.45$^{+0.03}_{-0.04}$ &  -0.18$^{+0.06}_{-0.06}$ &    12.20 &         3.10 &    3.61 &    0.00 \\
212628098 &  0.88$^{+0.03}_{-0.03}$ &  0.77$^{+0.02}_{-0.03}$ &   4109$^{+85}_{-115}$ &  4.44$^{+0.03}_{-0.05}$ &  -0.01$^{+0.09}_{-0.09}$ &    13.47 &         4.67 &   -5.25 &    0.00 \\
212628477 &  1.35$^{+0.07}_{-0.06}$ &    1.0$^{+0.2}_{-0.06}$ &    5715$^{+95}_{-97}$ &   4.2$^{+0.03}_{-0.04}$ &  -0.09$^{+0.07}_{-0.07}$ &    12.62 &         2.35 &    1.58 &    0.00 \\
212634172 &  0.39$^{+0.01}_{-0.01}$ &  0.41$^{+0.01}_{-0.01}$ &    3431$^{+41}_{-48}$ &  4.86$^{+0.01}_{-0.01}$ &   0.32$^{+0.08}_{-0.07}$ &    15.26 &         9.89 &   12.53 &   15.65 \\
212639319 &  2.56$^{+0.22}_{-0.18}$ &  1.39$^{+0.08}_{-0.07}$ &    5456$^{+95}_{-93}$ &  3.77$^{+0.04}_{-0.05}$ &   0.26$^{+0.05}_{-0.05}$ &    12.42 &         1.29 &   15.23 &    4.68 \\
212661144 &   1.0$^{+0.06}_{-0.05}$ &  0.96$^{+0.08}_{-0.07}$ &  5749$^{+206}_{-191}$ &  4.43$^{+0.05}_{-0.06}$ &  -0.03$^{+0.17}_{-0.19}$ &    13.74 &         1.86 &   -3.08 &    0.00 \\
212690867 &  0.41$^{+0.01}_{-0.01}$ &  0.43$^{+0.01}_{-0.01}$ &    3713$^{+37}_{-37}$ &  4.85$^{+0.01}_{-0.01}$ &  -0.13$^{+0.09}_{-0.09}$ &    15.30 &         6.34 &    3.76 &    1.88 \\
212797028 &  1.77$^{+0.13}_{-0.11}$ &  1.14$^{+0.05}_{-0.05}$ &    5767$^{+87}_{-78}$ &   4.0$^{+0.05}_{-0.05}$ &    0.1$^{+0.06}_{-0.06}$ &    13.11 &         1.15 &   -2.08 &    0.00 \\
251319382 &  0.95$^{+0.02}_{-0.02}$ &  0.98$^{+0.04}_{-0.04}$ &    5791$^{+81}_{-81}$ &  4.47$^{+0.03}_{-0.03}$ &  -0.05$^{+0.07}_{-0.07}$ &    11.11 &         5.65 &   16.02 &    7.46 \\
251554286 &  0.99$^{+0.03}_{-0.03}$ &  0.87$^{+0.02}_{-0.02}$ &    5698$^{+55}_{-55}$ &  4.38$^{+0.03}_{-0.03}$ &  -0.21$^{+0.04}_{-0.04}$ &    12.10 &         3.70 &    2.84 &    0.00 \\
%212099230
\hline
\end{tabular}

==> scratch.tex <==
\subsubsection{EPIC 211897691}
\begin{itemize}
    \item 2 planets with short and long periods but similar radius (~2 Rearth)
    \item low SNR and \vespa computed FPP=85\% for both candidates
    \item active star in 3 campaigns
\end{itemize}

\subsubsection{EPIC 212072539}
\begin{itemize}
    \item outer candidate by \citet{2018YuC16} and inner candidate by \citet{2019KruseC0to8}
    \item outer candidate is hi SNR but the outer is low and a bit V-shaped and hence \vespa computed FPP=95\%
    \item in 3 campaigns but C16 lc is bad
\end{itemize}

\subsubsection{EPIC 212555594}
\begin{itemize}
    \item CP accdg to exofop by \citet{2018MayoC1to10} but there is another candidate by \citet{2018PetiguraC5to8} but identical period
\end{itemize}

\subsubsection{Multi-planet system within the radius valley}
%\subsubsection{EPIC 211988320}
EPIC 211988320 has two planets straddling the radius valley \citep[1.5<\Rp<2.0;][]{2017FultonGap} with periods of 6.79 and 18.52 d.  %reminiscent of Davide's planets? 
The outer planet was detected by \cite{2019KruseC0to8} and \citet{2017DressingC1to7planets} while the inner planet is a new candidate validated in this work.
The other planet is actually larger than Rp>2Re

\begin{figure*}
    \includegraphics[clip,trim={0 0 0 0},width=1\textwidth]{fig_effect_of_parallax.png}
    \caption{Assessment of the impact of parallax on the stellar parameters used in this work. The red and blue points correspond to stars with (8 out of \numvp in our sample) and without high resolution optical or medium resolution NIR spectroscopic constraints, respectively (see \S\ref{sec:spec}). 
    The x/y-axes correspond to the value of each stellar parameter before/after incorporating parallaxes from Gaia DR2, and the dashed gray lines indicate the line y = x for reference. Without parallax information, two stars in our sample are confused as bright, faraway evolved giants when in fact they are faint, nearby dwarf stars.}
    \label{fig:parallax}
\end{figure*}

There are 14 muti-planetary system candidates in Cancri & Virginis constellations.
There are 54 nexsci PC with spec+imaging obs from exofop

@MISC{2016NewvilleLMFit,
  organisation = {{Newville}, M. and {Stensitzki}, T. and {Allen}, D.~B. and {Rawlik}, M. and 
	{Ingargiola}, A. and {Nelson}, A.},
    title = "{Lmfit: Non-Linear Least-Square Minimization and Curve-Fitting for Python}",
 keywords = {Software},
howpublished = {Astrophysics Source Code Library},
     year = 2016,
    month = jun,
archivePrefix = "ascl",
  eprint = {1606.014},
  adsurl = {http://adsabs.harvard.edu/abs/2016ascl.soft06014N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

\subsection{Host star properties}
planets in early type stars are rare
thin or thick disk origin?
The thin disc is vertically thin (Bovy et al. 2012; Haywood et al. 2013), rotation dominated (Edvardsson et al. 1993; Rix \& Bovy 2013), has a metallicity range of $-0.7 < \feh < +0.5$ dex (Bensby et al. 2014), and has ongoing star formation.  
The thick disc (Yoshii 1982; Gilmore \& Reid 1983) has larger vertical scale-heights but smaller radial scale-lengths than the thin disc (Bovy et al. 2012; Haywood et al. 2013; Hayden et al. 2015), and has rotation but also higher velocity dispersion (Haywood et al. 2013; Kordopatis et al. 2013b). It is also chemically different than the thin disc, having lower metallicities and higher [$\alpha$/Fe] (Edvardsson et al. 1993; Bensby et al. 2003; Kordopatis et al. 2013b; Nidever et al. 2014), pointing to a scenario where it is older than the thin disc.
Alpha elements (O, Mg, Si, S, Ca) are dispersed into the interstellar medium due to core-collapse supernova (SN II). However, [α/Fe] goes down with time as supernova Type Ia (SNe Ia) events start to happen that contribute more Fe. Stars with enhanced [α/Fe] are formed from gas that was enriched primarily by core-collapse supernovae. Therefore, [α/Fe] is indicative of a stellar populations’ star formation history, with stars having high [α/Fe] being older, on average

Recon Spectroscopy to identify astrophysical false positives and to contribute to improved stellar parameters for the host star in those cases where the uncertainty in the planetary mass and radius is limited by the  uncertainties in the mass and radius of the host star. Recon spectroscopy can identify eclipsing binaries that masquerade as transiting planets by revealing large velocity variations due to an orbiting stellar companion consistent with the photometric ephemeris from TESS. Blends of a target star with a nearby (usually fainter) eclipsing binary that is not spatially resolved can show composite spectra where the orbit of the contaminating eclipsing binary is consistent with the photometric ephemeris from TESS. These are but two examples of the false positives revealed by Recon Spectroscopy. Spectroscopic determinations of effective temperature, surface gravity, and metallicity can often contribute to improved estimates of the mass and radius of the host star, when analyzed with the help of stellar models or empirical relations

SED: We retrieved archival photometry for each target by cross-matching our sample against sources from the Howell-Everett (HE, Everett et al. 2012), Sloan Digitial Sky Survey (SDSS, Ahn et al. 2012), Two-Micron All-sky Survey (2MASS, Skrutskie et al. 2006), and Wide-field Infrared Survey Explorer (WISE, Cutri & et al. 2014) catalogues on Vizier using a 2' search cone  to construct SEDs, excluding targets which had fewer than five photometric data points.

\begin{figure*}
    \includegraphics[clip,trim={0 0 0 0},width=0.8\textwidth]{epic212297394_plots.pdf}
    \caption{Phase-folded plots of two planet candidates detected in EPIC 21227394 with \Porb of 2.29 d and 5.21 d.}
    \label{fig:lc}
\end{figure*}

\subsubsection{EPIC 211314705}
This target was observed in K2/C5 and we detected the signal in both \everest and \ktwosff light curves. \panstarrs images rule out potential nearby EB within the photometric aperture and our AO and speckle images further extend the constraint down to within a few arcseconds. We obtained an FPP<1\% using \vespa which rule out remaining false positive scenarios not constrained by our observations and hence the planet is validated.

\subsubsection{EPIC 211579112}
This target was observed in K2/C5 \& C18 and we detected the transits in both campaigns. \citet{2019KruseC0to8} detected the \Porb$=$17.7 d candidate using C5 light curve only and reported that the \Rp$=1.46\pm0.11$ candidate is near or within the habitable zone. \panstarrs show a faint nearby star which we ruled out as a potential nearby EB in \S \ref{sec:dilution}. Our AO and speckle contrast curves further extend the constraint down to within a few arcseconds. We obtained an FPP<1\% using \vespa which rule out remaining false positive scenarios not constrained by our observations and hence the planet is validated.

\subsubsection{EPIC 211763214}
This target was observed in K2/C5, C16, and C18 but we did not detect the \Porb$=$21.2 d candidate in the last campaign due to relatively high scattering in the light curve. Only light curve in C5 was previously analyzed by \citet{2019KruseC0to8} and \citet{2018MayoC1to10} so we added C16 data in this work. \citet{2018MayoC1to10} did not validate the candidate due to the lack of AO imaging data despite the reported very low FPP$=$0.5\%. Our AO and speckle images show no companions which enable us to finally validate the planet.

We also cross-matched the host star with the TIC-Gaia catalog \citet{2020CarilloTGv8} which provide a 95\% probability for the star to be in the thin-disc similar to the majority of known host stars.

\subsubsection{EPIC 211965883}
This target was previously analyzed by \citet{2017DressingC1to7planets} who reported the candidate with \Porb$=$10.55422 d 
%\Rp$=$2.86$\pm$0.28 \rearth using \rstar$=$0.60$\pm$0.03 \rsun 
but did not validate it due to the large FPP$=$34\%.
%\citet{2019KruseC0to8} derived a smaller radius, \Rp=1.33$^{+0.13}_{-0.29}$ \Rearth, as a result of larger but imprecise adopted stellar radius, $\Rstar=0.66$ from \gaia DR2.
We found no contaminating stars within the photometric aperture as well as close to the target using our AO and speckle images. We recomputed the FPP using these constraints which resulted to FPP<1\% and hence the planet is validated.

\subsubsection{EPIC 212088059}
This target was observed in K2/C5, C16, \& C18 and we detected the \Porb$=$10.4 d candidate in both \everest and \ktwosff light curves. \panstarrs images show a faint source within the aperture but our analysis in \S \ref{sec:dilution} rule out the nearby source as potential nearby EB. Also, our AO and speckle contrast curves further extend the constraint down to within a few arcseconds. We obtained an FPP<1\% using \vespa which rule out remaining false positive scenarios not constrained by our observations and hence the planet is validated.

\subsubsection{EPIC 212132195}
This target was observed in K2/C5 \& C16 but we detected the \Porb$=$26.2 d candidate marginally in C5, due to higher scatter in the second half of the campaign. The candidate was previously analyzed by \citet{2018MayoC1to10} using only the C5 data and did not validate it due to the lack of AO/speckle data which we provide in this work coupled with the C16 light curve. Archival POSS1 images help rule out background EBs. We recomputed FPP using \vespa and yielded FPP<1\% and hence the planet is validated. We also note that the star has a 69\% thin disc probability based on the TIC-Gaia catalog \citet{2020CarilloTGv8}.

\subsubsection{EPIC 212161956}
We detected the candidate with \Porb=7.2 d in both in K2/C5 \& 18 light curves. \panstarrs image shows two faint stars near the edge of the photometric aperture. As discussed in \S \ref{sec:dilution}, multi-aperture analysis rules out the nearby stars as potential sources of the signal. Our contrast curve extends the constraint down to within a few arcseconds. We obtained an FPP<1\% using \vespa which rule out remaining false positive scenarios not constrained by our observations and hence the planet is validated.

\subsubsection{EPIC 212278644}
This target was observed in K2/C6 and we detected the \Porb$=$12.4 d candidate in both \everest and \ktwosff light curves. \panstarrs image show a faint star within the photometric aperture which we ruled out as a potential nearby EB in \S \ref{sec:dilution}. We obtained an FPP<1\% using \vespa which rule out remaining false positive scenarios not constrained by our observations and hence the planet is validated.

\subsubsection{EPIC 212330265}
This target was observed in K2/C6 and we detected the candidate with \Porb$=$4.2 d recently reported by \citet{2019KruseC0to8}. \panstarrs images show no nearby, contaminating stars within the photometric aperture and archival POSS1 images help rule out potential background EBs. We recomputed the FPP using these constraints which resulted to FPP<1\% and hence the planet is validated.

\subsubsection{EPIC 212398508}
This target was observed in K2/C6 and we detected the \Porb$=$46.4 d candidate reported recently by \citet{2019KruseC0to8}. \gaia indicates a nearby star which is not bright enough to reproduce the signal. \panstarrs images show no other nearby, contaminating stars within the photometric aperture and archival POSS1 images help rule out potential background EBs. We recomputed the FPP using these constraints which resulted to FPP<1\% and hence the planet is validated.

\subsubsection{EPIC 212495601}
This target was observed in K2/C6 \& C17 and but we did not detect the \Porb=21.7 d candidate in C17 data due to noisy light curves. \panstarrs images show no nearby, contaminating stars within the photometric aperture and our contrast curves further extend the constraint down to within a few arcseconds. We obtained an FPP<1\% using \vespa which rule out remaining false positive scenarios not constrained by our observations and hence the planet is validated.

\subsubsection{EPIC 212543933}
This target was observed in K2/C6 and we detected the \Porb$=$21.7 d candidate in both \everest and \ktwosff light curves. \panstarrs images rule out potential nearby EB within the photometric aperture. We reran \vespa using our speckle contrast curve and obtained an FPP<1\% and hence the planet is validated.

\subsubsection{EPIC 212420823}
This target was observed in K2/C6 and we detected the \Porb=9 d candidate in both \everest and \ktwosff light curves. \panstarrs images rule out potential nearby EB within the photometric aperture and our contrast curve further extends the constraint down to within a few arcseconds. We obtained an FPP<1\% using \vespa which rule out remaining false positive scenarios not constrained by our observations and hence the planet is validated.

\subsection{Multi-planet systems}

\subsubsection{EPIC 212297394}
This target was observed in K2/C6 and we detected two planet candidates with \Porb=2.29 and 5.21 d. Both candidates were previously detected by \citet{2019KruseC0to8} but only the inner planet has so far been validated \citet{2019HellerTLS2} (Not clear why). \panstarrs image and our contrast curve further rules out nearby EBs. We obtained an FPP<1\% and hence the outer planet is validated.

\subsubsection{EPIC 212440430}
This target was observed in C6 \& C17 and we detected two planets with \Porb 4.16 d and 20.0 d (approximately in 5:1 \Porb resonance) in both in C6 and C17 light curves but only marginally in C17 due to higher scatter in the second half of the campaign. The outer planet was previously detected by \citet{2019KruseC0to8} using C5 light curve while the inner planet is a new detection. \panstarrs image and our contrast curve rules out potential nearby EBs. %Owing to multiplicity boost (CITE), these evidences significantly lowers their FPP (see Table \ref{tab:planet}). %Pope only reported one candidate while Cruz reported both candidates and and Heller validated the inner (2-day) planet.  
%https://arxiv.org/pdf/1905.09038.pdf

\section{Planet Validation}
%NEB (Nearby Eclipsing Binary): Indicates that the TESS detection was caused by a nearby eclipsing binary contaminating the TESS aperture, as determined from follow-up photometry that resolved the nearby eclipsing binary. BEB (Blended Eclipsing Binary): Indicates that an eclipsing binary blended in the follow-up and TESS apertures caused the TESS detection. These systems are generally classified as BEB as a result of a chromatic transit depth in follow-up photometry.  EB (Eclipsing Binary): Indicates that the TESS detection is caused by an event on target, but the event is too deep to be caused by an orbiting planet. 

\begin{comment}
\begin{figure*}
    \subfloat[EPIC-211314705b]{\includegraphics[clip,trim={4.5cm 1.75cm 4.5cm 0},width=0.3\textwidth]{epic211314705_4x4-eps-converted-to.pdf}}
    \hfill
    \subfloat[EPIC-211579112b]{\includegraphics[clip,trim={4.5cm 1.75cm 4.5cm 0},width=0.3\textwidth]{epic211579112_4x4-eps-converted-to.pdf}}
    \hfill
    \subfloat[EPIC-211763214b]{\includegraphics[clip,trim={4.5cm 1.75cm 4.5cm 0},width=0.3\textwidth]{epic211763214_4x4-eps-converted-to.pdf}}
    \hfill
    \subfloat[EPIC-211965883b]{\includegraphics[clip,trim={4.5cm 1.75cm 4.5cm 0},width=0.3\textwidth]{epic211965883_4x4-eps-converted-to.pdf}}
    \hfill
    \subfloat[EPIC-212088059b]{\includegraphics[clip,trim={4.5cm 1.75cm 4.5cm 0},width=0.3\textwidth]{epic212088059_4x4-eps-converted-to.pdf}}
    \hfill
    \subfloat[EPIC-212132195b]{\includegraphics[clip,trim={4.5cm 1.75cm 4.5cm 0},width=0.3\textwidth]{epic212132195_4x4-eps-converted-to.pdf}}
    \hfill
\includegraphics[clip,trim={0 0 0 0},width=0.49\textwidth]{fig_cc.png}
\caption{Subaru/IRCS images of the host stars. \textcolor{red}{Combine cc with inset AO images.}}
\label{fig:ao}
\end{figure*}

\begin{figure}
    \includegraphics[clip,trim={0 0 0 0},width=0.49\textwidth]{fig_cc_plot.png}
    \caption{5-$\sigma$ contrast curves extracted from the reduced Subaru/IRCS images in Figure \ref{fig:ao}.}
    \label{fig:cc}
    \end{figure}
\end{comment}

\subsection{M-R relation}
%Assuming that the M-R relation can be described as a power law with a dispersion that is constant and normally distributed, we find that M/M⊕ = 2.7(R/R⊕)^1.3, a scatter in mass of 1.9M⊕, and a mass constraint to physically plausible densities, is the "best-fit" probabilistic M-R relation for the sample of RV-measured transiting sub-Neptunes (Rpl < 4 R⊕).

We estimate the masses of each of the candidate planet based on their precise radii using the M-R relation \citep{2016WolfgangMRrelation}), applicable for transiting sub-Neptunes ($R_p$ < 4 \rearth) and assuming that the M-R relation can be described as a power law with a dispersion that is constant and normally distributed.

\textcolor{red}{See newer references for Mass-Radius relation for small planets: \citep[e.g.,][]{2018VanEylenRadiusValley,2017FultonGap}.}

\subsection{Interesting systems/Characterization targets}
% \item expanded vespa description/discussion
% \item add figure showing transits of multi-planet systems
% \item small/large aperture comparison
% \item archival imaging (if high proper motion)
% \item run vespa with phase-folded lightcurves from K2SFF
% \item compute mass upper limits (if any)
% \item decide on validated planets w/o imaging

%USP?

%\subsection{Mass characterization via precision RV}
% Our validated planet sample includes 18 planets smaller than 2R , several of which orbit bright host stars (J ≈ 7–9). These small planets thus present opportunities for detailed studies of terrestrial worlds via either RV measurements or transmission spectroscopy. 

Using the empirical mass-radius relation for small planets < 14.26\rearth from \citet{2017ChenKippingMRrelation}, we compute the maximum likelihood masses $m_p$
of our planet candidates and single transit events to then infer their expected RV semi-amplitudes using
\begin{equation}
    K_{RV}=2.4\ms \Big(\frac{m_p}{5M_{\oplus}}\Big) \Big(\frac{M_s}{0.5M_{\odot}}\Big)^{-2/3} \Big(\frac{P}{10 d}\Big)^{-1/3} 
\end{equation}

These values are shown in the first panel of Figure~\ref{fig:K} verson the V magnitude superposed with the set of confirmed transiting planets from the NASA Exoplanet Archive. Many existing high performance RV spectrographs are stable at the level of a few cm/s but RV observations are often limited by photon noise and intrinsic stellar activity at the level of 1 to a few m/s, even for relatively inactive stars (Fischer et al. 2016). The majority of our targets have expected $K_{RV}$ values in excess of this typical RV sensitivity limit and are reported in Table X.%~\ref{tab:planet}.


\begin{figure}
    \includegraphics[width=0.49\textwidth]{fig_MR.png}
    \caption{Mass estimates based on the Mass-Radius relation of \citet{2016WolfgangMRrelation}. The various curves denote the densities from H to Fe. %The majority of the validated planets reside within the Fulton gap denoted by black vertical lines.
    }
    \label{fig:MR}
\end{figure}

\begin{figure}
    \includegraphics[width=0.49\textwidth]{fig_RV_mag.png}
    \caption{\textcolor{red}{RV semi-amplitude as a function of \kepler magnitude. Our brightest targets have amplitudes <8 m/s  detectable with current generation spectrographs.}}
    \label{fig:K}
\end{figure}

\begin{figure}
    \includegraphics[width=0.49\textwidth]{fig_MR_comparison.png}
    \caption{Mass estimate comparison between \citet{2016WolfgangMRrelation} and \citet{2014Weiss&Marcy}.}
    \label{fig:MR_comparison}
\end{figure}

\subsubsection{Multi-aperture light curve analysis}
There have been six validated planets shown to be false positives by follow-up observations and analysis \citep{2017Cabrera3FP,2017Shporer3FP}. We briefly examine whether these instances are a cause for concern in our own results.

In the case of \citet{2017Cabrera3FP}, they found that two false positives exhibited increased transit depths for larger aperture masks (suggesting a nearby star was responsible for the eclipses) while the third showed a secondary eclipse at phase = 0.62 when they used a different data reduction process. The first two false positives would have failed the multi-aperture size test %variable-sized mask test 
we apply via our diagnostic plots, while the secondary eclipse from the third false positive would have been caught through a combination of our data reduction process and the "model-shift uniqueness" test we apply \citep{2016CoughlinModelShiftTest}.

As for \citet{2017Shporer3FP}, the vespa fit to the available photometry for each false positive was very poor and all three of the false positives were reported to be very large "planets." We addressed these concerns in two ways. First, we decided to only use 2MASS photometry in order to avoid systematic errors between photometric bands. Second, we chose not to validate any planet candidates larger than 8 $R\oplus$, since a candidate of that size or larger could actually be a small M dwarf. The only exception to this rule is if there are RV measurements that can rule out the eclipsing binary scenario, in which case we do report the FPP (and validate for FPP < 0.001) regardless of planet size.

\begin{itemize}
\item Our transit analyses (without density priors) yield mean stellar densities ($\rho_{*,LC}$) within 1$\sigma$ of the values from our independent assessment (\S X).
\item vespa FPP
\item gaia
\item AO imaging
\item using contrast curves and isochrones inputs listed in Table X, we find an FPP of X
\item From the observed transit depth, an EB with 100\% eclipse depths that is less than X mag fainter than the primary could reproduce the observed transit depth
\end{itemize}
% 1. There is not a composite spectrum.
% 2. There is not a companion in the aperture. (This was determined from archival imaging.)
% 3. There is not a companion in AO and/or speckle images. (This was determined from our AO and speckle images as well as any images for our candidates uploaded to https://exofop.ipac.caltech.edu/k2/ before 2017 August 9.)
% 4. There is no evidence of a secondary eclipse (at any arbitrary phase).
% 5. There is not an ephemeris match (see Section 2.4). If any of the above were false, the FPP was not re-
% ported in Table 4 and the candidate was not validated regardless of the FPP value vespa provided.

\subsubsection{NOT/FIES}
We also used the FIbre-fed Ec\'helle Spectrograph \citep[FIES;][]{1999FrandsenLindbergFIES,2014TeltingFIES} on the 2.56-m Nordic Optical Telescope (NOT) of Roque de los Muchachos Observatory in La Palma, Spain to collect high-resolution ($R\approx$67,000) spectra for X campaign X candidates (EPIC-XXXXXXXX, EPIC-XXXXXXXX, etc.). The observations were carried out between X to X UTC, within observing programs XXX and XXX. We followed the same strategy as in \citet{2013GandolfiKepler77} and traced the RV drift of the instrument by bracketing the science exposures with 90-sec ThAr spectra. We reduced the data using standard IRAF routines and extracted the RVs via multi-order cross-correlations using different RV standard stars observed with the same instrument.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The NASA {\it K2} mission \citep{2014HowellK2} has extended the legacy of {\it Kepler} by monitoring stars a series of $\sim$100 deg$^2$ fields along the ecliptic plane for $\sim$80 days each. {\it K2} has so far discovered $\sim$300 statistically validated or confirmed exoplanets exhibiting a broad diversity of properties and system architectures \citep[e.g.][]{2016CrossfieldC1to5,2018MayoC1to10}. The wider sky coverage of {\it K2} (compared to {\it Kepler}) has enabled discoveries of planets in a variety of stellar environments, including the first transiting multi-planet system in a cluster \citep{2018ALivingstonHyades}, as well as a planet orbiting a 5--10 Myr star \citep{2016DavidK2-33}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Using the mass-radius relation of \citet{2017ChenKippingMRrelation}, we estimate a mass of $\sim$4\,$M_{\rm{Jup}}$, with large uncertainties. However, because of the possibility that this planet is an inflated hot Jupiter, we consider the possibility that the planet has a mass as low as $\sim$1$\,M_\mathrm{Jup}$. Using Table 5 of \citet{2013ApJS..208....9P}\footnote{The updated version of the table is available at \url{http://www.pas.rochester.edu/~emamajek/EEM_dwarf_UBVIJHK_colors_Teff.txt}} along with the Gaia DR2 values of $\teff$ and $R_\star$ (see Table~\ref{tab:star}), the spectral type and mass of the host star are K6V and 0.68\,$M_\odot$, respectively. The host star mass, measured orbital period, and predicted planet mass result in an expected radial velocity semi-amplitude of $\sim$200--800 m\,s$^{-1}$. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{EPIC-211314705b}
Kepmag = 14.422.
V-Ks color: $M2.5\pm0.2$.
% Has TRES spectrum on ExoFOP (bieryla).
Has Subaru/IRCS AO.
% P = 3.79 d.
Has WIYN/NESSI, TRES


\subsubsection{EPIC-211579112b}
Kepmag = 15.768.
J-H color: $M3.9\pm1.2$.
% No spectra on ExoFOP.
Has Subaru/IRCS AO.
Has WIYN/NESSI
% P = 17.7 d.

\subsubsection{EPIC-211763214b}
Kepmag = 12.529.
V-Ks color: $K3.0\pm2.8$.
% Has TRES spectrum on ExoFOP (bieryla).
Has Subaru/IRCS AO.
Has WIYN/NESSI, TRES
% Predicted mass = $2.34^{+2.11}_{-1.00}$ Mearth.
% Predicted K = $0.58^{+0.52}_{-0.25}$ m/s.
% P = 21.197 d.

\subsubsection{EPIC-211965883b}
Kepmag = 14.138.
V-Ks color: $K6.4\pm0.2$.
Has TSPEC spectrum on ExoFOP (Dressing)
% Dressing+17: $M0V$ (not consistent with Huber).
Has Subaru/IRCS AO.
Has WIYN/NESSI
% Predicted mass = $6.47^{+5.09}_{-2.77}$ Mearth.
% Predicted K = $2.45^{+1.88}_{-1.04}$ m/s.
% P = 10.56 d.
\teff=4211 80,79;
\rstar=0.600 0.027,0.027;
\mstar=0.674 0.014,0.012 according to Table 4 of \citet[]{2017ApJ...836..167D}.
%see https://docs.google.com/spreadsheets/d/1Giwxhjnc7kq1K1-IfWDI1DZpVcCfyzZgHBgs_VHn-3w/edit#gid=0

\subsubsection{EPIC-212088059b}
Kepmag = 14.757.
V-Ks color: $M1.6\pm0.3$.
% No spectra on ExoFOP.
Has Subaru/IRCS AO.
Has WIYN/NESSI
% P = 10.37 d.

\subsubsection{EPIC-212132195b}
Kepmag = 11.670.
V-Ks color: $K3.4\pm0.1$.
Has SpeX spectrum on ExoFOP (Dressing).
% Dressing+17: $K3V$.
Has Subaru/IRCS AO.
Has WIYN/NESSI, TRES
% Predicted mass = $5.59^{+4.20}_{-2.33}$ Mearth.
% Predicted K = $1.50^{+1.14}_{-0.61}$ m/s.
% P = 26.195 d.

\subsubsection{EPIC-212161956b}
Kepmag = 14.778.
% No spectra on ExoFOP.
V-Ks color: $K5.2\pm0.2$.
Has WIYN/NESSI
% Predicted mass = $4.94^{+3.71}_{-1.94}$ Mearth.
% Predicted K = $2.29^{+1.69}_{-0.91}$ m/s.
% P = 7.19 d.

\subsubsection{EPIC-212278644b}
Kepmag = 13.949.
V-Ks color: $G5.1\pm1.1$.
% No spectra on ExoFOP.
Has WIYN/NESSI
% Predicted mass = $6.34^{+4.99}_{-2.72}$ Mearth.
% Predicted K = $1.81^{+1.43}_{-0.76}$ m/s.
% P = 12.43 d.
Has recon spec at McDonald 2.7m (B. Cochran)

\subsubsection{EPIC-212297394b}
Kepmag = 14.138.
V-Ks color: $K2.3\pm0.2$.
% No spectra on ExoFOP.
Has WIYN/DSSI on ExoFOP (Everett)
Has FIES
% Possible multi -- see ESPRINT spreadsheet.
% Predicted mass = $5.59^{+4.20}_{-2.26}$ Mearth.
% Predicted K = $2.35^{+1.77}_{-0.98}$ m/s.
% P = 5.21 d.

\subsubsection{EPIC-212330265b}
Kepmag = 14.949.
J-H color: $K5.1\pm2.4$.
% No spectra on ExoFOP.
Has WIYN/NESSI
% Predicted K = 1.3 m/s.
% P = 4.174 d.

\subsubsection{EPIC-212398508b}
Kepmag = 13.629.
V-Ks color: $K4.0\pm3.4$.
% No spectra on ExoFOP.
Has WIYN/NESSI
% Predicted mass = $6.47^{+5.09}_{-2.70}$ Mearth.
% Predicted K = $1.29^{+1.01}_{-0.54}$ m/s.
% P = 46.42 d.
Has recon spec at McDonald 2.7m (B. Cochran)

\subsubsection{EPIC-212420823b}
%ask 
Kepmag = 14.166.
V-Ks color: $K2.1\pm0.3$.
% No spectra on ExoFOP.
Has WIYN/NESSI
Has FIES
% Predicted mass = $5.48^{+4.11}_{-2.28}$ Mearth.
% Predicted K = $1.91^{+1.43}_{-0.79}$ m/s.
% P = 9.03 d.
% TTVs?

\subsubsection{EPIC-212440430b}
Kepmag = 13.267.
V-Ks color: $G6.0\pm0.9$.
% No spectra on ExoFOP.
Has WIYN/DSSI on ExoFOP (Everett)
% Predicted mass = $8.47^{+6.36}_{-3.73}$ Mearth.
% Predicted K = $2.04^{+1.61}_{-0.90}$ m/s.
% P = 19.99 d.
% Possible multi -- see ESPRINT spreadsheet.
% KEST note: $McDonald: Teff=5780+/-49 K, [Fe/H]=-0.02+/-0.03 dex, logg=4.44+/-0.12 (cgs), vsini=3.31+/-0.29 km/s, RV=-22.275+/-0.064 km/s$
Has recon spec at McDonald 2.7m (B. Cochran)

%\subsubsection{EPIC-212480208b}
%Kepmag = 10.892.
%V-Ks color: $G6.3\pm2.1$.
%Has TRES spectrum on ExoFOP (Bieryla).
%Has WIYN/DSSI on ExoFOP (Everett).
%Has WIYN/NESSI
% Predicted mass = $0.10^{+0.10}_{-0.05}$ Mearth.
% Predicted K = $0.03^{+0.03}_{-0.02}$ m/s.
% P = 10.09 d.
% KEST note: $RV=-12.731 +/- 1.453 km/s (RAVE survey). Mc Donald Mar16: Teff=5640+/-51 K, logg= 4.31+/-0.06 (cgs), [Fe/H]=-0.27+/-0.02 dex, vsini=3.15+/-0.32, RV=-10.55+/-0.24$ km/s (see PICK2\_201603.txt). Prot=30 days? Super cool object but super tough case!
%Has recon spec at McDonald 2.7m (B. Cochran)

\subsubsection{EPIC-212495601b}
Kepmag = 13.821.
V-Ks color: $G5.2\pm1.1$.
% No spectra on ExoFOP.
Has WIYN/NESSI
% Predicted mass = $5.26^{+4.14}_{-2.13}$ Mearth.
% Predicted K = $1.40^{+1.08}_{-0.57}$ m/s.
% P = 21.67 d.
Has recon spec at McDonald 2.7m (B. Cochran)

% \subsubsection{EPIC-212496592b}
% Kepmag = 12.966.
% V-Ks color: $K2.1\pm0.1$.
% Has TRES spectrum on ExoFOP (Bieryla).
% Has WIYN/DSSI on ExoFOP (Everett)
% Predicted mass = $2.65^{+2.19}_{-1.07}$ Mearth.
% Predicted K = $1.33^{+1.14}_{-0.55}$ m/s.
% P = 2.86 d.
% KEST note: $Mc Donald (Mar 2016): Teff = 5180+/-73 K, logg = 4.44+/-0.12 (cgs), [Fe/H] = -0.04+/-0.03 dex, vsini=1.85+/-0.22, RV= -9.02+/-0.16 km/s$ (see PICK2\_201603.txt).

\subsubsection{EPIC-212543933b}
Kepmag = 14.010.
V-Ks color: $G5.0\pm1.5$.
No spectra on ExoFOP.
Has WIYN/DSSI on ExoFOP (everett).
Predicted mass = $6.21^{+4.89}_{-2.66}$ Mearth.
Predicted K = $2.11^{+1.72}_{-0.88}$ m/s.
P = 7.8 d.
Bill Cochran got recon spec at McDonald 2.7m during May run.

\subsubsection{EPIC-212563850b}
Kepmag = 13.172.
V-Ks color: $K6.6\pm0.2$.
% No spectra on ExoFOP.
Has WIYN/NESSI
% Predicted mass = $1.13^{+0.85}_{-0.44}$ Mearth.
% Predicted K = $0.51^{+0.41}_{-0.20}$ m/s.
% P = 14.3 d.
Has recon spec at McDonald 2.7m (B. Cochran)

% \subsubsection{EPIC-212572439b}
% Kepmag = 12.835.
% V-Ks color: $K1.2\pm0.5$.
% Has TRES spectrum on ExoFOP (bieryla).
% Has TSPEC spectrum on ExoFOP (dressing), classified as K2V.
% Has SpeX spectrum on ExoFOP (dressing), classified as K2V.
% Has WIYN/DSSI on ExoFOP (everett).
% Has Gemini/DSSI on ExoFOP (everett).
% Predicted mass = $27.63^{+23.85}_{-12.80}$ Mearth.
% Predicted K = $15.01^{+13.13}_{-6.98}$ m/s.
% P = 2.58 d.
% Possible false positive based on DAVE pipeline (http://keplertcert.seti.org/DAVE/). Significant centroid offset measured. See the full report at: http://keplertcert.seti.org/DAVE/AllK2/Output/212572439/
% Possible false positive = Yes (Suspect contamination from EPIC 212351048.)

%-----------------------ADDITIONAL c16-------------------
\subsubsection{212178066}
% saturated based on Yu+16; https://arxiv.org/pdf/1803.04091.pdf
Bill Cochran got recon spec at McDonald 2.7m
has FASTcam Lucky imaging

\subsubsection{251319382}
3-planet system.
Bill Cochran got recon spec at McDonald 2.7m
TRES extracted spectra on ExoFOP (bieryla)
has FASTcam Lucky imaging

\subsubsection{211502222}
3-planet system.
Bill Cochran got recon spec at McDonald 2.7m
TRES extracted spectra on ExoFOP (bieryla)
has FASTcam Lucky imaging

\subsubsection{212048748}
bright M-dwarf.
Bill Cochran got recon spec at McDonald 2.7m
Has Subaru/IRCS AO.

\subsubsection{212081533}
Bill Cochran got recon spec at McDonald 2.7m
Has Subaru/IRCS AO.

% \subsubsection{EPIC-211446060b}
% Very nice candidate! M67 cluster member! Short transit duration suggests a dwarf host, maybe a warm Jupiter if the star is a dwarf. 

% \subsubsection{EPIC-212737443b}
% Kepmag = 14.461.
% J-H color: $M4.3\pm1.9$.
% Has TSPEC spectrum on ExoFOP (dressing), classified as K3V.
% Observing with WIYN/NESSI this semester.
% Predicted mass = $5.26^{+3.76}_{-2.13}$ Mearth.
% Predicted K = $1.95^{+1.44}_{-0.78}$ m/s.
% P = 13.6 d.

%Davide for FIES
%WIYN/NESSI: Livingston (or Howell/Everett)
%WIYN/DSSI: Howell/Everett (usually)
%McDonald: B. Cochran/ M. Endl


\begin{figure*}
    \includegraphics[width=1\textwidth]{fig_with-without-rhostar-prior.png}
\caption{Difference of resulting MCMC best-fit transit parameters with and without stellar density prior for each star (denoted by its last 4 EPIC numbers).}
\label{fig:rhostar-prior}
\end{figure*}



==> tables/tab_ao.tex <==

211941472

Separation (arcsec) = 0.203
Position angle (degr. N through E) = 117.346
Magnitude difference = 0.37

832nm
------
Separation (arcsec) = 0.203
Position angle (degr. N through E) = 116.595
Magnitude difference = 0.32

211886472
Filter (nm) = 692
Separation (arcsec) = 0.323
Position angle (degr.) = 278.867
Mag. difference = 4.015

Filter (nm) = 880
Separation (arcsec) = 0.326
Position angle (degr.) = 279.746
Mag. difference = 3.767


==> tables/tab_lc.tex <==
EPIC      & c5           & c6           & c16          & c17          & c18          \\
\hline
211314705 & $\checkmark$ &              &              &              &              \\
211579112 & $\checkmark$ &              &              &              &              \\
211763214 & $\checkmark$ &              & $\checkmark$ &              & $\checkmark$ \\
211965883 & $\checkmark$ &              &              &              &              \\
212088059 & $\checkmark$ &              & $\checkmark$ &              & $\checkmark$ \\
212132195 & $\checkmark$ &              &              &              &              \\
212161956 & $\checkmark$ &              &              &              &              \\
212278644 &              & $\checkmark$ &              &              &              \\
212297394 &              & $\checkmark$ &              &              &              \\
212330265 &              & $\checkmark$ &              &              &              \\
212398508 &              & $\checkmark$ &              &              &              \\
212420823 &              & $\checkmark$ &              &              &              \\
212440430 &              & $\checkmark$ &              & $\checkmark$ &              \\
212495601 &              & $\checkmark$ &              & $\checkmark$ &              \\
212543933 &              & $\checkmark$ &              &              &  
     \\
%212563850 &              & $\checkmark$ &              & $\checkmark$ &              \\
\hline

==> tables/tab_obs2.tex <==
\begin{tabular}{ccccccccc}
\hline
EPIC & C5 & C6 & C16 & C17 & C18 & AO$^a$ & SI$^b$ & RS$^c$ \\
\hline
212072539 & \cmark & & \cmark & & \cmark &  &   &   \\
212081533 & & & \cmark & & & \cmark &   &  \cmark\\
212088059 & \cmark & & \cmark & & \cmark &  & \cmark & \cmark  \\ %dressing
212096658 & \cmark & & \cmark & & \cmark &  &   &   \\
212132195 & \cmark & & & & \cmark & \cmark & \cmark &   \\
212138198 & \cmark & & & & \cmark &  & \cmark  & \cmark \\ %Gemini-N/DSSI (692,880nm) %isaacson
212178066 & & & \cmark & & \cmark &  &   &  \cmark\\
212204403 & & & \cmark & & &  &   &  \cmark\\
212278644 & & \cmark & & & &  &   &  \cmark\\
212297394 & & \cmark & & & &  & \cmark &   \\
212315941 & & \cmark & & & &  & \cmark &   \\
212330265 & & \cmark & & & &  &   & \cmark \\ %dressing
212398508 & & \cmark & & & &  & \cmark &  \cmark\\
212422536 & & \cmark & & & &  &   &   \\
212428509 & & \cmark & & \cmark & &  & \cmark & \cmark \\ %isaacson
212435047 & & \cmark & & \cmark & &  & \cmark &  \cmark \\ %isaacson
212440430 & & \cmark & & \cmark & &  & \cmark &  \cmark\\
212495601 & & \cmark & & \cmark & &  & \cmark &  \cmark\\
212534729 & & \cmark & & \cmark & &  & \cmark &  \cmark\\
212543933 & & \cmark & & & &  & \cmark &  \cmark\\
212570977 & & \cmark & & \cmark & &  & \cmark &  \cmark \\ %isaacson
212585579 & & \cmark & & & &  & \cmark & \cmark \\ %isaacson
212586030 & & \cmark & & \cmark & &  & \cmark & \cmark \\ %isaacson
212587672 & & \cmark & & \cmark & &  & \cmark & \cmark \\
212628098 & & \cmark & & \cmark & &  &   &   \\
212634172 & & \cmark & & \cmark & &  &   & \cmark \\ %dressing
212639319 & & \cmark & & \cmark & &  & \cmark &  \cmark \\ %isaacson
212690867 & & \cmark & & \cmark & &  &   & \cmark \\ %dressing
212703473 & & \cmark & & & &  & \cmark &  \cmark\\
212773272 & & \cmark & & \cmark & &  & \cmark & \cmark \\
212797028 & & \cmark & & \cmark & &  & \cmark &   \\
251288417 & & & \cmark & & &  &   & \cmark \\ %dressing
251319382 & & & \cmark & & &  & \cmark &  \cmark\\
212178066 & & & \cmark & & \cmark &  &   &  \cmark\\
212204403 & & & \cmark & & &  &   &  \cmark\\
212278644 & & \cmark & & & &  &   &  \cmark\\
212297394 & & \cmark & & & &  & \cmark &   \\
212315941 & & \cmark & & & &  & \cmark &   \\
212330265 & & \cmark & & & &  &   & \cmark \\ %dressing
212398508 & & \cmark & & & &  & \cmark &  \cmark\\
212422536 & & \cmark & & & &  &   &   \\
212428509 & & \cmark & & \cmark & &  & \cmark & \cmark \\ %isaacson
212435047 & & \cmark & & \cmark & &  & \cmark &  \cmark \\ %isaacson
212440430 & & \cmark & & \cmark & &  & \cmark &  \cmark\\
212495601 & & \cmark & & \cmark & &  & \cmark &  \cmark\\
212534729 & & \cmark & & \cmark & &  & \cmark &  \cmark\\
212543933 & & \cmark & & & &  & \cmark &  \cmark\\
212570977 & & \cmark & & \cmark & &  & \cmark &  \cmark \\ %isaacson
212585579 & & \cmark & & & &  & \cmark & \cmark \\ %isaacson
212586030 & & \cmark & & \cmark & &  & \cmark & \cmark \\ %isaacson
212587672 & & \cmark & & \cmark & &  & \cmark & \cmark \\
212628098 & & \cmark & & \cmark & &  &   &   \\
212634172 & & \cmark & & \cmark & &  &   & \cmark \\ %dressing
212639319 & & \cmark & & \cmark & &  & \cmark &  \cmark \\ %isaacson
212690867 & & \cmark & & \cmark & &  &   & \cmark \\ %dressing
212703473 & & \cmark & & & &  & \cmark &  \cmark\\
212773272 & & \cmark & & \cmark & &  & \cmark & \cmark \\
212797028 & & \cmark & & \cmark & &  & \cmark &   \\
251288417 & & & \cmark & & &  &   & \cmark \\ %dressing
251319382 & & & \cmark & & &  & \cmark &  \cmark\\
%211335816, 211428897, 212150006, 212099230, 212420823, 212470904, 212563850, 212572439,  212684448, 211446060, 211604981, 211858489, 212036875, 212048748, 251554286, 212628477
\hline
\multicolumn{9}{l}{$^a$ Adaptive optics}\\
\multicolumn{9}{l}{$^b$ Speckle imaging}\\
\multicolumn{9}{l}{$^c$ Reconnaissance spectroscopy}\\
\end{tabular}
% %see https://docs.google.com/spreadsheets/d/1Giwxhjnc7kq1K1-IfWDI1DZpVcCfyzZgHBgs_VHn-3w/edit#gid=994714091
% EPIC      & photometry        & AO imaging  &  /lucky imaging & recon.  specarchival imaging \\ \hline %& parallax\\ \hline
% 211314705 & \ktwo/c5           & Subaru/IRCS & WIYN/NESSI & TRES & - \\%& Gaia DR2 \\ %NOT in Kruse+2019
% 211579112 & \ktwo/c5           & Subaru/IRCS & WIYN/NESSI & - & - \\%& Gaia DR2 \\ %planet candidates in or near the habitable zone with planet radii small than 2 R⊕ also found recently by Kruse+2019
% 211763214 & \ktwo/c5,16,18  & Subaru/IRCS   & WIYN/NESSI,DSSI & - %TRES: no uncertainty 
% & POSS \\%& Gaia DR2\\
% 212088059 & \ktwo/c5,16,18  & Subaru/IRCS & WIYN/NESSI & - & POSS \\%& Gaia DR2\\
% 212132195 & \ktwo/c5           & Subaru/IRCS & WIYN/NESSI,DSSI & SpEX, TRES & POSS \\%& Gaia DR2\\
% 212161956 & \ktwo/c5,18        &     -        & WIYN/NESSI & - & POSS \\%& Gaia DR2\\
% 212278644 & \ktwo/c6           &     -       &  -          & McDonald/Tull & - \\%& Gaia DR2\\ %NOT in Kruse+2019
% 212297394 & \ktwo/c6           &     -        & WIYN/DSSI  & NOT/FIES & - \\%& Gaia DR2\\ %multiplanet; 0.2 has 2.28896-d based on TLS survey II (Heller+2019)
% 212330265 & \ktwo/c6           &     -        &  -          & -  & POSS \\%& Gaia DR2\\ 
% 212398508 & \ktwo/c6           &     -        & WIYN/NESSI & McDonald/Tull & POSS \\%& Gaia DR2\\
% 212420823 & \ktwo/c6           &     -        & WIYN/NESSI & NOT/FIES & - \\%& Gaia DR2\\
% 212440430 & \ktwo/c6,17      &       -      & WIYN/DSSI & McDonald/Tull & - \\%& Gaia DR2\\
% 212495601 & \ktwo/c6,17      &       -      & WIYN/NESSI & McDonald/Tull & - \\%& Gaia DR2 \\
% 212543933 & \ktwo/c6           &     -        & WIYN/DSSI & McDonald/Tull & - \\%& Gaia DR2\\
% %212563850 & \ktwo/c6,17      &             & WIYN/NESSI & McDonald/Tull & POSS1 & Gaia DR2\\  %FP
% %\hline
% % additional
% %212178066 & \ktwo/c16 &             & FASTcam & McDonald/Tull \\
% %251319382 & \ktwo/c16 &             & FASTcam & McDonald/Tull, TRES \\
% %211502222 & \ktwo/c16 &             & FASTcam & McDonald/Tull, TRES \\
% %212048748 & \ktwo/c16 & Subaru/IRCS &         & McDonald/Tull \\
% %212081533 & \ktwo/c16 & Subaru/IRCS &         & McDonald/Tull \\
% %TSPEC
% % http://www.astro.caltech.edu/palomar/observer/200inchResources/tspecspecs.html
% %WIYN/NESSI (NASA Exoplanet Star (and)   Imager) is a   instrument that utilizes two electron-multiplying CCD cameras to capture   images in two colors simultaneously.   observations provide resolutions at or near the diffraction limit of the telescope allowing companion detection and characterization to delta magnitudes of approximately 5. NESSI will have remote controlled filter wheels in each beam, split by the dichroic at 686.4nm.
% % http://www.wiyn.org/Instruments/wiynnessi.html
% %DSSI (Differential   Survey Instrument, built by Elliott Horch, SCSU) provides simultaneous 2-band diffraction-limited high-resolution optical imaging (FWHM~0.05" at 650nm) of targets as faint as V~15, over a ~2.8 arcsecond field-of-view. DSSI will be offered once or twice in the semester, depending on demand. The visiting DSSI instrument team will operate a mini-queue program during these runs and will take all observations for successful proposers. The DSSI team will provide their standard pipeline-reduced data products (includes reconstructed image and sensitivity curve) to PIs. There is no requirement to collaborate with the DSSI team for this level of service. Details of the use of DSSI at WIYN are given in Howell et al., 2011, AJ, 142, 19, Horch et al., 2012, AJ, 143, 10, and 2011, AJ, 141, 180. The PI for this program is Steve Howell (NASA Ames Research Center).
% %TRES (Tillinghast Reflector Echelle Spectrograph) is a fiber-fed (sky+object+calibration spectrum) optical echelle spectrograph on the 1.5-meter Tillinghast telescope at the Smithsonian Astrophysical Observatory's Fred L. Whipple Observatory on Mt. Hopkins in Arizona.
% % http://tdc-www.harvard.edu/instruments/tres/
